Dynamic Tolling for Inducing Socially Optimal Traffic Loads

How to design tolls that induce socially optimal traffic loads with dynamically arriving travelers who make selfish routing decisions? We propose a two-timescale discrete-time stochastic dynamics that adaptively adjusts the toll prices on a parallel link network while accounting for the updates of traffic loads induced by the incoming and outgoing travelers and their route choices. The updates of loads and tolls in our dynamics have three key features: (i) The total demand of incoming and outgoing travelers is stochastically realized; (ii) Travelers are myopic and selfish in that they choose routes according to a perturbed best response given the current latency and tolls on parallel links; (iii) The update of tolls is at a slower timescale as compared to the the update of loads. We show that the loads and the tolls eventually concentrate in a neighborhood of the fixed point, which corresponds to the socially optimal load and toll price. Moreover, the fixed point load is also a stochastic user equilibrium with respect to the toll price. Our results are useful for traffic authorities to efficiently manage traffic loads in response to the arrival and departure of travelers.

==> Dynamic_Routing_Regular (Arxiv)/FigPlots.tex <==
\begin{figure}
\begin{subfigure}{.4\textwidth}
  \centering
  % include first image
  \includegraphics[scale = 0.4]{Figures/3LinkSetting13FlowWPrice.eps}  
  \caption{Parameter setting \ref{enum: Setting1}}
  \label{fig:3LinkFlowProfileL1}
\end{subfigure}
\begin{subfigure}{.4\textwidth}
  \centering
  % include second image
  \includegraphics[scale = 0.4]{Figures/3LinkSetting13Price.eps}
  \caption{Parameter setting \ref{enum: Setting1}}
  \label{fig:3LinkPriceProfileL1}
\end{subfigure}
\begin{subfigure}{.4\textwidth}
  \centering
  % include first image
  \includegraphics[scale = 0.4]{Figures/3LinkSetting3FlowWPrice.eps}  
  \caption{Parameter Setting \ref{enum: Setting2}}
  \label{fig:3LinkFlowProfileL2}
\end{subfigure}
\begin{subfigure}{.4\textwidth}
  \centering
  % include first image
  \includegraphics[scale = 0.4]{Figures/3LinkSetting3Price.eps}  
  \caption{Parameter setting \ref{enum: Setting2}}
  \label{fig:3LinkPriceProfileL2}
\end{subfigure}
\caption{Comparison between the trajectories of discrete time stochastic process \eqref{eq: CombinedDT} (dotted trajectories) and the continuous time approximation to it \eqref{eq: singularPerturbedODE}(solid trajectories) for the case when $\numLinks = 3$, $\meanInflow= 0.1$, $\meanOutflow = 0.1$ and \(a=0.0015\) (i.e. \ref{enum: Setting1}) in \textsf{(A),(B)} while $\meanInflow= 0.1$, $\meanOutflow = 0.05$ and \(a=0.0015\) (i.e. \ref{enum: Setting2}) \textsf{(C),(D)}. For discrete time trajectories above we have averaged out the trajectories from \(20\) independent rollouts. }
\label{fig:3LinkSetting}
\end{figure}


\begin{figure}
\begin{subfigure}{.4\textwidth}
  \centering
  % include first image
  \includegraphics[scale = 0.4]{Figures/3LinkSetting13FlowWOPrice.eps}  
  \caption{Paramter setting \ref{enum: Setting3}}
  \label{fig:3LinkFlowPriceProfileL1NoToll}
\end{subfigure}
\begin{subfigure}{.4\textwidth}
  \centering
  % include second image
  \includegraphics[scale = 0.4]{Figures/3LinkSetting3FlowWOPrice.eps}
  \caption{Paramter setting \ref{enum: Setting4}}
  \label{fig:3LinkPriceProfileL2NoToll}
\end{subfigure}
\caption{Comparison between flow obtained without toll pricing (solid lines) and socially optimal level (dashed line). The vertical axis represents flow on corresponding link. The horizontal axis represents the time scale which normalized between the continuous trajectory and discrete time trajectory for comparison.  For discrete time trajectories (solid lines) above we have averaged out the trajectories from \(20\) independent rollouts.} 
    \label{fig:3LinkNoPrice}
\end{figure}


\begin{figure}
\begin{subfigure}{.4\textwidth}
  \centering
  % include first image
  \includegraphics[scale = 0.4]{Figures/6LinkSetting14FlowWPrice.eps}  
  \caption{Paramter setting \ref{enum: Setting5}}
  \label{fig:6LinkFlowProfileL1}
\end{subfigure}
\begin{subfigure}{.4\textwidth}
  \centering
  % include second image
  \includegraphics[scale = 0.4]{Figures/6LinkSetting14Price.eps}
  \caption{Paramter setting \ref{enum: Setting5}}
  \label{fig:6LinkPriceProfileL1}
\end{subfigure}
\begin{subfigure}{.4\textwidth}
  \centering
  % include first image
  \includegraphics[scale = 0.4]{Figures/6LinkSetting4FlowWPrice.eps}  
  \caption{Paramter setting \ref{enum: Setting6}}
  \label{fig:6LinkFlowProfileL2}
\end{subfigure}
\begin{subfigure}{.4\textwidth}
  \centering
  % include first image
  \includegraphics[scale = 0.4]{Figures/6LinkSetting4Price.eps}  
  \caption{Parameter setting \ref{enum: Setting6}}
  \label{fig:6LinkPriceProfileL2}
\end{subfigure}
\caption{  Comparison between the trajectories of discrete time stochastic process \eqref{eq: CombinedDiscreteDyn} (dotted trajectories) and the continuous time approximation to it \eqref{eq: singularPerturbedODE}(solid trajectories) for the case when $\numLinks = 6$, $\meanInflow= 0.1$, $\meanOutflow = 0.05$ and \(a=0.0015\) in \textsf{(A),(B)} (i.e. \ref{enum: Setting5})  and $\numLinks = 6$,$\meanInflow= 0.18$, $\meanOutflow = 0.05$ and \(a=0.0015\) \textsf{(C),(D)} (i.e. \ref{enum: Setting6}). For discrete time trajectories above we have averaged out the trajectories from \(20\) independent rollouts. }
\label{fig:6LinkSetting1}
\end{figure}




\begin{figure}
\begin{subfigure}{.4\textwidth}
  \centering
  % include first image
  \includegraphics[scale = 0.4]{Figures/6LinkSetting14FlowWOPrice.eps}  
  \caption{Parameters setting \ref{enum: Setting7}}
  \label{fig:6LinkPriceProfileL1NoToll}
\end{subfigure}
\begin{subfigure}{.4\textwidth}
  \centering
  % include second image
  \includegraphics[scale = 0.4]{Figures/6LinkSetting4FlowWOPrice.eps}
  \caption{Parameters setting \ref{enum: Setting8}}
  \label{fig:6LinkPriceProfileL2NoToll}
\end{subfigure}
\caption{Comparison between flow obtained without toll pricing (solid lines) and socially optimal level (dashed line). The vertical axis represents flow on corresponding link. The horizontal axis represents the time scale which normalized between the continuous trajectory and discrete time trajectory for comparison. For discrete time trajectories (solid lines) above we have averaged out the trajectories from \(20\) independent rollouts. } 
    \label{fig:6LinkNoPrice}
\end{figure}

==> Dynamic_Routing_Regular (Arxiv)/FigPlots_arxiv.tex <==
% \begin{figure}[htp]
% \begin{subfigure}{.4\textwidth}
%   \centering
%   % include first image
%   \includegraphics[scale = 0.4]{Figures/3LinkSetting13FlowWPrice.eps}  
%   \caption{Parameter setting \ref{enum: Setting1}}
%   \label{fig:3LinkFlowProfileL1}
% \end{subfigure}
% \begin{subfigure}{.4\textwidth}
%   \centering
%   % include second image
%   \includegraphics[scale = 0.4]{Figures/3LinkSetting13Price.eps}
%   \caption{Parameter setting \ref{enum: Setting1}}
%   \label{fig:3LinkPriceProfileL1}
% \end{subfigure}
% \begin{subfigure}{.4\textwidth}
%   \centering
%   % include first image
%   \includegraphics[scale = 0.4]{Figures/3LinkSetting3FlowWPrice.eps}  
%   \caption{Parameter Setting \ref{enum: Setting2}}
%   \label{fig:3LinkFlowProfileL2}
% \end{subfigure}
% \begin{subfigure}{.4\textwidth}
%   \centering
%   % include first image
%   \includegraphics[scale = 0.4]{Figures/3LinkSetting3Price.eps}  
%   \caption{Parameter setting \ref{enum: Setting2}}
%   \label{fig:3LinkPriceProfileL2}
% \end{subfigure}
% \caption{Comparison between the trajectories of discrete time stochastic process \eqref{eq: CombinedDT} (dotted trajectories) and the continuous time approximation to it \eqref{eq: singularPerturbedODE}(solid trajectories) for the case when $\numLinks = 3$, $\meanInflow= 0.1$, $\meanOutflow = 0.1$ and \(a=0.0015\) (i.e. \ref{enum: Setting1}) in \textsf{(A),(B)} while $\meanInflow= 0.1$, $\meanOutflow = 0.05$ and \(a=0.0015\) (i.e. \ref{enum: Setting2}) \textsf{(C),(D)}. For discrete time trajectories above we have averaged out the trajectories from \(20\) independent rollouts. }
% \label{fig:3LinkSetting}
% \end{figure}


% \begin{figure}
% \begin{subfigure}{.4\textwidth}
%   \centering
%   % include first image
%   \includegraphics[scale = 0.4]{Figures/3LinkSetting13FlowWOPrice.eps}  
%   \caption{Paramter setting \ref{enum: Setting3}}
%   \label{fig:3LinkFlowPriceProfileL1NoToll}
% \end{subfigure}
% \begin{subfigure}{.4\textwidth}
%   \centering
%   % include second image
%   \includegraphics[scale = 0.4]{Figures/3LinkSetting3FlowWOPrice.eps}
%   \caption{Paramter setting \ref{enum: Setting4}}
%   \label{fig:3LinkPriceProfileL2NoToll}
% \end{subfigure}
% \caption{Comparison between flow obtained without toll pricing (solid lines) and socially optimal level (dashed line). The vertical axis represents flow on corresponding link. The horizontal axis represents the time scale which normalized between the continuous trajectory and discrete time trajectory for comparison.  For discrete time trajectories (solid lines) above we have averaged out the trajectories from \(20\) independent rollouts.} 
%     \label{fig:3LinkNoPrice}
% \end{figure}


\begin{figure}[htp]
\begin{subfigure}{.4\textwidth}
  \centering
  % include first image
  \includegraphics[scale = 0.4]{Figures/6LS14FWP.png}  
  \caption{Loads in (\textbf{S1})}
  \label{fig:6LinkFlowProfileL1}
\end{subfigure}
\begin{subfigure}{.4\textwidth}
  \centering
  % include second image
  \includegraphics[scale = 0.4]{Figures/6LS14P.png}
  \caption{Tolls in (\textbf{S1})}
  \label{fig:6LinkPriceProfileL1}
\end{subfigure}
\begin{subfigure}{.4\textwidth}
  \centering
  % include first image
  \includegraphics[scale = 0.4]{Figures/6LS4FWP.png}  
  \caption{Loads in (\textbf{S2})}
  \label{fig:6LinkFlowProfileL2}
\end{subfigure}
\begin{subfigure}{.4\textwidth}
  \centering
  % include first image
  \includegraphics[scale = 0.4]{Figures/6LS4P.png}  
  \caption{Tolls in (\textbf{S2})}
  \label{fig:6LinkPriceProfileL2}
\end{subfigure}
\caption{Loads and Tolls in discrete-time stochastic update \eqref{eq: FlowDynamics} -- \eqref{eq: PricingDynamics} (dots) and continuous-time dynamical system \eqref{eq: singularPerturbedODE} (solid lines) in \textbf{(S1)} and \textbf{(S2)}.}
\label{fig:6LinkSetting1}
\end{figure}




\begin{figure}[htp]
\begin{subfigure}{.4\textwidth}
  \centering
  % include first image
  \includegraphics[scale = 0.4]{Figures/6LS14FWOP.png}  
  \caption{ Loads in (\textbf{S3})}
  \label{fig:6LinkPriceProfileL1NoToll}
\end{subfigure}
\begin{subfigure}{.4\textwidth}
  \centering
  % include second image
  \includegraphics[scale = 0.4]{Figures/6LS4FWOPThin.png}
  \caption{Loads in (\textbf{S4})}
  \label{fig:6LinkPriceProfileL2NoToll}
\end{subfigure}
\caption{Comparison between loads induced by the discrete-time stochastic update \eqref{eq: FlowDynamics}(solid lines) when \(P_n=0\) and the socially optimal load (dashed lines) in \textbf{(S3)} and \textbf{(S4)}.} 
    \label{fig:6LinkNoPrice}
\end{figure}

==> Dynamic_Routing_Regular (Arxiv)/Preliminaries.tex <==
\section{Preliminaries}

\subsection{Static Routing}

Consider a parallel traffic network with a single source and single destination. These are connected with each other through \(\numLinks\) parallel links\footnote{We fix an enumeration of routes to be used as reference throughout the article, $i = \{1, \dots, R\}$}. The total demand that needs to be routed through the network is \(\demand\in \R\). Let \(\flowLink\in\R^{\numLinks}\) be the flow profile on the network such that \(\flowLink_i\) denotes
the flow on link \(i\in[\numLinks]\).

The congestion cost on a link \(i\in[\numLinks]\) with flow \(\flowLink_i\) is denoted by \(\costLink_i(\flowLink_i)\). Above is the situation.


For ease of exposition, we further define \(\costLink(\flowLink)\defas (\costLink_1(\flowLink_1),\dots,\costLink_\numLinks(\flowLink_\numLinks)) \in \R^{\numLinks} \). The aforementioned routing game setup will be concisely represented as \((\numLinks,\demand,\costLink)\) going forward.  

\begin{assumption}
The functions $C_i(\cdot)$ are increasing and convex. 
\end{assumption}
\begin{definition}
A flow \(x\in\R^{\numLinks}\) is called \emph{feasible} if 
\[
\sum_{i\in[\numLinks]} \flowLink_i = \demand.
\]
We denote the set of feasible flows by \(\feasibleFlow\).
\end{definition} 
\begin{definition}[Wardrop equilibrium]
A feasible flow profile \(\flowLink\in\R^\numLinks\) is a \emph{Wardrop equilibrium} of $(\numLinks,\demand,\costLink)$ if for any \(i\in[\numLinks]\) such that \(\flowLink_i>0\) we have 
\[
\costLink_i(\flowLink_i) \leq \costLink_j(\flowLink_j) \quad \forall \ i\neq j 
\].
\end{definition}

\begin{definition}[Stochastic user equilibrium \cite{cominetti2012modern}]
A feasible flow profile \(\flowLink\in\R^{\numLinks}\) is a \emph{stochastic user equilibrium} of \((\numLinks,\demand,\costLink)\) if the flow on route \(i\) satisfies 
\[
\flowLink_i = \demand\Pr[\costLink_i(x_i)+\noise_i \leq \min_{j\in [\numLinks]}\costLink_j(x_j)+\noise_j] \quad \forall \ i,
\]
where \(\{\noise_i\}_{i\in [R]}\) are zero mean random variables. 
\end{definition}

Further, there is an equivalent convex optimization problem that characterizes the stochastic user equilibrium
\begin{theorem}[\cite{cominetti2012modern}]\label{thm: EqOptProb} An equivalent convex optimization based characterization of Wardrop and stochastic user equilibrium:
\begin{enumerate}
    \item A flow profile \(\flowLink\in\R^{\numLinks}\) is a Wardrop equilibrium \emph{if and only if} it solves the following optimization problem:
    \begin{align*}
    \min_{\flowLink\in\feasibleFlow} \sum_{i\in\numLinks} \int_{0}^{\flowLink_i} \costLink_i(z) \dd z
    \end{align*}
    
    \item A flow profile \(\flowLink\in\R^{\numLinks}\), with \(\{\noise_i\}_{i\in[\numLinks]}\) a zero-mean \(\gumbel(\beta)\) distribution\footnote{Write about Gumbel dist} for some \(\beta>0\), is a stochastic user equilibrium \emph{if and only if} it solves the following optimization problem:
\begin{align*}
    \min_{\flowLink\in F} \sum_{i\in[\numLinks]}\int_{0}^{x_i} \costLink_i(z)\dd z + \frac{1}{\beta} \sum_{i\in[\numLinks]} \flowLink_i \ln{\flowLink_i}.
\end{align*}
\end{enumerate}
\end{theorem}

\begin{corollary}
[\cite{cominetti2012modern}]\label{thm: UniqueSUE} By the strict convexity of the optimization problem (2) in \ref{thm: EqOptProb} there exists a unique stochastic user equilibrium for every \((\numLinks,\demand,\costLink)\).
\end{corollary}
\begin{remark}
An immediate conclusion from the optimization problems presented in Theorem \ref{thm: EqOptProb} is that if \(\beta\rightarrow +\infty\) then stochastic user equilibrium and Wardrop equilibrium coincide. 
\end{remark}

\subsection{Socially Optimal Routing}
We now give a summary of behavior that a central planner would like to induce for the routing game. 

\begin{definition}\label{thm: SocialCost}
The function 
\[
\socialCost(\flowLink) \defas \sum_{i=1}^{\numLinks} \flowLink_i \costLink_i(\flowLink_i).
\]
is called the \emph{social cost function} (SCF) and its minimizer over the feasible set \(\feasibleFlow\), \(\minSocial\), is called the \emph{socially optimal flow}. 
\end{definition}

\begin{definition}
Let \(\marginalCost(x)\) denote the \emph{marginal cost function} (MCF) corresponding to $C$ defined as \[
\marginalCost_i(\flowLink_i) \defas \marginalCost_i(\flowLink_i) + \flowLink_i\grad_x \costLink_i(\flowLink_i)
\]

\end{definition} 
% \begin{definition}
% We define the \textbf{social cost function} 
% \begin{align}
    
% \end{align}
% and we call any feasible flow that minimizes the social cost function an \textbf{optimal flow}.
% \end{definition}

% \begin{definition}
% We define the \textbf{marginal cost function}
% \begin{align}
%     \tilde{C}_i(x_i) = C_i(x_i) + x_i C_i'(x_i)
% \end{align}
% \end{definition}

Given these definitions, we have the following proposition from \cite{roughgarden2010algorithmic}.

\begin{proposition}
[\cite{roughgarden2010algorithmic}] A feasible flow $x \in \feasibleFlow$ is a minimizer of the social cost function for $(\numLinks,\demand,\costLink)$ \emph{if and only if} it is a Wardrop equilibrium for $(\numLinks,\demand, \marginalCost)$, where $\marginalCost$ is the marginal cost function corresponding to $\costLink$.
\end{proposition} 

\subsection{Stochastic Approximation}
In this section we shall recall some of the relevant results from stochastic approximation \cite{borkar2009stochastic}. 

Consider a \(d-\) dimensional stochastic process defined as 
\begin{align}\label{eq: StochasticProcess}
X(n+1) = X(n)+ a\ls{h(X(n)) + M(n+1)}, \quad n \geq 0
\end{align}
where \(h:\R^d \ra \R^d\), \(\{a > 0\}\) is the step sizes and \(\{M(n):n\in \N\}\) is uncorrelated and zero mean. Let \(\mc{F}_n \defas \sigma(X(i),M(i),i\leq n)\). 

\begin{assumption}\label{assm: SA Assumption}
We impose the following assumptions on the stochastic process mentioned in \eqref{eq: StochasticProcess}:
\begin{enumerate}[leftmargin = *]
    \item The function \(h\) is Lipschitz continuous and  there exists function \(h_{\infty}:\R^d\ra\R^d\) defined as 
    \[
    h_\infty(x) \defas \lim_{s\ra\infty} \frac{h(sx)}{s}, \quad \forall x\in \R^d 
    \]
    such that origin is an asymptotically stable equilibrium of the ode \(\dot{x}(t) = h_\infty(x(t))\). 
    \item Let \(\{M(n)\}_{n\in\N}\) be \(\mc{F}_n-\)adapted martingale difference sequence. Furthermore, for some \(C_0 < \infty\) and any initial state \(X(0)\) we posit 
    \[
    \avg[\|M(n+1)\|^2|\mc{F}_n] \leq C_0 \lr{1+\|X(n)\|^2}, \quad n \in \N.
    \]
\end{enumerate}
\end{assumption}

Under the above set of assumptions, one can ensure that the mean squared iterate will be bounded. That is, 
\begin{theorem}
Under the Assumption \ref{assm: SA Assumption}, there exists \(a^\star\) such that for all \(0<a<a^\star\) and \(X(0)\in \R^d\) we have \[
\limsup_{n\ra \infty} \avg[\|X(n)\|^2] \leq C_1
\]
\end{theorem}

==> Dynamic_Routing_Regular (Arxiv)/Proof.tex <==
% \section{Proof of Proposition \ref{prop: xEqExist}}\label{proof: Prop31}

% \section{Proof of Lemma \ref{lem: MonotonicityFlow}}\label{proof: lemMonotonic}
% Recall from the proof of Proposition \ref{prop: xEqExist} (\ref{thm: claim2} to be precise) that for any \(p\in\R^{\numLinks}\), \(\fixedPointFlow(p)\) is a solution to the optimization problem \eqref{eq: OptimizationProblem}. Let the feasible region in the optimization problem \eqref{eq: OptimizationProblem} be denoted by \(F\). Using first order conditions for constrained optimization we obtain the variational inequality: 
% \begin{align}\label{eq: ConstrainedOptimalityP}
%     \sum_{r\in[\numLinks]} \lr{\costPrice_r\lr{\fixedPointFlow_r(p),p} + \frac{1}{\beta}\lr{\ln\lr{\fixedPointFlow_r(p)}+1}}\lr{x_r-\fixedPointFlow_r(p)} \geq0 \quad \forall x \in F.
% \end{align}
% Similarly writing the above condition for \(p'\), we obtain \begin{align}\label{eq: ConstrainedOptimalityPD}
%     \sum_{r\in[\numLinks]} \lr{\costPrice_r\lr{\fixedPointFlow_r(p'),p'} + \frac{1}{\beta}\lr{\ln\lr{\fixedPointFlow_r(p')}+1}}\lr{y_r-\fixedPointFlow_r(p')} \geq0 \quad \forall y \in F.
% \end{align}
% Choosing \(x=\fixedPointFlow(p')\)  in \eqref{eq: ConstrainedOptimalityP} and \(y=\fixedPointFlow(p)\) in \eqref{eq: ConstrainedOptimalityPD} and adding the two equations we obtain
% \begin{align*}
%     &\sum_{r\in[\numLinks]} \lr{ \costPrice_r(\fixedPointFlow_r(p),p)-\costPrice_r(\fixedPointFlow_r(p'),p')}\lr{\fixedPointFlow_r(p')-\fixedPointFlow_r(p)} \\ &\quad \quad +\sum_{r\in[\numLinks]} \lr{ \frac{1}{\beta} \ln(\fixedPointFlow_r(p))-\ln(\fixedPointFlow_r(p')) }\lr{\fixedPointFlow_r(p')-\fixedPointFlow_r(p)} \geq 0.
% \end{align*}
% From the fact that prices enter additively, we have 
% \begin{align*}
%     &\sum_{r\in[\numLinks]} \lr{ \costEdge_r(\fixedPointFlow_r(p))-\costEdge_r(\fixedPointFlow_r(p'))}\lr{\fixedPointFlow_r(p')-\fixedPointFlow_r(p)}\\ &\quad\quad + \sum_{r\in[\numLinks]} \lr{ p_r-p_r'+ \frac{1}{\beta} \ln(\fixedPointFlow_r(p))-\ln(\fixedPointFlow_r(p')) }\lr{\fixedPointFlow_r(p')-\fixedPointFlow_r(p)} \geq 0.
% \end{align*}
% This gives 
% \begin{align*}
%     &\lara{\fixedPointFlow(p)-\fixedPointFlow(p'),p-p'} \\&\leq \lara{\costEdge(\fixedPointFlow(p))-\costEdge(\fixedPointFlow(p')),\fixedPointFlow(p')-\fixedPointFlow(p)}\\&\quad +\frac{1}{\beta} \lara{ \ln(\fixedPointFlow(p)) - \ln(\fixedPointFlow(p')), \fixedPointFlow(p')-\fixedPointFlow(p)}\\
% &< 0,
% \end{align*}
% where the last inequality follows due to the monotonicity of the cost function and natural logarithm.

% The claim that \(\frac{\partial \fixedPointFlow_i(\priceContinuous)}{\partial \priceContinuous_i} < 0\) also follows from the monotonicity of \(\fixedPointFlow(\priceContinuous)\). Indeed, if we choose two price profiles that differ only at one index then the monotonicity property of \(\fixedPointFlow(p)\) ensures \(\fixedPointFlow(\priceContinuous)\). 
% This completes the proof. 

% \section{Proof of Proposition \ref{prop: ConnectionToWardrop}}\label{proof: PropWardrop}
% \begin{proof}
% Let's denote the flow under static Wardrop equilibrium and price \(p\) by \(\flowWardrop(p)\). The proof follows by observing that for any \(p\in\R^{\numLinks}\) and \(\beta>0\), \(\fixedPointFlow(p)\) is the unique solution to the convex optimization problem \eqref{eq: OptimizationProblem} as is presented in Proposition \ref{prop: xEqExist}. In the optimization problem \eqref{eq: OptimizationProblem} as \(\beta\uparrow +\infty\) the effect of entropy regularization diminishes and the resulting optimization program is the one that characterizes Wardrop equilibrium \cite[p. 214]{cominetti2012modern}. That is \(\fixedPointFlow(\cdot) \ra \flowWardrop(\cdot)\) as \(\beta\uparrow+\infty\) in a pointwise sense.  



% For the purpose of this proof, we shall introduce the notation \(\fixedPointPrice^{(\beta)}\) to the solution of \eqref{eq: pEquilibrium}. That is, for any \(i\in[\numLinks]\)
% \begin{align}\label{eq: PriceBeta}
%     \fixedPointPrice_i^{(\beta)} = \fixedPointFlow_i(\fixedPointPrice^{(\beta)}) \grad_x \costEdge_i(\fixedPointFlow_i(\fixedPointPrice^{(\beta)}))
% \end{align}

% Let 
% \begin{align*}
%   x^\star = \argmin_{y\in F} \lr{ \sum_{i\in[\numLinks]} y_i\costEdge_i(y_i) + \frac{1}{\beta}\sum_{i\in[\numLinks]} y_i\log(y_i)},
% \end{align*}
% where \(F= \{y: \sum_{i\in[\numLinks]}y_i = \frac{\meanInflow}{\meanOutflow}\}\) is the feasible set. We claim that \(x^\star =  \fixedPointFlow(\fixedPointPrice^{(\beta)})\).

% To show this claim, we first note that the above problem is a strictly convex optimization problem. The necessary and sufficient conditions for constrained optimality ensures that for any \(y\in F\): 
% \begin{align}\label{eq: SocialCostFirst}
%     \sum_{i\in[\numLinks]} \lr{ \costEdge_i(x^\star_i) + x_i^\star\grad_x\costEdge_i(x_i^\star) + \frac{1}{\beta} \lr{1+\log(x_i^\star)}}\lr{ y_i-x_i^\star} \geq 0. 
% \end{align}

% Now recall that \(\fixedPointFlow(\fixedPointPrice^{(\beta)})\) satisfies 
% \begin{align*}
%     \fixedPointFlow(\fixedPointPrice^{(\beta)}) = \argmin_{y\in F} \sum_{i\in[\numLinks]} \int_{0}^{y_i}\lr{\costEdge_i(z)+\fixedPointPrice^{(\beta)}_i } \textsf{d}z+\frac{1}{\beta}\sum_{i\in[\numLinks]} y_i\log(y_i).
% \end{align*}
% Note that we have already mentioned in proof of Proposition \ref{prop: xEqExist} that the above optimization problem is strictly convex. The constraint optimality conditions ensures that for any \(y\in F\):
% \begin{align}\label{eq: SelfishCostFirst}
%     \sum_{i\in[\numLinks]}\lr{\costEdge_i(\fixedPointFlow_i(\fixedPointPrice^{(\beta)})) + \fixedPointPrice_i^{(\beta)} + \frac{1}{\beta} \lr{1+\log(\fixedPointFlow_i(\fixedPointPrice^{(\beta)}))}}\lr{y_i-\fixedPointFlow_i(\fixedPointPrice^{(\beta)})} \geq 0. 
% \end{align}
% Note that using \eqref{eq: PriceBeta} in \eqref{eq: SelfishCostFirst} we obtain that for any \(y\in F\): 
% \begin{align}\label{eq: SocialCostSecond}
%     \sum_{i\in[\numLinks]}\lr{\costEdge_i(\bar{x}) + \bar{x}_i \grad_x \costEdge_i(\bar{x}_i) + \frac{1}{\beta} \lr{1+\log(\bar{x}_i)}}\lr{y_i-\bar{x}_i} \geq 0, 
% \end{align}
% where we have used \(\bar{x} = \fixedPointFlow(\fixedPointPrice^{(\beta)})\) to simplify expression. Comparing expression \eqref{eq: SocialCostFirst} and \eqref{eq: SocialCostSecond} we conclude that \(x^\star =\fixedPointFlow(\fixedPointPrice^{(\beta)}) \). 

% % {
% % \color{red}
% % From Theorem 18.27 of \cite{roughgarden2010algorithmic}, we recall that the optimal flows to the problem:
% % \begin{align}
% %     x^{\star} = \arg \min_{x: \sum_{i=1}^{R} x_i = \frac{\meanInflow}{\meanOutflow}} S(x) = \arg \min_{x: \sum_{i=1}^{R} x_i = \frac{\meanInflow}{\meanOutflow}} \sum_{i=1}^{R} x_i c_i(x)
% % \end{align}
% % the equilibrium flows to the static routing problem $(G, \frac{\meanInflow}{\meanOutflow}, c_i+ \fixedPointFlow(\fixedPointPrice) \nabla_x c_r(\fixedPointFlow(\fixedPointPrice))$.

% % Let's denote the Wardrop flow at price \(p\), by 
% % \[
% % \bar{x}^W_i(p) = \lim_{\beta \ra \infty} \fixedPointFlow(p)
% % \]
% % We know that the above quantity exists and is unique. The price at Wardrop equilibrium should satisfy 
% % \[
% % \bar{p}^W_i = \bar{x}^W_i(\bar{p}^W_i)\grad_x\costEdge_i(\bar{x}^W_i(\bar{p}^W_i))
% % \]

% % We know that for any fixed \(\beta\) the following equation has unique solution
% % \[
% % \bar{p}_i^{(\beta)} = \fixedPointFlow(\bar{p}_i^{(\beta)})\grad_x \costEdge_i(\fixedPointFlow(\bar{p}_i^{(\beta)}))
% % \]

% % The price should satisfy 
% % \begin{align*}
% %     \bar{p}^\infty_i = \lim_{\beta \ra \infty} \fixedPointFlow_i(\fixedPointPrice^\infty) \grad_x\costEdge_i()
% % \end{align*}
% % }

% \end{proof}

==> Dynamic_Routing_Regular (Arxiv)/conclusion.tex <==
\section{Conclusions and Future Work}\label{sec: Conclusion}
We propose a two timescale discrete-time stochastic dynamics that captures the joint evolution of loads in parallel network and adaptive adjustment of tolls. We analyze the properties of fixed points and the convergence of loads and tolls in this dynamics. We find that under our dynamics, the tolls eventually induce a socially optimal load with high probability. Our results allow a central authority to set tolls in networks \textit{adaptively} and \emph{optimally} in response to the dynamic arrival of travelers who myopically make routing decisions. 

One future direction of interest is to extend our results on parallel networks to general networks. The challenge of setting tolls on general networks is to account for the fact that travelers may change their route choices at intermediate nodes of the network due to the change of loads on links during their trips. Therefore, the toll updates need to account for the myopic route choice of incoming travelers as well as the change of routing decisions for travelers in the network. 

Another extension of this work is to design toll pricing that only set tolls on a subset of links instead of the entire network. This extension is of practical importance since setting high tolls on many links is difficult in implementation, and is not socially desirable. 

==> Dynamic_Routing_Regular (Arxiv)/experiments.tex <==
\section{Numerical Experiments}\label{sec: NumExp}
In this section we present an extensive numerical study of the results presented in \S\ref{sec: Results}. 
Specifically, 
\begin{enumerate}[align=left,leftmargin=*]
    \item we compare the evolution of the stochastic process \eqref{eq: CombinedDT} and the continuous time dynamical system \eqref{eq: singularPerturbedODE} under different parameter settings when toll pricing is implemented;
    \item we compare the evolution of stochastic process \eqref{eq: CombinedDT} with the socially optimal flow when \(a=0\) (i.e. no toll pricing). 
\end{enumerate}

In all the experiments, we set $\beta = 100$ which ensures that we are reasonably close to Wardrop equilibrium (ref Proposition \ref{prop: ConnectionToWardrop}). Furthermore, we set the edge cost function to take the following form: 
\begin{align}
    \costEdge_i(x) = i x^2 + i, \quad \quad i \in [\numLinks].
\end{align}
We implement the stochastic process for \(N=2000\) iterations. In order to plot the continuous time dynamical system and stochastic process we identify \(n\) iterations of stochastic process with \(n\meanOutflow\) units of flow of the continuous time dynamical system.  

We conduct the experiments in the following eight settings of parameters: 
\begin{enumerate}[label = (\textsf{S}-\Roman*), widest=viii, align=left, leftmargin=*]
    \item \label{enum: Setting1} $\numLinks = 3$,  $\meanInflow= 0.1$, $\meanOutflow = 0.1$ and \(a=0.0015\);
    \item \label{enum: Setting2}$\numLinks = 3$, $\meanInflow= 0.1$, $\meanOutflow = 0.05$ and \(a=0.0015\);
    \item \label{enum: Setting3} $\numLinks = 3$,  $\meanInflow= 0.1$, $\meanOutflow = 0.1$ and \(a=0\);
    \item \label{enum: Setting4}$\numLinks = 3$, $\meanInflow= 0.1$, $\meanOutflow = 0.05$ and \(a=0\);
    \item \label{enum: Setting5} $\numLinks = 6$,  $\meanInflow= 0.1$, $\meanOutflow = 0.05$ and \(a=0.0015\);
    \item \label{enum: Setting6} $\numLinks = 6$, $\meanInflow= 0.18$, $\meanOutflow = 0.05$ and \(a=0.0015\);
    \item \label{enum: Setting7} $\numLinks = 6$,  $\meanInflow= 0.1$, $\meanOutflow = 0.05$ and \(a=0\);
    \item \label{enum: Setting8} $\numLinks = 6$, $\meanInflow= 0.18$, $\meanOutflow = 0.05$ and \(a=0\).
\end{enumerate}

We now present the main observations from the numerical study.
In Fig. \ref{fig:3LinkSetting}, Fig. \ref{fig:6LinkSetting1} we observe that introducing the tolling dynamics allows the flow to converge to a neighborhood of the socially optimal flow. Note that socially optimal flow and price are the ones obtained by asymptotic limit of the continuous time dynamical systems \eqref{eq: singularPerturbedODE} (represented by solid lines in the plots).

 Note that the difference between setting \ref{enum: Setting1} and \ref{enum: Setting2} is different values of mean outflow \(\meanOutflow\). This naturally changes the ratio of mean inflow to mean outflow. This ratio, \(\meanInflow/\meanOutflow\), is the {equivalent demand} in the asymptotic limit (as stated in Proposition \ref{prop: xEqExist}) and the equilibrium flow is the flow obtained by performing static one shot routing using this equivalent demand. The significance of this equivalent demand is illustrated in 
     Fig. \ref{fig:3LinkFlowProfileL1} and Fig. \ref{fig:3LinkFlowProfileL2}. Observe that increasing this equivalent demand fills up the blue link (in Fig. \ref{fig:3LinkFlowProfileL2}) which was un-utilized in Fig. \ref{fig:3LinkFlowProfileL1}. 
     
    The settings \ref{enum: Setting5} and \ref{enum: Setting6} are also designed to capture the effect of variable equivalent demand on bigger network.  Interestingly, between these settings we have kept the mean outflow constant but changed mean inflow. This will naturally also change the equivalent demand, whose effect is seen in Fig. \ref{fig:6LinkFlowProfileL1} and Fig. \ref{fig:6LinkFlowProfileL2}. As we increase the equivalent demand the black and magenta link in Fig. \ref{fig:6LinkFlowProfileL2} starts filling up. These were un-utilized in Fig. \ref{fig:6LinkFlowProfileL1}. The effect of increasing the number of links is that some of the links may remain unfilled for quite a long time before starting to fill up (compare Fig.\ref{fig:3LinkFlowProfileL1}-Fig.\ref{fig:3LinkFlowProfileL2} 
     with 
     Fig.\ref{fig:6LinkFlowProfileL1}-Fig.\ref{fig:6LinkFlowProfileL2}
     ). 
     
     Next, we compare the changes in flow evolution when tolling is inactive (i.e. \(a=0\)). For the case of three link network, in Fig. \ref{fig:3LinkFlowPriceProfileL1NoToll} and Fig.\ref{fig:3LinkPriceProfileL2NoToll} we represent the socially optimal flow by dashed lines while flow obtained by stochastic rule \eqref{eq: CombinedDT} by solid lines. The flow allocation is inefficient in such settings. Low cost links are disproportionately over-utilized. Furthermore increasing the equivalent demand exacerbates the situation (compare Fig.\ref{fig:3LinkFlowPriceProfileL1NoToll} and Fig.\ref{fig:3LinkPriceProfileL2NoToll}). Similarly, when the number of links are increased a lot many links remain un-utilized when tolling is absent (refer Fig.\ref{fig:6LinkPriceProfileL1NoToll}-Fig.\ref{fig:6LinkPriceProfileL2NoToll}).


It is also interesting to mention the transient behavior observed when tolling is active (i.e. \(a>0\)). Since the pricing dynamics is slowly updated, during the initial phase of trajectory the flow evolution takes place as if there is no tolling and tries to reach near Wardrop equilibrium. But this phase does not last very long and the pricing dynamics diverts flow from the overutilized links to underutilized links. This effect is very distincly visible, for instance, in Fig.\ref{fig:6LinkFlowProfileL2}. The green link tries to reach its Wardrop point (similar to Fig. \ref{fig:6LinkPriceProfileL2NoToll}) but the pricing dynamics suppress this grown and diverts the flow to magenta and black link.

Note that it takes longer for the price trajectories (refer Fig. \ref{fig:3LinkPriceProfileL1},Fig.\ref{fig:3LinkPriceProfileL2}, Fig.\ref{fig:6LinkPriceProfileL1}, Fig.\ref{fig:6LinkPriceProfileL2}) to converge to their equilibrium as  compared to the flow trajectories. This is attributed to their evolution on slower time scale (recall \(a<<\mu\)).
\input{FigPlots}


==> Dynamic_Routing_Regular (Arxiv)/experiments_arxiv.tex <==
\section{Numerical Experiments}\label{sec: NumExp}

In this section we present numerical experiments for the results presented in \S\ref{sec: Results}. %Broadly speaking, we study the effect of tolls on the emergent load on the links. Furthermore, we evaluate how incoming loads, discharging loads, and the step size of the toll update affect the emergent load behavior.  
We observe that loads and tolls concentrate on a neighborhood of the socially optimal loads and tolls, and the continuous-time dynamical system \eqref{eq: singularPerturbedODE} closely approximates the discrete-time stochastic updates \eqref{eq: FlowDynamics} -- \eqref{eq: PricingDynamics}. Our numerical results are consistent with Theorems \ref{theorem: fixed_point}  and \ref{theorem:discrete_convergence}. %the theory of two-timescale stochastic approximation as applied to the load and price stochastic updates.

% Furthermore, when tolls are active ($a > 0$) the trajectories of continuous-time dynamical system \eqref{eq: singularPerturbedODE} (and consequently the discrete-time stochastic update \eqref{eq: CombinedDT}) converge to socially optimal load and toll-prices. Meanwhile, when tolls are inactive ($a = 0$), we observe that some links are underutilized while the others are relatively congested. By incorporating the proposed tolling update the disproportionate use of network resources is minimized. 

% More formally,  
% \begin{enumerate}
% %[align=left,leftmargin=*]
%     \item we compare the evolution of the stochastic process \eqref{eq: CombinedDT} and the continuous-time dynamical system \eqref{eq: singularPerturbedODE} under different parameter settings when toll pricing is implemented;
%     \item we compare the evolution of the discrete-time update \eqref{eq: CombinedDT} with the socially optimal flow when \(a=0\) (i.e. no toll pricing). 
% \end{enumerate}

Consider a network with six parallel links (i.e. $R=6$) with the following link latency functions: 
\begin{align}
    \costEdge_i(x) = i x^2 + i, \quad \quad \forall \ i \in [\numLinks].
\end{align}

%In order to plot the continuous-time dynamical system and discrete-time stochastic update on same timescale, we identify \(n\) steps of the update with \(n\meanOutflow\) units of flow of the continuous-time dynamical system.  
We set the total time steps of discrete-time stochastic update as $N=2000$, and the dispersion parameter $\beta = 100$. We conduct the four sets of experiments with the following parameters: 
% \begin{enumerate}%[label = (\textsf{S}-\Roman*), widest=viii, align=left, leftmargin=*]
    % \item \label{enum: Setting1} $\numLinks = 3$,  $\meanInflow= 0.1$, $\meanOutflow = 0.1$ and \(a=0.0015\);
    % \item \label{enum: Setting2}$\numLinks = 3$, $\meanInflow= 0.1$, $\meanOutflow = 0.05$ and \(a=0.0015\);
    % \item \label{enum: Setting3} $\numLinks = 3$,  $\meanInflow= 0.1$, $\meanOutflow = 0.1$ and \(a=0\);
    % \item \label{enum: Setting4}$\numLinks = 3$, $\meanInflow= 0.1$, $\meanOutflow = 0.05$ and \(a=0\);
    
    (\textbf{S1}) $\meanInflow= 0.1$, $\meanOutflow = 0.05$ and \(a=0.0015\);
    
    (\textbf{S2}) $\meanInflow= 0.2$, $\meanOutflow = 0.05$ and \(a=0.0015\);
    
    (\textbf{S3})  $\meanInflow= 0.1$, $\meanOutflow = 0.05$ and \(a=0\);
    
    (\textbf{S4}) $\meanInflow= 0.2$, $\meanOutflow = 0.05$ and \(a=0\).

We note that tolls are updated with positive stepsizes in (\textbf{S1}) -- (\textbf{S2}), but remain zero in (\textbf{S3}) -- (\textbf{S4}). Also, the mean incoming load of travelers in each step $\meanInflow$ is high in (\textbf{S1}) and (\textbf{S3}), and low in (\textbf{S2}) -- (\textbf{S4}). In Fig. \ref{fig:6LinkSetting1}, we demonstrate the loads and tolls obtained in the discrete-time stochastic updates \eqref{eq: FlowDynamics} -- \eqref{eq: PricingDynamics} (represented by dots), and those induced by the continuous-time dynamical system \eqref{eq: singularPerturbedODE} (represented by solid lines) in (\textbf{S1}) and (\textbf{S2}), respectively. In Fig. \ref{fig:6LinkNoPrice}, we demonstrate the loads in the discrete-time updates and the socially optimal load for (\textbf{S3}) and (\textbf{S4}). We omit the figures for tolls since tolls are not updated with step size $a=0$. 


We now present the main observations from the numerical study.
Firstly, we observe that in Fig. \ref{fig:6LinkSetting1}, the trajectories of continuous-time dynamical system \eqref{eq: singularPerturbedODE} closely track the discrete-time stochastic load update. Moreover, we observe that it takes more time steps for the tolls (refer Fig.\ref{fig:6LinkPriceProfileL1}, Fig.\ref{fig:6LinkPriceProfileL2}) to converge compared to the loads. This is because tolls are updated at a slower timescale (i.e. \(a\ll\mu\)). 
% Moreover, as in the asymptotic limit the trajectories continuous-time dynamical system \eqref{eq: singularPerturbedODE} converge to socially (represented by solid lines in the plots). This therefore validates that the discrete-time stochastic update asymptotically tracks the continuous-time dynamical system. 

Secondly, we show that the repeatedly updated tolls eventually induce the perturbed socially optimal load in Fig. \ref{fig:6LinkFlowProfileL1} and \ref{fig:6LinkFlowProfileL2}. On the other hand, when tolls are zero (i.e. inactive) in all steps, loads converge to a stochastic user equilibrium (Fig. \ref{fig:6LinkPriceProfileL1NoToll} and \ref{fig:6LinkPriceProfileL2NoToll}), which is different from the socially optimal load. This means that links are inefficiently utilized when tolls are inactive. We observe that the low cost links (links 1, 2, and 3) are disproportionately over-utilized while the remaining links are underused especially in the setting with high incoming load $\lambda$ (Fig.\ref{fig:6LinkPriceProfileL2NoToll}).  %compare the changes in load evolution when tolls are inactive (i.e. \(a=0\)). Note that in setting (\textbf{S3}), (\textbf{S4}) the load at the stochastic user equilibrium is obtained by performing static one-shot routing with equivalent demand \(\frac{\meanInflow}{\meanOutflow}\).      In Fig. \ref{fig:6LinkNoPrice} we represent the socially optimal loads by dashed lines while load obtained from the stochastic discrete-time update \eqref{eq: CombinedDT} is represented by solid lines. We observe that the 
     
     
 Thirdly, we note that both the perturbed socially optimal load and the stochastic user equilibrium change with the average incoming load $\lambda$. In particular, more links are utilized at fixed point with high $\lambda$ (Fig. \ref{fig:6LinkFlowProfileL2} for \textbf{(S2)} and Fig. \ref{fig:6LinkPriceProfileL2NoToll} for \textbf{(S4)}) compared to that with low $\lambda$ (Fig. \ref{fig:6LinkFlowProfileL1} for \textbf{(S2)} and Fig. \ref{fig:6LinkPriceProfileL1NoToll} for \textbf{(S4)}).
 
 %Notice that the difference between setting (\textbf{S1}) and (\textbf{S2}) (and correspondingly in setting (\textbf{S3}) and (\textbf{S4})) is different values of the {equivalent demand} \(\frac{\meanInflow}{\meanOutflow}\).  The effect of altering equivalent demand is illustrated . Observe that increasing the equivalent demand causes the black and magenta links in Fig. \ref{fig:6LinkFlowProfileL2} to fill up which remain relatively un-utilized in Fig. \ref{fig:6LinkFlowProfileL1}.
     
%Finally, we notice when tolling is active (i.e. \(a>0\)). During the initial phase of routing, since the tolling update is on a slower timescale than the load, the load evolution takes place as if there is no tolling and tries to reach near Wardrop equilibrium. But this phase does not last very long and the tolling updates divert the load from the over-utilized links to underutilized links. This effect is visible in Fig.\ref{fig:6LinkFlowProfileL2}. The green link tries to reach its Wardrop point (similar to Fig. \ref{fig:6LinkPriceProfileL2NoToll} where the tolling is inactive) but the tolling update suppresses this growth and diverts the load to the magenta and black link.
     
   





\input{FigPlots_arxiv}


==> Dynamic_Routing_Regular (Arxiv)/intro.tex <==
\section{Introduction}\label{sec: Intro}

% \begin{itemize}
%     \item 
%     \item 
%     \item We are proposing a new tolling mechanism that have two time scales -- one is ..., the other is ... why one is slower than the other
% \end{itemize}


% \tdBox{Main point to include in the intro
% 1. Brief account of real world cases where the congestion pricingi is implemented. Practical issues with this

% 2. Bringing out computationaly efficiency of scheme 


% }
%%%% Motivation of the problem

Efficient traffic routing is an increasingly important problem as congestion aggravates on urban transportation networks. Many cities around the world have implemented congestion pricing (tolling) to regulate the demand of travelers (\cite{latimes2021,nyt2021}). Tolling, when properly set in response to real-time traffic conditions, can effectively alleviate congestion and even induce socially optimal loads \cite{sharon2017real, paccagnan2019incentivizing}. 

One challenge of setting tolls is that travelers continuously arrive at and depart from the network, which creates a dynamic involvement of traffic loads in the network. Additionally, travelers are selfish in that they prefer to choose the routes with the minimum cost - travel time cost and the tolls combined. A dynamic tolling mechanism that induces efficient traffic load must account for the dynamic nature of traffic demand and the selfish nature of individuals' routing decisions. In particular, the mechanism must enable the tolls to \textit{adaptively} change in response to changing traffic conditions. 


%In real world traffic networks, users arrive dynamically and make routing decisions based on the existing congestion of the network, and the natural equilibria in routing games (Wardrop, stochastic user (\cite{cominetti2012modern}), etc.) are inefficient in the sense that they are not minimizers of the social cost function \cite{roughgarden2002bad}. how should we set tolls dynamically such that the joint evolution of the load and price converges to social optimality? 

% Para 1 on modeling 
We propose a discrete-time stochastic dynamics to capture the joint evolution of the loads and tolls in a parallel-route network. In each time step of the dynamics, non-atomic travelers arrive at the origin of the network, and they make routing decisions according to a perturbed best response based on the travel time cost and toll of each route in that step. Additionally, a fraction of load on each route is discharged from the network. Both the incoming and outgoing demand are randomly realized from an identical and independent distribution. Therefore, the sequence of link loads forms a Markov process, and the discrete-time stochastic dynamics of loads is governed by the total arriving demand, the stochastic user equilibrium, and the load discharge rate. Furthermore, in each time step, a traffic authority adjusts the toll on each route by interpolating between the current toll and a new increment dependent on the marginal cost of travel time given the load in that step. 

We assume that the dynamics of the toll evolves at a slower time-scale compared to that of the load dynamics. This assumption avoids the situation that tolls change during the trip of individual travelers, which is undesirable in practice (\cite{farokhi2015piecewise}). Therefore, travelers view the tolls as static when they make routing decisions at the arrival. %Therefore, price does not change during their trip. That is, when travelers make routing decisions at , extending the extensive literature on tolling in static routing (\cite{brown2016robustness}, \cite{yang1998principle}, \cite{yang2004trial}). 

%This model builds upon existing work in dynamic traffic routing in two main ways: 1) We incorporate a ``two-timescale'' toll update, in which tolls evolve slowly as compared to the loads, and 2) our model allows for stochasticity in the incoming demand and outgoing loads.
%, and therefore, we are able to analyze the dynamics as a random process. 

% Para 1 of Results: Convergence results

 


We show that the loads and tolls in the discrete-time stochastic dynamics asymptotically concentrate in a neighborhood of a unique fixed point with high probability. The fixed point load is \emph{socially optimal} in that it minimizes the total travel time costs on all routes in the network when the total arriving and discharging traffic demand reach a \emph{steady state}, and the fixed point toll on each route equals to the marginal cost. That is, our dynamic tolling eventually induces the socially optimal loads that account for the incoming and discharging travelers and their selfish routing behavior. Furthermore, we emphasize that our dynamic tolling is \emph{distributed} in that the traffic authority only uses the information of the cost and load on each route to update its toll.  % (\cite{roughgarden2010algorithmic, farokhi2015piecewise}). The socially optimal load corresponds to the {\color{red}``steady-state''} equilibrium of our dynamics when the tolls are set at the socially optimal values. 

% Para 2 of Results: Link between the discrete time and continuous time 

Our technical approach to proving the main result involves: \emph{(i)} Constructing a continuous-time deterministic dynamical system associated with the two timescale discrete-time stochastic dynamics; \emph{(ii)} Demonstrating that the flow of the continuous-time dynamical system has a unique fixed point that corresponds to the socially optimal load and tolls; \emph{(iii)} Proving that the unique fixed point of the flow of the continuous time dynamics is globally stable. In particular, we apply the theory of two time-scale stochastic approximation to show that the loads and tolls under the stochastic dynamics concentrates with high probability in the neighborhood of the fixed point of the flow of continuous time dynamics constructed in \emph{(i)} (\cite{borkar2009stochastic}). Additionally, our proof in \emph{(ii)} on the uniqueness and optimality of fixed point of the flow of continuous time dynamics builds on a variational inequality, and extends the analysis of stochastic user equilibrium in static routing games to account for the steady state of the network given the arriving and discharging traffic (\cite{cominetti2012modern}). Furthermore, we show that the continuous time dynamical system is cooperative, and thus its flow must converge to its fixed point (\cite{hirsch1985systems}). 


%In order to prove the main result we consider an underlying continuous-time deterministic dynamical system that ``closely'' approximates the discrete-time stochastic dynamical system. Such a continuous-time dynamical system is obtained by leveraging the slower update of toll-price dynamics. This property is popularly referred as the ``two-timescale'' property \cite{borkar2009stochastic}.  We show that the continuous-time dynamical system admits unique fixed points that are the same as the socially optimal loads and tolls respectively.  Furthermore, we show that the trajectories of the continuous-time dynamical system in fact converge to the fixed points, which in turn ensures that the discrete-time dynamics concentrates in a neighborhood of socially optimal load with high probability.

% Para 3 of Results: Discuss the techniques
%We design the discrete-time dynamics such that the fixed point of the underlying continuous-time load dynamics, at any \emph{fixed} toll-price, is a game theoretically motivated quantity -- namely it is the ``steady-state'' stochastic user equilibrium at that toll under an \emph{equivalent demand} dependent on the inload and outload. One of our main technical results we establish that such fixed points are monotonic in toll-prices. Broadly speaking, this property ensures that increasing toll-prices on particular link reduces the load on that link.  The convergence of the underlying continuous-time dynamics is established by exploiting this monotonicity in conjunction with the results from \emph{cooperative dynamical systems theory} \cite{hirsch1985systems}. 

Our model and results contribute to the rich literature on designing tolling mechanisms for inducing socially optimal route loads. Classical literature on static routing games has focused on measuring the inefficiency of selfish routing by bounding the "price of anarchy", and designing marginal cost tolling to induce socially optimal route loads (\cite{christodoulou2005price, roughgarden2002bad, roughgarden2010algorithmic}). In static routing games, optimal tolling does not account for the dynamic arrival and departure of travelers. The computation of optimal tolls relies on knowledge of the entire network structure and the equilibrium route flows, which are challenging to compute. 

Dynamic toll pricing has been studied in a variety of settings to account for the continuous arrival and discharge of travelers in the network. The paper \cite{borkar2009cooperative} analyzed a discrete-time stochastic dynamics of the arrival and discharge of non-atomic travelers, and discussed the impact of tolling on routing strategies. We consider an adaptive adjustment of tolls using marginal toll pricing, and analyze the long-run outcomes of the joint evolution of the route loads and tolls. We prove that the tolls updated in our dynamics converge, and eventually induce a socially optimal traffic load associated with the steady state of the network. Additionally, we have removed the assumption in \cite{borkar2009cooperative} that the equilibrium routing strategy is monotonic in tolls. In fact, we \emph{prove} that the monotonicity condition is a feature of the equilibrium routing strategy. 

Moreover, \cite{como2021distributed} proposed a continuous-time dynamical system to study socially optimal tolling when strategic travelers continuously arrive and make selfish routing decisions. In their model, the arrival and discharged loads are balanced so that the aggregate load in the network is a constant. In our setting, both the total arrival load and discharged load are random variables. Therefore, our fixed point analysis needs to account for the total load at the steady state of the network. Moreover, \cite{como2021distributed} assumes that the tolls are adjusted at a faster time scale than their traveler's route preferences, while we assume that the update of tolls is at a slower timescale compared to the change of routing decisions.  

Finally, this article is also related to the literature on learning in routing games, and learning for tolling with unknown network condition. In particular, a variety of algorithms have been proposed to study how travelers learn an equilibrium by repeatedly adjusting their routing decisions based on the observed travel time in the network (e.g. \cite{cominetti2010payoff, krichene2014convergence, kleinberg2009multiplicative}). Additionally, papers \cite{farokhi2015piecewise, poveda2017class, meigs2017learning, wu2020bayesian} have analyzed how the traffic authority adaptively updates the tolls while learning the unknown network condition using crowd-sourced data on traffic load and time costs.




%We note that much of the literature on dynamics in traffic routing focuses on learning dynamics such as those found in \cite{krichene2014convergence}, or casts the problem of dynamic traffic routing as a repeated game \cite{la2002optimal}. This literature does not take into account the \textit{residual loads} and \textit{delays} that are present in real-world traffic networks.

%The works closest to ours in philosophy are \cite{borkar2009cooperative}, \cite{pietrabissa2018discrete}, and \cite{como2021distributed}. These build in a dynamic load adjustment at the network level scheme based on conservation laws whose steady states are Wardrop equilibria, and thus the strategic decisions made by loads are accounted for. However, \cite{borkar2009cooperative} and \cite{pietrabissa2018discrete} do not address the issue of dynamic pricing to social optima, and \cite{como2021distributed} addresses the question of fast-changing pricing (and correspondingly slow-changing preferences) for a large class of dynamic feedback control policies. In contrast we study \textit{slow-changing marginal cost tolls} which are more preferable to users \cite{farokhi2015piecewise}.

This article is organized as follows: we introduce the dynamic tolling model and the discrete time stochastic dynamics in Sec. \ref{sec: Model}. We present the main result in Sec. \ref{sec: Results}, and numerical examples in Sec. \ref{sec: NumExp}. We conclude our work in Sec. \ref{sec: Conclusion}. We only present the key ideas of our prove techniques in the Sec. \ref{sec: Results}, and include all proofs in Appendix \ref{appsec: ProofLemma}. 
%We also note that our scheme allows for computationally tractable marginal cost tolls, as the central authority can \textit{adaptively} compute the tolls based on only the available state information. This is in contrast with the literature on static traffic assignment and tolling, in which the authority would need to compute the traffic equilibrium (known to be computationally intractable problem \cite{papadimitriou2007complexity}) in order to impose tolls. 

%Dynamic traffic routing and tolling presents a novel problem as technologies like navigation apps have enabled flexible routing both spatially and temporally \cite{aswani2011game}. As road congestion worsens as a result of selfish game-theoretic behavior from traffic, it is important to study the effect of interventions like tolling on network state. 



\begin{comment}
{\color{red} Beyond this point it is yet to be updated}
In this article, we use techniques from \emph{cooperative} dynamical systems theory \cite{hirsch1985systems} and two-timescale stochastic approximation \cite{borkar2009stochastic} to prove the convergence of these stochastic dynamics to socially optimal tolls and loads. We show that the discrete-time dynamics asymptotically track a continuous time o.d.e., and that the o.d.e. converges to the socially optimal loads and tolls given a particular construction of the tolls that uses the \textit{marginal cost} incurred on each link. 
We prove a novel monotonicity result 

% \todo[inline]{Model description, comments, and discussion/techniques: Add our contributions here. Second paragraph should focus on model, begin paragraph with ``We propose a discrete time stochastic dynamics that addresses the joint evolution of load and tolls. The introduction should tell about the model. People arrive at origin and make decisions; tolls are set by central authority. Comment on dynamics of $x$ and $p$. End with question: how should we set tolls in this dynamics such that the dynamic converges to social optimality. We also need to justify two time-scale in the next paragraph.

% Also a paragraph to emphasize the novelty of the model.}
% \tdBox{Results around 3 paragraph: Dynamics converge to the socially optimal load. Find continuous dynamics approximating this dynamics. Find continuous dynamics is equilibirium}
% \tdBox{Comment about the techniques: Hirsch and monotonicity. DONT give sense that it is direct deployment. Point out game theoretic aspect. }
Correspondingly, time dynamical routing and its convergence to game theoretic equilibria has been studied in \cite{borkar2009cooperative}. This routing framework allows one to keep track of loads dynamically as they travel through a network, in contrast to the static or repeated routing schemes traditionally found in the literature.  

The challenge is that there is a need for a new mechanism to set tolls adaptively in response to the dynamically evolving traffic conditions, which are determined by the coming and going of traffic in the network and also by the \textit{selfish} routing decisions made by the travelers.
%This paper extends previous work by including a pricing dynamic that ensures link loads minimizes a utilitarian measure of social optimality. 
Taking inspiration from marginal cost pricing \cite{roughgarden2010algorithmic}, we construct an adaptive pricing scheme that ensures that the emergent traffic behavior minimizes a utilitarian measure of social optimality in long run. To this end, we construct a \emph{two-timescale} discrete-time routing algorithm that makes use of this converged price to tax the links and therefore drive them toward the socially optimal loads. This turns the selfish equilibria achieved through dynamic routing into socially optimal ones. 

We also note that our scheme allows for computationally tractable marginal cost tolls, as the central authority can \textit{adaptively} compute the tolls based on only the available state information. This is in contrast with the literature on static traffic assignment and tolling, in which the authority would need to compute the traffic equilibrium (known to be computationally intractable problem \cite{papadimitriou2007complexity}) in order to impose tolls. 


\todo[inline]{We may not be able to cite this as we are only studying parallel links.}

\subsection*{Relevant Work}
\todo[inline]{We don't need a specific section on relevant work.}
It has been known that the natural equilibria in routing games (Wardrop, stochastic user (\cite{cominetti2012modern}), etc.) are inefficient in the sense that they are not minimizers of the social cost function \cite{roughgarden2002bad}. Going back to \cite{pigou1924economics}, there have been attempts at developing tolling schemes to alleviate this problem. In particular, \cite{beckmann1956studies} mathematically demonstrated the efficacy of tolls at rates that would measure the cost to others caused by the average road user, which led to the notion of ``marginal cost tolling". Since then, there has been an extensive literature on tolling in static routing (\cite{brown2016robustness}, \cite{yang1998principle}, \cite{yang2004trial}). 
Dynamic pricing has also been studied in the repeated games setting, as in \cite{farokhi2015piecewise}. 

Dynamic pricing for ramp metering applications, especially the stabilization of traffic loads, have been studied in \cite{papageorgiou1991alinea}, \cite{yin2009dynamic}. These schemes use techniques from feedback control to control traffic load. We provide two critiques for such schemes: they are computationally intractable for the same reason as static tolling, in that they require the computation of a reference load in equilibrium that one would like the trajectory to track. Further, they do not achieve optimality of the social cost function in general without the Wardrop equilibrium to track. 

There are also corresponding optimization based schemes, such as \cite{toledo2015simulation}, {\color{red}[INCOMPLETE]}

\todo[inline]{Combine with game theoretic relevance of results.}
Further, there has been a line of work on converting the static equilibrium concepts found in \cite{wardrop1952road} into a dynamic system. Much of the literature focuses on learning dynamics such as the  found in \cite{krichene2014convergence}, or casts the problem of dynamic traffic routing as a repeated game \cite{la2002optimal}. This literature does not take into account the residual loads and delays that are present in real-world traffic networks. Therefore, the timescale of such algorithms is in days.

\todo[inline]{Maybe not needed.}
We should also mention that there are various natural ways of extending the static routing framework into a dynamic one based on conservation laws at the link level. The cell-transmission model  discretizes links into cells and models traffic as a fluid \cite{daganzo1994cell}, and there is a line of work going back to \cite{lighthill1955kinematic} that studies traffic through partial differential equations (PDEs) and load conservation. We note that these models do not preserve the game theoretic relevance that we desire to model the \textit{strategic} interactions in traffic on networks. 

\todo[inline]{Move before.}
The works closest to ours in philosophy are \cite{borkar2009cooperative}, \cite{pietrabissa2018discrete}, and \cite{como2021distributed}. These build in a dynamic load adjustment at the network level scheme based on conservation laws whose steady states are Wardrop equilibria. Therefore, the strategic decisions made by loads are accounted for. However, \cite{borkar2009cooperative} and \cite{pietrabissa2018discrete} do not address the issue of dynamic pricing to social optima, and \cite{como2021distributed} addresses the question of fast-changing pricing (and correspondingly slow-changing preferences) for a large class of dynamic feedback control policies, in contrast to our study specifically of \textit{slow-changing marginal cost tolls}. There is evidence in the economics literature that users prefer slow-changing taxes \cite{farokhi2015piecewise}.


\end{comment}

\begin{comment}
\begin{center}
    \begin{tabular}{|c|l|}
    \hline 
    Notation & Description \\
    \hline 
      \(\flowDiscrete_i(n)\)  & load on link \(i\) at time \(n\)\\
         \(\priceDiscrete_i(n)\) & price on the link \(i\) at time \(n\)\\ \(\costEdge_i(\cdot)\) & congestion cost as a function of load on that edge \\ 
         \(\costPrice_i(\cdot,\cdot)\) & congestion cost as a function of load and the price assigned \\ 
         \(\sueParameter\) & the parameter which parametrizes the assignment ratios \\ 
         \(\meanInflow\) & mean inflow rate \\
         \(\meanOutflow\) & mean outflow rate \\ 
         \(\inflow_i(n)\) & random variable that decides inflow on link \(i\) at time \(n\) \\ 
         \(\outflow_i(n)\) & random variable that decides the outflow ratio on link \(i\) at time \(n\) \\ 
         \(\flowContinuous_i(t)\) & flow on link \(i\) at time \(t\) in the ode \\
         \(\priceContinuous_i(t)\) & price on link \(i\) at time \(t\) in the ode \\
         \(\numLinks\) & number of links in the network\\
         \(\stepPrice\)& step size used to update the pricing dynamics\\
         \hline 
     \end{tabular}
\end{center}
\end{comment}


\subsection*{Notations}
We denote the set of non-negative real numbers by \(\Rp\). For any natural number \(R\), we succinctly write \([R] = \{1,2,\dots,R\}\). For any vector \(x\in \R^n\), we define \(\diag(x)\in\R^{n\times n}\) to be a diagonal matrix with its diagonals filled with entries of \(x\). 








==> Dynamic_Routing_Regular (Arxiv)/intro_revised.tex <==
\section{Introduction}\label{sec: Intro}

Efficient traffic routing is an increasingly important problem as congestion aggravates on urban transportation networks. Many cities around the world have implemented congestion pricing (tolling) to regulate the demand of travelers (\cite{latimes2021,nyt2021}). Tolling, when properly set in response to real-time traffic conditions, can effectively alleviate congestion and even induce socially optimal loads \cite{sharon2017real, paccagnan2019incentivizing}. 

One challenge of setting tolls is that travelers continuously arrive at and depart from the network, which creates a dynamic evolvement of traffic loads in network. Additionally, travelers are selfish in that they prefer to choose the routes with the minimum cost - travel time cost and the tolls combined. To design tolling that induces efficient traffic load, we must account for the dynamics of incoming and outgoing traffic demands and the selfish nature of travelers' route choices. In particular, the tolls must be updated in response to the changing traffic conditions. 


%In real world traffic networks, users arrive dynamically and make routing decisions based on the existing congestion of the network, and the natural equilibria in routing games (Wardrop, stochastic user (\cite{cominetti2012modern}), etc.) are inefficient in the sense that they are not minimizers of the social cost function \cite{roughgarden2002bad}. how should we set tolls dynamically such that the joint evolution of the load and price converges to social optimality? 

% Para 1 on modeling 
We propose a discrete-time stochastic dynamics to capture the joint evolution of the loads and tolls in a parallel network. In each time step of the dynamics, non-atomic travelers arrive at the origin of the network, and they make routing decisions according to a perturbed best response based on the travel time cost and toll of each link in that step. Additionally, a fraction of load on each link leaves the network. Both the incoming and outgoing demand are randomly realized, and are identically and independently distributed across steps. Therefore, the discrete-time stochastic dynamics of loads forms a Markov process, which is governed by the total arriving demand, the stochastic user equilibrium, and the load discharge rate. Furthermore, at each time step, a traffic authority adjusts the toll on each link by interpolating between the current toll and a new increment dependent on the marginal cost of travel time given the load at that step. 

In our setting, the dynamics of the toll evolves at a slower time-scale compared to that of the load dynamics. In practice, fast changing tolls are undesirable (\cite{farokhi2015piecewise}). This property ensures that the tolls change very slowly, and thus travelers can view the tolls as static when they make routing decisions at the arrival. %Therefore, price does not change during their trip. That is, when travelers make routing decisions at , extending the extensive literature on tolling in static routing (\cite{brown2016robustness}, \cite{yang1998principle}, \cite{yang2004trial}). 

%This model builds upon existing work in dynamic traffic routing in two main ways: 1) We incorporate a ``two-timescale'' toll update, in which tolls evolve slowly as compared to the loads, and 2) our model allows for stochasticity in the incoming demand and outgoing loads.
%, and therefore, we are able to analyze the dynamics as a random process. 

% Para 1 of Results: Convergence results

 


We show that the loads and tolls in the discrete-time stochastic dynamics asymptotically concentrate in a neighborhood of a unique fixed point with high probability. The fixed point load is \emph{socially optimal} in that it minimizes the total travel time costs when the incoming and outgoing traffic demands reach a \emph{steady state}, and the fixed point toll on each link equals to the marginal cost. That is, with high probability, our dynamic tolling eventually induces the socially optimal loads that accounts for the incoming and outgoing travelers and their selfish routing behavior. Furthermore, we emphasize that our dynamic tolling is \emph{distributed} in that the traffic authority only uses the information of the cost and load on each link to update its toll.  % (\cite{roughgarden2010algorithmic, farokhi2015piecewise}). The socially optimal load corresponds to the {\color{red}``steady-state''} equilibrium of our dynamics when the tolls are set at the socially optimal values. 

% Para 2 of Results: Link between the discrete time and continuous time 

Our technical approach to proving the main result involves: \emph{(i)} Constructing a continuous-time deterministic dynamical system associated with the two timescale discrete-time stochastic dynamics; \emph{(ii)} Demonstrating that the flow of the continuous-time dynamical system has a unique fixed point that corresponds to the socially optimal load and tolls; \emph{(iii)} Proving that the unique fixed point of the flow of the continuous time dynamical system is globally stable. In particular, we apply the theory of two time-scale stochastic approximation to show that the loads and tolls under the stochastic dynamics concentrates with high probability in the neighborhood of the fixed point of the flow of continuous time dynamics constructed in \emph{(i)} (\cite{borkar2009stochastic}). Additionally, our proof in \emph{(ii)} on the uniqueness and optimality of fixed point of the flow of continuous time dynamics builds on a variational inequality, and extends the analysis of stochastic user equilibrium in static routing games to account for the steady state of the network given the incoming and outgoing demand (\cite{cominetti2012modern}). Furthermore, we show that the continuous time dynamical system is cooperative, and thus its flow must converge to its fixed point (\cite{hirsch1985systems}). 


%In order to prove the main result we consider an underlying continuous-time deterministic dynamical system that ``closely'' approximates the discrete-time stochastic dynamical system. Such a continuous-time dynamical system is obtained by leveraging the slower update of toll-price dynamics. This property is popularly referred as the ``two-timescale'' property \cite{borkar2009stochastic}.  We show that the continuous-time dynamical system admits unique fixed points that are the same as the socially optimal loads and tolls respectively.  Furthermore, we show that the trajectories of the continuous-time dynamical system in fact converge to the fixed points, which in turn ensures that the discrete-time dynamics concentrates in a neighborhood of socially optimal load with high probability.

% Para 3 of Results: Discuss the techniques
%We design the discrete-time dynamics such that the fixed point of the underlying continuous-time load dynamics, at any \emph{fixed} toll-price, is a game theoretically motivated quantity -- namely it is the ``steady-state'' stochastic user equilibrium at that toll under an \emph{equivalent demand} dependent on the inload and outload. One of our main technical results we establish that such fixed points are monotonic in toll-prices. Broadly speaking, this property ensures that increasing toll-prices on particular link reduces the load on that link.  The convergence of the underlying continuous-time dynamics is established by exploiting this monotonicity in conjunction with the results from \emph{cooperative dynamical systems theory} \cite{hirsch1985systems}. 

Our model and results contribute to the rich literature on designing tolling mechanisms for inducing socially optimal route loads. Classical literature on static routing games has focused on measuring the inefficiency of selfish routing by bounding the "price of anarchy", and designing marginal cost tolling to induce socially optimal route loads (\cite{christodoulou2005price, roughgarden2002bad, roughgarden2010algorithmic}). In static routing games, optimal tolling does not account for the dynamic arrival and departure of travelers. The computation of optimal tolls relies on knowledge of the entire network structure and the equilibrium route flows, which are challenging to compute. 

Dynamic toll pricing has been studied in a variety of settings to account for the continuous incoming and outgoing traffic demand. The paper \cite{borkar2009cooperative} analyzed a discrete-time stochastic dynamics of of non-atomic travelers, and discussed the impact of tolling on routing strategies. We consider an adaptive adjustment of tolls using marginal toll pricing. This allows us to analyze the long-run outcomes of the joint evolution of the route loads and tolls, and shows that the tolls eventually induce a socially optimal traffic load associated with the steady state of the network. Additionally, we prove that the monotonicity condition  -- the equilibrium routing strategy is monotonic in tolls (which is an assumption in \cite{borkar2009cooperative}) -- holds for any equilibrium routing strategy. 

Moreover, \cite{como2021distributed} proposed a continuous-time dynamical system to study socially optimal tolling when strategic travelers continuously arrive and make selfish routing decisions. In their model, the incoming and outgoing traffic demands are equal so that the aggregate load in the network is a constant. In our setting, both the incoming and outgoing traffic demands are random variables. Therefore, our fixed point analysis needs to account for the total load at the steady state of the network. Moreover, \cite{como2021distributed} assumes that the tolls are adjusted at a faster time scale than their traveler's route preferences, while we assume that the update of tolls is at a slower timescale compared to the change of routing decisions.  

Finally, this article is also related to the literature on learning in routing games, and learning for tolling with unknown network condition. In particular, a variety of algorithms have been proposed to study how travelers learn an equilibrium by repeatedly adjusting their routing decisions based on the observed travel time in the network (e.g. \cite{cominetti2010payoff, krichene2014convergence, kleinberg2009multiplicative}). Additionally, papers \cite{farokhi2015piecewise, poveda2017class, meigs2017learning, wu2020bayesian} have analyzed how the traffic authority adaptively updates the tolls while learning the unknown network condition using crowd-sourced data on traffic load and time costs.




%We note that much of the literature on dynamics in traffic routing focuses on learning dynamics such as those found in \cite{krichene2014convergence}, or casts the problem of dynamic traffic routing as a repeated game \cite{la2002optimal}. This literature does not take into account the \textit{residual loads} and \textit{delays} that are present in real-world traffic networks.

%The works closest to ours in philosophy are \cite{borkar2009cooperative}, \cite{pietrabissa2018discrete}, and \cite{como2021distributed}. These build in a dynamic load adjustment at the network level scheme based on conservation laws whose steady states are Wardrop equilibria, and thus the strategic decisions made by loads are accounted for. However, \cite{borkar2009cooperative} and \cite{pietrabissa2018discrete} do not address the issue of dynamic pricing to social optima, and \cite{como2021distributed} addresses the question of fast-changing pricing (and correspondingly slow-changing preferences) for a large class of dynamic feedback control policies. In contrast we study \textit{slow-changing marginal cost tolls} which are more preferable to users \cite{farokhi2015piecewise}.

This article is organized as follows: we introduce the dynamic tolling model and the discrete time stochastic dynamics in Sec. \ref{sec: Model}. We present the main result in Sec. \ref{sec: Results}, and numerical examples in Sec. \ref{sec: NumExp}. We conclude our work in Sec. \ref{sec: Conclusion}. We present the key ideas of our prove techniques in the main text, and include all proofs in the appendix. 
%We also note that our scheme allows for computationally tractable marginal cost tolls, as the central authority can \textit{adaptively} compute the tolls based on only the available state information. This is in contrast with the literature on static traffic assignment and tolling, in which the authority would need to compute the traffic equilibrium (known to be computationally intractable problem \cite{papadimitriou2007complexity}) in order to impose tolls. 

%Dynamic traffic routing and tolling presents a novel problem as technologies like navigation apps have enabled flexible routing both spatially and temporally \cite{aswani2011game}. As road congestion worsens as a result of selfish game-theoretic behavior from traffic, it is important to study the effect of interventions like tolling on network state. 



\begin{comment}
{\color{red} Beyond this point it is yet to be updated}
In this article, we use techniques from \emph{cooperative} dynamical systems theory \cite{hirsch1985systems} and two-timescale stochastic approximation \cite{borkar2009stochastic} to prove the convergence of these stochastic dynamics to socially optimal tolls and loads. We show that the discrete-time dynamics asymptotically track a continuous time o.d.e., and that the o.d.e. converges to the socially optimal loads and tolls given a particular construction of the tolls that uses the \textit{marginal cost} incurred on each link. 
We prove a novel monotonicity result 

% \todo[inline]{Model description, comments, and discussion/techniques: Add our contributions here. Second paragraph should focus on model, begin paragraph with ``We propose a discrete time stochastic dynamics that addresses the joint evolution of load and tolls. The introduction should tell about the model. People arrive at origin and make decisions; tolls are set by central authority. Comment on dynamics of $x$ and $p$. End with question: how should we set tolls in this dynamics such that the dynamic converges to social optimality. We also need to justify two time-scale in the next paragraph.

% Also a paragraph to emphasize the novelty of the model.}
% \tdBox{Results around 3 paragraph: Dynamics converge to the socially optimal load. Find continuous dynamics approximating this dynamics. Find continuous dynamics is equilibirium}
% \tdBox{Comment about the techniques: Hirsch and monotonicity. DONT give sense that it is direct deployment. Point out game theoretic aspect. }
Correspondingly, time dynamical routing and its convergence to game theoretic equilibria has been studied in \cite{borkar2009cooperative}. This routing framework allows one to keep track of loads dynamically as they travel through a network, in contrast to the static or repeated routing schemes traditionally found in the literature.  

The challenge is that there is a need for a new mechanism to set tolls adaptively in response to the dynamically evolving traffic conditions, which are determined by the coming and going of traffic in the network and also by the \textit{selfish} routing decisions made by the travelers.
%This paper extends previous work by including a pricing dynamic that ensures link loads minimizes a utilitarian measure of social optimality. 
Taking inspiration from marginal cost pricing \cite{roughgarden2010algorithmic}, we construct an adaptive pricing scheme that ensures that the emergent traffic behavior minimizes a utilitarian measure of social optimality in long run. To this end, we construct a \emph{two-timescale} discrete-time routing algorithm that makes use of this converged price to tax the links and therefore drive them toward the socially optimal loads. This turns the selfish equilibria achieved through dynamic routing into socially optimal ones. 

We also note that our scheme allows for computationally tractable marginal cost tolls, as the central authority can \textit{adaptively} compute the tolls based on only the available state information. This is in contrast with the literature on static traffic assignment and tolling, in which the authority would need to compute the traffic equilibrium (known to be computationally intractable problem \cite{papadimitriou2007complexity}) in order to impose tolls. 


\todo[inline]{We may not be able to cite this as we are only studying parallel links.}

\subsection*{Relevant Work}
\todo[inline]{We don't need a specific section on relevant work.}
It has been known that the natural equilibria in routing games (Wardrop, stochastic user (\cite{cominetti2012modern}), etc.) are inefficient in the sense that they are not minimizers of the social cost function \cite{roughgarden2002bad}. Going back to \cite{pigou1924economics}, there have been attempts at developing tolling schemes to alleviate this problem. In particular, \cite{beckmann1956studies} mathematically demonstrated the efficacy of tolls at rates that would measure the cost to others caused by the average road user, which led to the notion of ``marginal cost tolling". Since then, there has been an extensive literature on tolling in static routing (\cite{brown2016robustness}, \cite{yang1998principle}, \cite{yang2004trial}). 
Dynamic pricing has also been studied in the repeated games setting, as in \cite{farokhi2015piecewise}. 

Dynamic pricing for ramp metering applications, especially the stabilization of traffic loads, have been studied in \cite{papageorgiou1991alinea}, \cite{yin2009dynamic}. These schemes use techniques from feedback control to control traffic load. We provide two critiques for such schemes: they are computationally intractable for the same reason as static tolling, in that they require the computation of a reference load in equilibrium that one would like the trajectory to track. Further, they do not achieve optimality of the social cost function in general without the Wardrop equilibrium to track. 

There are also corresponding optimization based schemes, such as \cite{toledo2015simulation}, {\color{red}[INCOMPLETE]}

\todo[inline]{Combine with game theoretic relevance of results.}
Further, there has been a line of work on converting the static equilibrium concepts found in \cite{wardrop1952road} into a dynamic system. Much of the literature focuses on learning dynamics such as the  found in \cite{krichene2014convergence}, or casts the problem of dynamic traffic routing as a repeated game \cite{la2002optimal}. This literature does not take into account the residual loads and delays that are present in real-world traffic networks. Therefore, the timescale of such algorithms is in days.

\todo[inline]{Maybe not needed.}
We should also mention that there are various natural ways of extending the static routing framework into a dynamic one based on conservation laws at the link level. The cell-transmission model  discretizes links into cells and models traffic as a fluid \cite{daganzo1994cell}, and there is a line of work going back to \cite{lighthill1955kinematic} that studies traffic through partial differential equations (PDEs) and load conservation. We note that these models do not preserve the game theoretic relevance that we desire to model the \textit{strategic} interactions in traffic on networks. 

\todo[inline]{Move before.}
The works closest to ours in philosophy are \cite{borkar2009cooperative}, \cite{pietrabissa2018discrete}, and \cite{como2021distributed}. These build in a dynamic load adjustment at the network level scheme based on conservation laws whose steady states are Wardrop equilibria. Therefore, the strategic decisions made by loads are accounted for. However, \cite{borkar2009cooperative} and \cite{pietrabissa2018discrete} do not address the issue of dynamic pricing to social optima, and \cite{como2021distributed} addresses the question of fast-changing pricing (and correspondingly slow-changing preferences) for a large class of dynamic feedback control policies, in contrast to our study specifically of \textit{slow-changing marginal cost tolls}. There is evidence in the economics literature that users prefer slow-changing taxes \cite{farokhi2015piecewise}.


\end{comment}

\begin{comment}
\begin{center}
    \begin{tabular}{|c|l|}
    \hline 
    Notation & Description \\
    \hline 
      \(\flowDiscrete_i(n)\)  & load on link \(i\) at time \(n\)\\
         \(\priceDiscrete_i(n)\) & price on the link \(i\) at time \(n\)\\ \(\costEdge_i(\cdot)\) & congestion cost as a function of load on that edge \\ 
         \(\costPrice_i(\cdot,\cdot)\) & congestion cost as a function of load and the price assigned \\ 
         \(\sueParameter\) & the parameter which parametrizes the assignment ratios \\ 
         \(\meanInflow\) & mean inflow rate \\
         \(\meanOutflow\) & mean outflow rate \\ 
         \(\inflow_i(n)\) & random variable that decides inflow on link \(i\) at time \(n\) \\ 
         \(\outflow_i(n)\) & random variable that decides the outflow ratio on link \(i\) at time \(n\) \\ 
         \(\flowContinuous_i(t)\) & flow on link \(i\) at time \(t\) in the ode \\
         \(\priceContinuous_i(t)\) & price on link \(i\) at time \(t\) in the ode \\
         \(\numLinks\) & number of links in the network\\
         \(\stepPrice\)& step size used to update the pricing dynamics\\
         \hline 
     \end{tabular}
\end{center}
\end{comment}


\subsection*{Notations}
We denote the set of non-negative real numbers by \(\Rp\). For any natural number \(R\), we succinctly write \([R] = \{1,2,\dots,R\}\). For any vector \(x\in \R^n\), we define \(\diag(x)\in\R^{n\times n}\) to be a diagonal matrix with its diagonals filled with entries of \(x\). 








==> Dynamic_Routing_Regular (Arxiv)/model.tex <==
\section{Model}\label{sec: Model}
  Consider a parallel link network with \(\numLinks\) links connecting a single source-destination pair. The network is occupied by the \emph{non-atomic} population of travellers that continuously arrive at the source node at each time $n =0, 1, 2, \dots$, and are routed through links \(\numLinks\) to the destination node. 
  
  At each time $n$, the flow (i.e. amount of travellers) on link \(i\in [\numLinks]\) is \(\flowDiscrete_i(n)\). The average latency experienced by the travellers on any link \(i \in [\numLinks]\) is a function of flow on the link \(\latency_i: \Rp \ra\Rp\). We assume the latency function is \emph{strictly-increasing} and \emph{convex}, which reflect the congestive nature of links and the fact that the latency increases faster when the flow is higher. 
  
  
  A traffic authority sets toll prices on links, denoted as $\priceDiscrete(n)=\left(\priceDiscrete_i(n)\right)_{i \in \R}$, where $\priceDiscrete_i(n)$ is the toll price on link $i$ at time $n$. The \emph{cost} of an individual traveller who uses any link \(i\in[\numLinks]\) at time $n$, denoted $\costPrice_i(\flowDiscrete_i(n), \priceDiscrete_i(n))$, equals to the experienced travel time cost, which is sum of the average latency function \(\latency_i(\flowDiscrete_i(n))\), a noise term $\upsilon_i(n)$ with zero mean, and the charged toll price: 
  \begin{align*}
      \costPrice_i(\flowDiscrete_i(n), \priceDiscrete_i(n)) \defas \latency_i(\flowDiscrete_i(n)) + \priceDiscrete_i(n)+\textcolor{red}{ \upsilon_i(n)}.
  \end{align*} 
  A schematic summarizing the aforementioned setup is presented in Fig. \ref{fig: SchematicFigure}.
  
  %Further, each link gets tolled by a price of $\priceDiscrete_i(n)$ at every time $n$ with the goal of achieving socially optimal routing of the travellers. To be precise, we demand that the flows on the links asymptotically correspond to the minimizer of the utilitarian \emph{social cost function}$S: \R^{\numLinks} \ra  \R$ where $ S(x) \defas \sum_{i\in [R]} x_i \latency_i(x_i)$. 
  
  
 

 
\begin{figure}[h]
\begin{tikzpicture}[main/.style = {draw, circle}] 
\node[main] (1) {$\mc{S}$}; 
\node[main] (2) [right= 8cm of 1] {$\mc{D}$}; 
\draw[->] (1) to [out=70,in=110,looseness=1.2] node[midway,above] {$\costPrice_1(\flowDiscrete_1(n), \priceDiscrete_1(n))$} (2);
\draw[->] (1) to [out=45,in=135,looseness=0.8] node[midway,above] {$\costPrice_2(\flowDiscrete_2(n) ,\priceDiscrete_2(n)$} (2);
\draw[->] (1) to [out=0,in=180,looseness=0.8] node[midway,above] {$\dots$} (2);
\draw[->] (1) to [out=-45,in=225,looseness=0.8] node[midway,below] {$\costPrice_{R-1}(\flowDiscrete_{R-1}(n), \priceDiscrete_{R-1}(n))$} (2);
\draw[->] (1) to [out=-70,in=-110,looseness=1.2] node[midway,below] {$\costPrice_{R}(\flowDiscrete_R(n), \priceDiscrete_R(n))$} (2);
\end{tikzpicture} 
\caption{Schematic of a \(\numLinks-\)link parallel network with source node \(\mc{S}\) and the destination node \(\mc{D}\) with the corresponding cost to travellers at time \(n\).}
\label{fig: SchematicFigure}
\end{figure}


  
  The demand of travellers arriving at the source node at time \(n\) is a random variable $\inflow(n)$. We assume that  \(\{\inflow(n)\}_{n\in\N}\) are independently and identically distributed (i.i.d) with bounded support $[\inflowLower,\inflowUpper]$ and a finite mean $\lambda$ (i.e. \(\avg[\inflow(n)] = \meanInflow\)). Travelers make routing decisions based on the latest cost vector $\costPrice(n-1)$ at time $n-1$. We denote travelers' routing strategy at time $n$ as $\flowIn(n) = \left(\flowIn_i(n)\right)_{i \in \R}$, where $\flowIn_i(n)$ is the demand of travelers who choose link $i$. We assume that $\flowIn(n)$ is a \emph{stochastic user equilibrium} defined as follows:  %Further, the fraction of flow leaving link $i$ at time $n$ is $\outflow_i(n)$, and $\{\outflow_i(n)\}_{n \in N}$ are i.i.d. as well, with a finite mean $\avg[\outflow_i(n)] = \meanOutflow \in (0,1)$. We also assume that $\inflow_i(n)$ and $\outflow_i(n)$ have bounded support. Specifically, for every \(i\in[\numLinks]\) and       \(n\in\N\), \(\inflow(n) \in [\inflowLower,\inflowUpper]\) almost surely and \(\outflow_i(n) \in [\outflowLower,\outflowUpper]\) almost surely. Moreover \(\outflowLower > 0\) and \(\outflowUpper < 1\).
  
  %The demand at the source node is allocated to different links in accordance to the allocations under \emph{stochastic user equilibrium}. Stochastic user equilibrium is a commonly used routing paradigm that captures the behavioral aspect of traveller's decision making in response to stochastic perception of travel cost associated with different links. 
 \begin{definition}[\textbf{Stochastic User Equilibrium} (\cite{})]\label{assm: InflowAssumption}
  At any time \(n\in \N\), a routing strategy $\flowIn(n)$ is a stochastic user equilibrium if 
  \begin{align}\label{eq: InflowEquation}
     \flowIn_i(n) \defas \frac{\exp(-\sueParameter \costPrice_i(\flowDiscrete_i(n-1), \priceDiscrete_i(n-1)))}{\sum_{j\in[R]}\exp(-\sueParameter \costPrice_j(\flowDiscrete_j(n-1), \priceDiscrete_j(n-1)))}\inflow(n), \quad \forall i \in \R,  
 \end{align}
 where $\beta \in [0, \infty)$. 
  \end{definition}
  
  \textcolor{red}{Here, the parameter $\sueParameter$ characterizes the relative weight the traveller assigns between higher and lower costs. As $\sueParameter \downarrow 0$, the inflows  $\flowIn_i(n) = \flowIn_j(n)$ for all $i,j$. However, as $\sueParameter \uparrow \infty$, $\flowIn_i(n) = \max_{j} (\flowIn_j(n))$ and $\flowIn_i(n) = 0$ for all $i \not\in\{ j : \flowIn_i(n) = \max_{j}(\flowIn_i(n))\}$.}
  
  
   \textcolor{red}{The route choice model represents a \emph{myopic, selfish}, and \textit{perturbed} best-response strategy for picking flow splitting, for $\beta$ finite and nonzero. That is, the flows pick the links with low cost (and leave higher cost links empty), but experience a perturbed version of the cost. Therefore, as $\beta \uparrow \infty$, the inflow approximates the route choice corresponding to Wardrop equilibrium \cite{cominetti2012modern}}.
   \todo[inline]{Borrow formal language}
  
Furthermore, for any \(i\in[\numLinks]\) the proportion of existing flow leaving that link at time \(n\) is given by the random variable \(\outflow_i(n) \in [0,1]\). Thus the flow actually leaving out from link \(i\in[\numLinks]\) at time \(n\in\N\) is given by \begin{align}\label{eq:outflow}
    \flowOut_i(n) \defas \flowDiscrete_i(n-1)\outflow_i(n).
\end{align}
  

\subsection{Discrete time stochastic dynamics} 
We characterize the evolution of the flow on each link in the network by the following discrete time stochastic dynamics: 
\begin{align}\label{eq:x_original}
    \flowDiscrete_i(n+1) &= \flowDiscrete_i(n) +  \flowIn_i(n+1) - \flowOut_i(n+1) .
\end{align}
We note that the stochasticity of the flow dynamics arises from the randomness in demand arrival $\flowIn(n)$ and the outflow rate $\flowOut(n)$. By combining \eqref{eq: InflowEquation} -- \eqref{eq:outflow}, We re-write \eqref{eq:x_original} as follows: 
\begin{equation}\label{eq: FlowDynamics}
\begin{aligned}
    \flowDiscrete_i(n+1) &=  \flowDiscrete_i(n) + \frac{\exp(-\sueParameter \costPrice_i(\flowDiscrete_i(n-1), \priceDiscrete_i(n-1)))}{\sum_{j\in[R]}\exp(-\sueParameter \costPrice_j(\flowDiscrete_j(n-1), \priceDiscrete_j(n-1)))}\inflow(n) -  \flowDiscrete_i(n-1)\outflow_i(n)\\
    &=(1-\meanOutflow) \flowDiscrete_i(n) + \textcolor{red}{\frac{\exp(-\sueParameter \costPrice_i(\flowDiscrete_i(n),\priceDiscrete_i(n)))}{\sum_{j\in[R]}\exp(-\sueParameter \costPrice_j(\flowDiscrete_j(n),\priceDiscrete_j(n)))}\meanInflow} + \meanOutflow\martingale_i(n+1),
\end{aligned}
\end{equation}

\begin{align}\label{eq: hVectorFieldDef}
\vectorFieldX_i(x,p) \defas \frac{\meanInflow}{\meanOutflow}\frac{\exp(-\sueParameter \costPrice_i(x,p))}{\sum_{j\in[R]}\exp(-\sueParameter \costPrice_j(x,p))}. 
\end{align}


where $\meanInflow$ and $\meanOutflow$ are the mean of the random variables $\flowIn(n)$ and $\flowOut(n)$, respectively, and
\begin{align}\label{eq: MartingaleDefinition}
\martingale_i(n+1) \defas \frac{1}{\meanOutflow} \lr{ \frac{\exp(-\sueParameter \costPrice_i(\flowDiscrete_i(n),\priceDiscrete_i(n) ))}{\sum_{j\in[R]}\exp(-\sueParameter \costPrice_j(\flowDiscrete_j(n), \priceDiscrete_j(n)))}\lr{\inflow_i(n+1) - \meanInflow } - \flowDiscrete_i(n)\lr{\outflow_i(n+1)- \meanOutflow} }. 
\end{align}


%The advantage of latter version of flow update is that it allows us to think about \(\meanOutflow\) as a step size.

Furthermore, the central authority updates the toll price vector $\priceDiscrete(n)$ in each time $n$ as follows: 
\begin{align}\label{eq: PricingDynamics}
\priceDiscrete_i(n+1) = (1-a)\priceDiscrete_i(n) + a \flowDiscrete_i(n)\grad_x\costPrice_i(\flowDiscrete_i(n), \priceDiscrete_i(n)) \quad \forall i \in [\numLinks], n\in \N, 
\end{align}
\color{red}where \(a>0\) is the step size.
That is, the toll price updates towards a small step in the direction of \emph{marginal cost} from its current value at time \(n\). We note that the toll update on each link $i$ only depends on the flow and cost of $i$ at time $n$ instead of the entire network. That is, the tolls are updated in a \emph{distributed} manner.  

We posit that the toll prices and latency additively realize the total cost on any link. That is,  $\costPrice_i(\flowDiscrete_i(n), \priceDiscrete_i(n)= \latency(\flowDiscrete_i(n)) + \priceDiscrete_i(n)$. This is consistent with the theory from tolling in static routing \cite{roughgarden2010algorithmic}, in which marginal cost prices also enter the cost functions of every link additively. 

For later reference, we present below the combined flow and price update dynamics \begin{equation}\label{eq: CombinedDT}
    \begin{aligned}
     \flowDiscrete_i(n+1) &=  \flowDiscrete_i(n) + \meanOutflow\lr{\frac{\meanInflow}{\meanOutflow}\frac{\exp(-\sueParameter \costPrice_i(\flowDiscrete_i(n),\priceDiscrete_i(n)))}{\sum_{j\in[R]}\exp(-\sueParameter \costPrice_j(\flowDiscrete_j(n),\priceDiscrete_j(n)))} - \flowDiscrete_i(n)} + \meanOutflow\martingale_i(n+1),\\
     \priceDiscrete_i(n+1) &= (1-a)\priceDiscrete_i(n) + a \flowDiscrete_i(n)\grad_x\costEdge_i(\flowDiscrete_i(n)) \quad \forall i \in [\numLinks], n\in \N.
    \end{aligned}
\end{equation}

% This model follows a class of dynamics in the spirit of \cite{borkar2009cooperative} and \cite{pietrabissa2018discrete}. In particular, we note that the dynamic is distinguished from classical dynamics in routing games (gradient descent, multiplicative weights, etc.) in that it explicitly accounts for the inflow and outflow of vehicles through a conservation law.

At last, we assume that in \eqref{eq: CombinedDT} the price dynamics update on a slower time scale than the flow dynamics. That is, \(a << \meanOutflow\). Slow price updation is a desirable feature to have from the traveller's perspective \cite{farokhi2015piecewise} as it gives them appropriate time to respond. 
\color{black}
% \textcolor{red}{
% \begin{itemize}
%     \item \sout{Introduce tolls in the beginning. Add toll prices in the cost function when it is first introduced in route choices rather than later }
%     \item \sout{Rephrase "assumptions" as setups, and put them in line}
%     \item \sout{You need to introduce two timescale here, and justify it}
%     \item Put technical parts in the technical section 
%     \item Avoid loose English and casual use of terminologies that you don't define 
%     \item \sout{Name the dynamics as X-update, p-update (or something else that makes sense to you). It is easier for readers to remember them since they are referred repeatedly throughout}
% \end{itemize}}

==> Dynamic_Routing_Regular (Arxiv)/model_revised.tex <==
\section{Model}\label{sec: Model}
  Consider a parallel link network with \(\numLinks\) links connecting a single source-destination pair. At each time step $n=1, 2, \dots$, a non-atomic traveler population arrives at the source node, and is routed through links \(\numLinks\) to the destination node. 
  
  At time step $n$, the traffic load (i.e. amount of travellers) on link \(i\in [\numLinks]\) is \(\flowDiscrete_i(n)\). The latency function on any link \(i \in [\numLinks]\) is a function of load on the link: \(\latency_i: \Rp \ra\Rp\). We assume that the latency function is \emph{strictly-increasing} and \emph{convex}, which reflect the congestible nature of links and the fact that the latency increases faster when the load is higher. 
  
  
  A traffic authority sets toll prices on links, denoted as $\priceDiscrete(n)=\left(\priceDiscrete_i(n)\right)_{i \in \R}$, where $\priceDiscrete_i(n)$ is the toll on link $i$ at step $n$. The \emph{cost function} on link \(i\in[\numLinks]\) at step $n$, denoted $\costPrice_i(\flowDiscrete_i(n), \priceDiscrete_i(n))$, is the sum of the latency function \(\latency_i(\flowDiscrete_i(n))\) and the charged toll price (see Fig. \ref{fig: SchematicFigure}): 
  \begin{align}\label{eq: costAssumption}
      \costPrice_i(\flowDiscrete_i(n), \priceDiscrete_i(n))) \defas \latency_i(\flowDiscrete_i(n)) + \priceDiscrete_i(n)
  \end{align}
  
  \begin{figure}[h]
\centering
\begin{tikzpicture}[main/.style = {draw, circle}] 
\node[main] (1) {$\mc{S}$}; 
\node[main] (2) [right= 5cm of 1] {$\mc{D}$}; 
\draw[->] (1) to [out=70,in=110,looseness=0.8] node[midway,above] {$\costPrice_1(\flowDiscrete_1(n), \priceDiscrete_1(n))$} (2);
\draw[->] (1) to [out=45,in=135,looseness=0.4] node[midway,above] {$\costPrice_2(\flowDiscrete_2(n) ,\priceDiscrete_2(n))$} (2);
\draw[->] (1) to [out=0,in=180,looseness=0.4] node[midway,above] {$\dots$} (2);
\draw[->] (1) to [out=-45,in=225,looseness=0.4] node[midway,below] {$\costPrice_{R-1}(\flowDiscrete_{R-1}(n), \priceDiscrete_{R-1}(n))$} (2);
\draw[->] (1) to [out=-70,in=-110,looseness=0.8] node[midway,below] {$\costPrice_{R}(\flowDiscrete_R(n), \priceDiscrete_R(n))$} (2);
\end{tikzpicture} 
\caption{A \(\numLinks-\)link parallel network with source node \(\mc{S}\), destination node \(\mc{D}\), and cost functions at step \(n\).}
\label{fig: SchematicFigure}
\end{figure}

  Furthermore, we define \(\tilde{\costPrice}_i(\flowDiscrete_i(n), \priceDiscrete_i(n), \nu_i(n)) \defas \costPrice_i(\flowDiscrete_i(n) , \priceDiscrete_i(n)) + \nu_i(n)\) to be the randomly realized travel cost experienced by the travelers, where $\nu_i(n)$ is an identically and independently distributed (i.i.d) random variable with zero mean. %Naturally, $\mathbb{E}_{\nu_i}[\tilde{\costPrice}_i(\flowDiscrete_i(n), \priceDiscrete_i(n), \nu_i(n))] = \costPrice(\flowDiscrete_i(n), \priceDiscrete_i(n))$. A schematic summarizing the aforementioned setup is presented in .
  
  %Further, each link gets tolled by a price of $\priceDiscrete_i(n)$ at every time $n$ with the goal of achieving socially optimal routing of the travellers. To be precise, we demand that the flows on the links asymptotically correspond to the minimizer of the utilitarian \emph{social cost function}$S: \R^{\numLinks} \ra  \R$ where $ S(x) \defas \sum_{i\in [R]} x_i \latency_i(x_i)$. 
  
  
 

 



  
  The demand of traffic arriving at the source node at step \(n+1\) is a random variable $\inflow(n+1)$. We assume that  \(\{\inflow(n)\}_{n\in\N}\) are i.i.d with bounded support $[\inflowLower,\inflowUpper]$ and the mean $\lambda$ (i.e. \(\avg[\inflow(n)] = \meanInflow\) for all \(n\)). At step \(n+1\), travelers make routing decisions $\flowIn(n+1) = \left(\flowIn_i(n+1)\right)_{i \in [\numLinks]}$ based on the latest cost vector at step $n$, where $\flowIn_i(n+1)$ is the demand of travelers who choose link $i$ at step \(n+1\). We assume that $\flowIn(n+1)$ is a perturbed best response defined as follows:  %Further, the fraction of flow leaving link $i$ at step $n$ is $\outflow_i(n)$, and $\{\outflow_i(n)\}_{n \in N}$ are i.i.d. as well, with a finite mean $\avg[\outflow_i(n)] = \meanOutflow \in (0,1)$. We also assume that $\inflow_i(n)$ and $\outflow_i(n)$ have bounded support. Specifically, for every \(i\in[\numLinks]\) and       \(n\in\N\), \(\inflow(n) \in [\inflowLower,\inflowUpper]\) almost surely and \(\outflow_i(n) \in [\outflowLower,\outflowUpper]\) almost surely. Moreover \(\outflowLower > 0\) and \(\outflowUpper < 1\).
  
  %The demand at the source node is allocated to different links in accordance to the allocations under \emph{stochastic user equilibrium}. Stochastic user equilibrium is a commonly used routing paradigm that captures the behavioral aspect of traveller's decision making in response to stochastic perception of travel cost associated with different links. 
 \begin{definition}\label{assm: InflowAssumption}(\textbf{Perturbed Best Response Strategy})
  At any step \(n+1\), the routing strategy $\flowIn_i(n+1)$ is \emph{perturbed best response} if for all \(i\in[\numLinks]\),
  \begin{align}\label{eq: InflowEquation}
     \flowIn_i(n+1) \defas \frac{\exp(-\sueParameter \costPrice_i(\flowDiscrete_i(n), \priceDiscrete_i(n)))}{\sum_{j\in[R]}\exp(-\sueParameter \costPrice_j(\flowDiscrete_j(n), \priceDiscrete_j(n)))}\inflow(n),  
 \end{align}
 where $\beta \in [0, \infty)$. 
  \end{definition}
  
  
The perturbed best response strategy reflects the myopic nature of travelers route choices. In particular, $\sueParameter$ is a dispersion parameter that governs the relative weight of link costs in making routing decisions. If $\beta \uparrow \infty$, $\flowIn_i(n+1)$ is a best response strategy in that travelers only take links with the minimum cost in $\flowIn_i(n+1)$. On the other hand, if $\beta\downarrow 0$, then $\flowIn_i(n+1)$ assigns the arrival demand uniformly across all links.  
 
%Here, The parameter $\sueParameter$ characterizes the relative weight the load assigns between higher and lower cost links, and will be referred as the \textit{dispersion parameter}. We define \(\mc{I}_{\min}(n)\defas\{j:\costPrice_j(\flowDiscrete_i(n),\priceDiscrete_i(n)) =  \min_k\costPrice_k(\flowDiscrete_k(n),\priceDiscrete_k(n))\}\). As $\sueParameter \uparrow \infty$, $\flowIn_i(n+1) =\frac{\inflow(n)}{|\mc{I}_{\min}(n)|}$ for all \(i\in \mc{I}_{\min}(n)\) and $\flowIn_i(n+1) = 0$ for all $i \not\in\mc{I}_{\min}(n)$. However, as $\sueParameter \downarrow 0$, the incoming loads  $\flowIn_i(n+1) = \flowIn_j(n+1)$ for all $i,j$. 
  
  
%route choice model represents a \emph{myopic, selfish}, and \textit{perturbed} best-response strategy for routing incoming load, for $\beta$ finite and nonzero. According to this choice model, the links with lower cost is chosen by a larger fraction of incoming load, but the load experiences a perturbed version of the cost. That is, the load experiences $\tilde{\costPrice}_i = \costPrice_i + \nu_i$ on each link. As $\beta \uparrow \infty$, the experienced perturbation $\nu_i$ reduces, and the incoming load chooses only the links with lowest cost, in a sense we make formal in Lemma \ref{lemma:gStochasticEquilibrium}.

  
Furthermore, the proportion of load discharged from link \(i\in[\numLinks]\) at step \(n+1\) is given by the random variable \(\outflow_i(n+1) \in (0,1)\). We assume that \(\{\outflow_i(n)\}_{i\in[\numLinks],n\in\N}\) are i.i.d. with bounded support \([\outflowLower,\outflowUpper]\) and mean \(\meanOutflow\) (i.e. \(\avg[\outflow_i(n)] = \mu\) for all \(i\in[\numLinks]\)). Thus the load discharged from link \(i\in[\numLinks]\) at step \(n+1\) is given by \begin{align}\label{eq:outflow}
    \flowOut_i(n+1) \defas \flowDiscrete_i(n)\outflow_i(n+1).
\end{align}
  


In each step $n$, the load on each link is updated as follows: %We characterize the evolution of the load on each link in the network by the following discrete-time stochastic : for every \(i\in[\numLinks]\),
\begin{align}\label{eq:x_original}
    \flowDiscrete_i(n+1) &= \flowDiscrete_i(n) +  \flowIn_i(n+1) - \flowOut_i(n+1) .
\end{align}
We note that the stochasticity of the load update arises from the randomness in the incoming load $\flowIn(n+1)$ and the outgoing load $\flowOut(n+1)$. We define 
\begin{align}\label{eq: hVectorFieldDef}
\vectorFieldX_i(x_i,p_i) \defas \frac{\meanInflow}{\meanOutflow}\frac{\exp(-\sueParameter \costPrice_i(x_i,p_i))}{\sum_{j\in[R]}\exp(-\sueParameter \costPrice_j(x_j,p_j))}. 
\end{align}
where $x, p \in \mathbb{R}^{\numLinks}$, and $\meanInflow$ (resp. $\meanOutflow$) is the mean of incoming (resp. outgoing) load respectively.
Using \eqref{eq: InflowEquation}, \eqref{eq:outflow}, and \eqref{eq: hVectorFieldDef}, we can re-write \eqref{eq:x_original} as follows: 
\begin{equation}\tag{Update-$\flowDiscrete$}\label{eq: FlowDynamics}
\begin{aligned}
    \flowDiscrete_i(n+1)
    %&=  \flowDiscrete_i(n) + \frac{\exp(-\sueParameter \costPrice_i(\flowDiscrete_i(n), \priceDiscrete_i(n)))}{\sum_{j\in[R]}\exp(-\sueParameter \costPrice_j(\flowDiscrete_j(n), \priceDiscrete_j(n)))}\inflow(n) \\&\hspace{2cm} -  \flowDiscrete_i(n)\outflow_i(n);\\
    &=(1-\meanOutflow) \flowDiscrete_i(n) + \meanOutflow \vectorFieldX_i(\flowDiscrete_i(n), \priceDiscrete_i(n)) + \meanOutflow\martingale_i(n+1),
\end{aligned}
\end{equation}
where
\begin{equation}
\begin{aligned}\label{eq: MartingaleDefinition}
\martingale_i(n+1)  & \defas   \vectorFieldX_i(\flowDiscrete_i(n), \priceDiscrete_i(n))(\inflow(n+1) - \meanInflow) \\ &\quad - \flowDiscrete_i(n)\lr{\outflow_i(n+1)- \meanOutflow}. 
\end{aligned}
\end{equation}


%The advantage of latter version of flow update is that it allows us to think about \(\meanOutflow\) as a step size.

The central authority updates the toll vector $\priceDiscrete(n) \in \mathbb{R}^{\numLinks}$ at each step $n$ as follows: 
\begin{align}\tag{Update-$\priceDiscrete$}\label{eq: PricingDynamics}
\priceDiscrete_i(n+1) = (1-a)\priceDiscrete_i(n) + a \flowDiscrete_i(n)\frac{d \costEdge_i(\flowDiscrete_i(n))}{d x}%\frac{\partial \costPrice_i(\flowDiscrete_i(n), \priceDiscrete_i(n)) }{\partial x}
\end{align}
where \( i \in [\numLinks], n\in \N\) and \(a\in [0, 1]\) is the step size.
That is, the updated toll is an interpolation between the current toll and the \emph{marginal cost} of the link given the current load. We note that the toll is updated in a distributed manner in that $\priceDiscrete_i(n+1)$ only depends on the load and cost on link $i$. %So, the tolls are updated in a \emph{distributed} manner (i.e. toll update on any link $i$ depends only on information corresponding to that link).  

%As we posited in Equation \eqref{eq: costAssumption}, the tolls and latency additively realize the total cost on any link. That is, for every \(i\in[\numLinks]\), $\costPrice_i(\flowDiscrete_i(n), \priceDiscrete_i(n))= \latency(\flowDiscrete_i(n)) + \priceDiscrete_i(n)$. We note that in on static routing \cite{roughgarden2010algorithmic}, marginal cost prices also enter the cost functions of every link additively. This ensures that the prices $\priceDiscrete_i(n)$ can be designed with the marginal cost on link $i$ at time $n$ to steer the system to social optimality. 

The updates of $(\flowDiscrete(n), \priceDiscrete(n))$ are jointly governed by the stochastic updates in \eqref{eq: FlowDynamics} and \eqref{eq: PricingDynamics}. We assume that tolls are updated at a slower timescale compared with the load. That is, \(a \ll \meanOutflow\), where $a$ (resp. $\meanOutflow$) is the step size in \eqref{eq: PricingDynamics} (resp. \eqref{eq: FlowDynamics}). % on a \textit{slower} time-scale than the load dynamics. That is, . A slow toll update has been noted as a desirable feature of dynamic routing schemes as it gives the load appropriate time to respond \cite{farokhi2015piecewise}. 
%For later reference, we present below the combined discrete-time stochastic load and toll update:
% \begin{equation}\label{eq: CombinedDT}
%     \begin{aligned}
%       \flowDiscrete_i(n+1) & =\flowDiscrete_i(n) + \meanOutflow\lr{\vectorFieldX_i(\flowDiscrete_i(n), \priceDiscrete_i(n))- \flowDiscrete_i(n)}  + \meanOutflow\martingale_i(n+1),\\
%      \priceDiscrete_i(n+1) & = (1-a)\priceDiscrete_i(n) + a \flowDiscrete_i(n)\frac{\partial \costEdge_i(\flowDiscrete_i(n))}{\partial x}.
%     \end{aligned}
% \end{equation}

% This model follows a class of dynamics in the spirit of \cite{borkar2009cooperative} and \cite{pietrabissa2018discrete}. In particular, we note that the dynamic is distinguished from classical dynamics in routing games (gradient descent, multiplicative weights, etc.) in that it explicitly accounts for the inflow and outflow of vehicles through a conservation law.


\color{black}
% \textcolor{red}{
% \begin{itemize}
%     \item \sout{Introduce tolls in the beginning. Add toll prices in the cost function when it is first introduced in route choices rather than later }
%     \item \sout{Rephrase "assumptions" as setups, and put them in line}
%     \item \sout{You need to introduce two timescale here, and justify it}
%     \item Put technical parts in the technical section 
%     \item Avoid loose English and casual use of terminologies that you don't define 
%     \item \sout{Name the dynamics as X-update, p-update (or something else that makes sense to you). It is easier for readers to remember them since they are referred repeatedly throughout}
% \end{itemize}}

==> Dynamic_Routing_Regular (Arxiv)/proofs_Arxiv.tex <==
\section{Proofs}\label{appsec: ProofLemma}
\subsection{{Proof of Lemma \ref{lemma:gStochasticEquilibrium}}}
In the subsequent proof we shall show that the following claims hold: 

\begin{enumerate}[label= (C-\Roman*),widest=ii,leftmargin=*,align=left]
    \item \label{thm: claim1} For any \(p\in\R^{\numLinks}\), the optimizer of \eqref{eq: OptimizationProblemRevised} is unique; call it \(y^\star(p)\);
    \item \label{thm: claim2} \(y^\star(p)\) is an optimal solution if and only if it satisfies \(h(y^\star(p),p) = y^\star\)
\end{enumerate}
Note that the above two claims ensure that \(\fixedPointFlow(p) = y^\star(p)\). The subsequent exposition establishes the validity of these claims.

To see that \ref{thm: claim1}  is true, we note that the feasible set of \eqref{eq: OptimizationProblemRevised} is a compact convex set.  Moreover, from the convexity of $\costEdge$ it follows that \(
    \sum_{i\in [\numLinks]} \int_{0}^{y_i} \costPrice_i(s,p_i)ds + \frac{1}{\beta} \sum_{i\in [\numLinks]} y_i \ln{y_i}
\) is a strictly convex function in \(y\). Strict convexity ensures the uniqueness of solution of a convex optimization problem on a convex compact set \cite{boyd2004convex}.

For \ref{thm: claim2}, we now employ KKT conditions of optimality: let \(\delta\in\R \) be the Lagrange multiplier corresponding to the equality constraint. Define the  Lagrangian as follows:
\[
L(y,\delta,p) \defas \sum_{i\in [\numLinks]} \int_{0}^{y_i} \costPrice_i(s,p_i)ds + \frac{1}{\beta} \sum_{i\in \numLinks} y_i \ln{y_i} + \delta \lr{\sum_{i\in[\numLinks]} y_i - \frac{\meanInflow}{\meanOutflow}}
\]

The optimal solution $y^{\star}(p)$ and Lagrange multiplier $\delta^\star$ satisfy: \begin{enumerate}[widest=ii,leftmargin=*,align=left]
    \item \(\nabla_{y}L(y^{\star}(p),\delta^{\star},p) = 0\). This gives us \(\costPrice_i(y_i^{\star}(p),p_i) + \frac{1}{\beta}\lr{1+\ln(y_i^{\star}(p))} +\delta^{\star} = 0\), which can be also written as follows
    \begin{align}
    \label{eq: Opt_y}
    y_i^{\star}(p) = \exp(-\beta \delta^\star-1)\exp(-\beta \costPrice_i(y_i^{\star}(p),p_i)), \quad \forall \ i\in[\numLinks].
    \end{align}
    \item \(\nabla_\delta L(y^{\star}(p),\delta^{\star},p) = 0\). That is, 
    \(
    \sum_{i\in \numLinks} y_i^{\star}(p)  = \frac{\meanInflow}{\meanOutflow}.
    \)
    \end{enumerate}
    From \eqref{eq: Opt_y}, summing over \(i\in[\numLinks]\) on both the sides, we obtain 
    \[
    \frac{\meanInflow}{\meanOutflow} = \exp(-\beta \delta^\star -1 ) {\sum_{i\in[\numLinks]}\exp(-\beta \costPrice_i(y_i^{\star}(p),p_i))}
    \]

The above conditions give us that \(y^\star(p)\) is an optimal solution of \eqref{eq: OptimizationProblemRevised} if and only if it satisfies
\[
y_i^\star(p) = \frac{\meanInflow}{\meanOutflow} \frac{\exp(-\beta \costPrice_i(y_i^\star(p),p_i))}{\sum_{i\in[\numLinks]}\exp(-\beta \costPrice_i(y_i^\star(p),p_i))} = \vectorFieldX_i(y^\star(p),\priceContinuous), \quad \forall \ i\in[\numLinks].
\]

\subsection{Proof of Lemma \ref{lemma:monotonicity}}
Before proving Lemma \ref{lemma:monotonicity}, we will first state the following result that will be useful later. 

 Define \(\diagC(x) \defas \diag\lr{\lr{\frac{d \costEdge_i(x)}{dx}}_{i=1}^{\numLinks}} \) and \(\diagMarginal(x) \defas \diag\lr{\lr{x_i\frac{d \costEdge_i(x)}{dx}}_{i=1}^{\numLinks}}\).
\begin{lemma}\label{lem: LipschitzFunction}
The function $h(x,p)$ presented in \eqref{eq: hVectorFieldDef} is Lipschitz in \(x\) and \(p\) and satisfies:
\begin{align}
    \grad_x \vectorFieldX(\fixedPointFlow(p),p) = \frac{\meanInflow}{\meanOutflow}\beta\fixedPointFlow(p)\fixedPointFlow(p)^\top \diagC(\fixedPointFlow(p)) - \beta\diagMarginal\lr{\fixedPointFlow(p)} 
\end{align}
\end{lemma}
\begin{proof}[Proof of Lemma \ref{lem: LipschitzFunction}]
To show that the function is Lipschitz, it is sufficient to show that the norm of the gradient of this function is bounded. This is due to the first order Taylor expansion of the function. 

Therefore, for every \(i\in[\numLinks]\) we first compute \(\grad_x h_i(x,p)\) entrywise as follows: 
\begin{equation}\label{eq: xDerivative}
\begin{aligned}
\frac{\partial h_i(x,p)}{\partial x_j} = \begin{cases}  \frac{\meanInflow}{\meanOutflow} \frac{-\beta\frac{d\costEdge_i(x_i)}{dx}\sum_{k\in[R]}\exp(-\sueParameter \costPrice_k(x_k,p_k))  \exp(-\beta \costPrice_i(x_i,p_i)) +\beta\frac{d\costEdge_i(x_i)}{dx} \lr{\exp(-\beta \costPrice_i(x_i,p_i))}^2 }{\lr{\sum_{k\in[R]}\exp(-\sueParameter \costPrice_k(x_k,p_k)) }^2} & \text{if}\ \ i=j;\\
\frac{\meanInflow}{\meanOutflow}\beta\frac{d\costEdge_j(x_j)}{dx}\exp(-\beta \costPrice_i(x_i,p_i))\frac{\exp(-\beta \costPrice_j(x_j,p_j))}{\lr{\sum_{k\in[R]}\exp(-\sueParameter \costPrice_k(x_k,p_k)) }^2} & \text{otherwise}
\end{cases}
\end{aligned}
\end{equation}
Evaluating the above derivative at \(\fixedPointFlow(p)\)
\begin{equation}\label{eq: xDerivativeFP}
\begin{aligned}
\frac{\partial h_i(\fixedPointFlow(p),p)}{\partial x_j} = \begin{cases}  \beta \frac{d \costEdge_i(\fixedPointFlow_i(p))}{dx} \lr{ -\fixedPointFlow_i(p) +\frac{\meanOutflow}{\meanInflow}\lr{\fixedPointFlow_i(p)}^2 } & \text{if}\ \ i=j;\\
\frac{\meanOutflow}{\meanInflow}\beta\frac{d\costEdge_j(\fixedPointFlow_j(p))}{dx}\fixedPointFlow_i(p)\fixedPointFlow_j(p) & \text{otherwise}
\end{cases}
\end{aligned}
\end{equation}
To state it concisely:
\begin{align}\label{eq: GradHEq}
\grad_x \vectorFieldX(\fixedPointFlow(p),p) = \frac{\meanInflow}{\meanOutflow}\beta\fixedPointFlow(p)\fixedPointFlow(p)^\top \diagC(\fixedPointFlow(p)) - \beta\diagMarginal\lr{\fixedPointFlow(p)} 
\end{align}
Similarly, 
\begin{equation}\label{eq: pDerivative}
\begin{aligned}
\frac{\partial h_i(x,p)}{\partial p_j} = \begin{cases}  \frac{\meanInflow}{\meanOutflow} \frac{-\beta\sum_{k\in[R]}\exp(-\sueParameter \costPrice_k(x_k,p_k))  \exp(-\beta \costPrice_i(x_i,p_i)) +\beta \lr{\exp(-\beta \costPrice_i(x_i,p_i))}^2 }{\lr{\sum_{k\in[R]}\exp(-\sueParameter \costPrice_k(x_k,p_k)) }^2} & \text{if}\ \ i=j;\\
\frac{\meanInflow}{\meanOutflow}\beta\exp(-\beta \costPrice_i(x_i,p_i))\frac{\exp(-\beta \costPrice_j(x_j,p_j))}{\lr{\sum_{k\in[R]}\exp(-\sueParameter \costPrice_k(x_k,p_k)) }^2} & \text{otherwise}
\end{cases}
\end{aligned}
\end{equation}
To conclude the proof we observe that on a bounded domain the derivative in \eqref{eq: xDerivative} and \eqref{eq: pDerivative} are bounded. 
\end{proof}

\subsubsection{\textbf{Proof of Lemma \ref{lemma:monotonicity}}}
Recall from the proof of Lemma \ref{lemma:gStochasticEquilibrium} (\ref{thm: claim2} to be precise) that for any \(p\in\R^{\numLinks}\), \(\fixedPointFlow(p)\) is a solution to the optimization problem \eqref{eq: OptimizationProblemRevised}. Let the feasible set in the optimization problem \eqref{eq: OptimizationProblemRevised} be denoted by \(F\). Using first order conditions for constrained optimization we obtain the variational inequality: 
\begin{align}\label{eq: ConstrainedOptimalityP}
    \sum_{i\in[\numLinks]} \lr{\costPrice_i\lr{\fixedPointFlow_i(p),p} + \frac{1}{\beta}\lr{\ln\lr{\fixedPointFlow_i(p)}+1}}\lr{x_i-\fixedPointFlow_i(p)} \geq0 \quad \forall x \in F.
\end{align}
Similarly writing the above condition for \(p'\), we obtain \begin{align}\label{eq: ConstrainedOptimalityPD}
    \sum_{i\in[\numLinks]} \lr{\costPrice_i\lr{\fixedPointFlow_i(p'),p'} + \frac{1}{\beta}\lr{\ln\lr{\fixedPointFlow_i(p')}+1}}\lr{y_i-\fixedPointFlow_i(p')} \geq0 \quad \forall y \in F.
\end{align}
Choosing \(x=\fixedPointFlow(p')\)  in \eqref{eq: ConstrainedOptimalityP} and \(y=\fixedPointFlow(p)\) in \eqref{eq: ConstrainedOptimalityPD} and adding the two equations we obtain
\begin{align*}
    &\sum_{i\in[\numLinks]} \lr{ \costPrice_i(\fixedPointFlow_i(p),p)-\costPrice_i(\fixedPointFlow_i(p'),p')}\lr{\fixedPointFlow_i(p')-\fixedPointFlow_i(p)} \\ &\quad \quad +\sum_{i\in[\numLinks]} \lr{ \frac{1}{\beta} \ln(\fixedPointFlow_i(p))-\ln(\fixedPointFlow_i(p')) }\lr{\fixedPointFlow_i(p')-\fixedPointFlow_i(p)} \geq 0.
\end{align*}
From the fact that prices enter additively, we have 
\begin{align*}
    &\sum_{i\in[\numLinks]} \lr{ \costEdge_i(\fixedPointFlow_i(p))-\costEdge_i(\fixedPointFlow_i(p'))}\lr{\fixedPointFlow_i(p')-\fixedPointFlow_i(p)}\\ &\quad\quad + \sum_{i\in[\numLinks]} \lr{ p_i-p_i'+ \frac{1}{\beta} \ln(\fixedPointFlow_i(p))-\ln(\fixedPointFlow_i(p')) }\lr{\fixedPointFlow_i(p')-\fixedPointFlow_i(p)} \geq 0.
\end{align*}
This gives 
\begin{align*}
    &\lara{\fixedPointFlow(p)-\fixedPointFlow(p'),p-p'} \\&\leq \lara{\costEdge(\fixedPointFlow(p))-\costEdge(\fixedPointFlow(p')),\fixedPointFlow(p')-\fixedPointFlow(p)}\\&\quad +\frac{1}{\beta} \lara{ \ln(\fixedPointFlow(p)) - \ln(\fixedPointFlow(p')), \fixedPointFlow(p')-\fixedPointFlow(p)}\\
&< 0,
\end{align*}
where the last inequality follows due to the monotonicity of the cost function and natural logarithm.

 Next, we show that $\fixedPointFlow(\priceContinuous)$ is a differentiable function of $\priceContinuous$.  Recall the notation \(\diagC(x) \defas \diag\lr{\lr{\frac{d \costEdge_i(x)}{dx}}_{i=1}^{\numLinks}} \) and \(\diagMarginal(x) \defas \diag\lr{\lr{x_i\frac{d \costEdge_i(x)}{dx}}_{i=1}^{\numLinks}}\).

 To show the differentiability of \(\fixedPointFlow(p)\) with respect to \(p\), we invoke the implicit function theorem for the map $\fixedGap(x, p) = x - h(x, p)$.
Note that for any fixed \(p\), \(\fixedPointFlow(p)\) is the zero of \(\fixedGap(\cdot,p)\). To satisfy the hypothesis for the implicit function theorem, for any \(\priceContinuous\) we compute the Jacobian of the function $\fixedGap(x, p)$ with respect to \(x\) and evaluate it at $\fixedPointFlow(\priceContinuous)$. Using Lemma \ref{lem: LipschitzFunction} the Jacobian is given by: 
\begin{align*}
   \grad_x \fixedGap(\fixedPointFlow(p),p) &= I - \grad_x \vectorFieldX(\fixedPointFlow(p),p) \\
   & = I - \frac{\meanOutflow}{\meanInflow}\beta\fixedPointFlow(p)\fixedPointFlow(p)^\top \diagC(\fixedPointFlow(p)) + \beta\diagMarginal\lr{\fixedPointFlow(p)} \\ 
   & = \lr{\lr{\diagMarginal^{-1}(\fixedPointFlow(p)) + \beta I}-\beta v\mathbbm{1}^\top}\diagMarginal(\fixedPointFlow(p)) 
\end{align*}
where \(v \defas \frac{\meanOutflow}{\meanInflow}\fixedPointFlow(p)\). Note that from \eqref{eq: xEquilibrium} we have \(\mathbbm{1}^\top v = 1\).
We claim that \(\det(\grad_x \fixedGap(\fixedPointFlow(p),p)) \neq 0\). Indeed, 
\begin{align*}
    \det(\grad_x \fixedGap(\fixedPointFlow(p),p)) &= \det\lr{\diagMarginal(\fixedPointFlow(p)} \det\lr{\lr{\diagMarginal^{-1}(\fixedPointFlow(p)) + \beta I}-\beta v\mathbbm{1}^\top }\\ 
   &= \det\lr{\diagMarginal(\fixedPointFlow(p)}\cdot
    \det\lr{I-\beta v\mathbbm{1}^\top\lr{\diagMarginal^{-1}(\fixedPointFlow(p)) + \beta I}^{-1} }\\&\quad\quad \cdot \det\lr{\diagMarginal^{-1}(\fixedPointFlow(p)) + \beta I}^{-1}
\end{align*}
It is sufficient to show that \( \det\lr{I-\beta v\mathbbm{1}^\top\lr{\diagMarginal^{-1}(\fixedPointFlow(p)) + \beta I}^{-1} }\neq 0\). Using the Sherman-Morrison formula \cite{gentle2007matrix} it is necessary and sufficient to show that \(\beta\mathbbm{1}^\top\lr{\diagMarginal^{-1}(\fixedPointFlow(p)) + \beta I}^{-1} v \neq 1 \). 

We show it by contradiction. Suppose \(\beta\mathbbm{1}^\top\lr{\diagMarginal^{-1}(\fixedPointFlow(p)) + \beta I}^{-1} v = 1 \). Then 
\begin{align*}
&\implies \quad \sum_{i=1}^{\numLinks} v_i \frac{\beta}{\frac{1}{m_i}+\beta} = 1\\
&\implies \quad \sum_{i=1}^{\numLinks} v_i \frac{\beta}{\frac{1}{m_i}+\beta} = \sum_{i=1}^{\numLinks} v_i \\ 
&\implies \sum_{i=1}^{\numLinks} v_i\frac{\frac{1}{m_i}}{\beta+\frac{1}{m_i}} = 0
\end{align*}
This is not possible as the terms on the left hand side are all positive. 


The claim that \(\frac{\partial \fixedPointFlow_i(\priceContinuous)}{\partial \priceContinuous_i} < 0\) also follows from the monotonicity of \(\fixedPointFlow(\priceContinuous)\). Indeed, if we choose two price profiles that differ only at one index then the monotonicity property of \(\fixedPointFlow(p)\) ensures \(\frac{\partial \fixedPointFlow_i(\priceContinuous)}{\partial \priceContinuous_i} < 0\). 
This completes the proof.
\subsection{Proof of Lemma \ref{lemma:unique_price}}
We shall first show the existence and then prove the uniqueness of \(\fixedPointPrice\). 

For any \(p\in\R^{\numLinks}, i\in[\numLinks]\), define \(z_i(p) = \fixedPointFlow(p)\frac{d \costEdge_i(\fixedPointFlow_i(p))}{dx}\). The equilibrium price \(\fixedPointPrice\) is then solution to the fixed point equation \(p=z(p)\) where $z(p) = [z_i(p)]_{i\in [\numLinks]}$.  Define a set \(K = \{y\in\R^{\numLinks}: y\geq 0, \|y\|_1 \leq \frac{\meanInflow}{\meanOutflow}\max_{i\in[\numLinks]}\frac{d c_i\lr{\frac{\meanInflow}{\meanOutflow}}}{dx}\}\). Observe that \(z(\cdot)\) maps the convex compact set \(K\) to itself. Therefore, Brouwer's fixed point theorem \cite{sastry2013nonlinear} guarantees the existence of fixed point \(\fixedPointPrice\).



Now, we prove the uniqueness of the fixed point $\fixedPointPrice$ satisfying \eqref{eq: pEquilibrium}.  
We shall prove this via a contradiction argument. Assume that there are two distinct price profiles $\fixedPointPrice, \fixedPointPrice' \in \R^{\numLinks}$ that both satisfy the fixed point equation \eqref{eq: pEquilibrium}, therefore for every \(i\in[\numLinks]\):
\begin{align*}
    \fixedPointPrice_i &= \fixedPointFlow_i(\fixedPointPrice) \frac{d \costEdge_i(\fixedPointFlow_i(\fixedPointPrice))}{dx} \\ \fixedPointPrice_i' &= \fixedPointFlow_i(\fixedPointPrice') \frac{d \costEdge_i(\fixedPointFlow_i(\fixedPointPrice'))}{dx}
\end{align*}
Taking the difference we get 
\begin{align*}
    \fixedPointPrice_i - \fixedPointPrice_i' &= \fixedPointFlow_i(\fixedPointPrice) \frac{d \costEdge_i(\fixedPointFlow_i(\fixedPointPrice))}{dx} - \fixedPointFlow_i(\fixedPointPrice') \frac{d \costEdge_i(\fixedPointFlow_i(\fixedPointPrice'))}{dx} , \\ 
    &= \fixedPointFlow_i(\fixedPointPrice) \frac{d \costEdge_i(\fixedPointFlow_i(\fixedPointPrice))}{dx} - \fixedPointFlow_i(\fixedPointPrice') \frac{d \costEdge_i(\fixedPointFlow_i(\fixedPointPrice))}{dx}\\
    &\quad \quad \quad + \fixedPointFlow_i(\fixedPointPrice') \frac{d \costEdge_i(\fixedPointFlow_i(\fixedPointPrice))}{dx} - \fixedPointFlow_i(\fixedPointPrice') \frac{d \costEdge_i(\fixedPointFlow_i(\fixedPointPrice'))}{dx},  \\
    &= \lr{\fixedPointFlow_i( \fixedPointPrice)-\fixedPointFlow_i(\fixedPointPrice')}   \frac{d\costEdge_i(\fixedPointFlow_i(\fixedPointPrice))}{dx}\\&\quad\quad\quad +\fixedPointFlow_i(\fixedPointPrice')\lr{\frac{d \costEdge_i(\fixedPointFlow_i(\fixedPointPrice))}{dx}-\frac{d \costEdge_i(\fixedPointFlow_i(\fixedPointPrice'))}{dx}},
\end{align*}
for every \(i\in[\numLinks]\). Multiplying \((\fixedPointFlow_i(\fixedPointPrice)-\fixedPointFlow_i(\fixedPointPrice'))\) in the preceding equation we obtain
\begin{equation}
\begin{aligned}\label{eq: pUniquenessContradiction}
    &(\fixedPointFlow_i(\fixedPointPrice)-\fixedPointFlow_i(\fixedPointPrice'))(\fixedPointPrice_i - \fixedPointPrice_i') = \lr{\fixedPointFlow_i(\fixedPointPrice)-\fixedPointFlow_i(\fixedPointPrice')}^2\frac{d \costEdge_i(\fixedPointFlow_i(\fixedPointPrice))}{dx}\\&\quad\quad\quad +\fixedPointFlow_i(\fixedPointPrice') \lr{\frac{d \costEdge_i(\fixedPointFlow_i(\fixedPointPrice))}{dx}-\frac{d \costEdge_i(\fixedPointFlow_i(\fixedPointPrice'))}{dx}} (\fixedPointFlow_i(\fixedPointPrice)-\fixedPointFlow_i(\fixedPointPrice')), 
\end{aligned}
\end{equation}
for every \(i\in[\numLinks]\). Convexity of the edge cost function ensures that right hand side of \eqref{eq: pUniquenessContradiction} is always non-negative for every \(i\in[\numLinks]\). 
Summing over \(i\in[R]\) and using Lemma \ref{lemma:monotonicity} we obtain:
\begin{align*}
    0>\lara{ \fixedPointFlow_i(\fixedPointPrice)-\fixedPointFlow_i(\fixedPointPrice'), \fixedPointPrice-\fixedPointPrice' } \geq 0.
\end{align*}
which contradicts our original hypothesis that there are two distinct price profiles satisfying \eqref{eq: pEquilibrium}. 

\subsection{Proof of Lemma \ref{lemma:optimality}}
% Let's denote the flow under static Wardrop equilibrium and price \(p\) by \(\flowWardrop(p)\). The proof follows by observing that for any \(p\in\R^{\numLinks}\) and \(\beta>0\), \(\fixedPointFlow(p)\) is the unique solution to the convex optimization problem \eqref{eq: OptimizationProblemRevised} as is presented in Lemma \ref{lemma:gStochasticEquilibrium}. In the optimization problem \eqref{eq: OptimizationProblemRevised} as \(\beta\uparrow +\infty\) the effect of entropy regularization diminishes and the resulting optimization program is the one that characterizes Wardrop equilibrium \cite[p. 214]{cominetti2012modern}. That is \(\fixedPointFlow(\cdot) \ra \flowWardrop(\cdot)\) as \(\beta\uparrow+\infty\) in a pointwise sense.  
Note that for any \(i\in[\numLinks]\)
\begin{align}\label{eq: PriceBeta}
    \fixedPointPrice_i = \fixedPointFlow_i(\fixedPointPrice) \frac{d \costEdge_i(\fixedPointFlow_i(\fixedPointPrice))}{dx}
\end{align}

Let 
\begin{align*}
   x^\star = \argmin_{y\in F} \lr{ \sum_{i\in[\numLinks]} y_i\costEdge_i(y_i) + \frac{1}{\beta}\sum_{i\in[\numLinks]} y_i\log(y_i)},
\end{align*}
where \(F= \{y: \sum_{i\in[\numLinks]}y_i = \frac{\meanInflow}{\meanOutflow}\}\) is the feasible set. We claim that \(x^\star =  \fixedPointFlow(\fixedPointPrice)\).

To show this claim, we first note that the above problem is a strictly convex optimization problem. The necessary and sufficient conditions for constrained optimality ensures that for any \(y\in F\): 
\begin{align}\label{eq: SocialCostFirst}
    \sum_{i\in[\numLinks]} \lr{ \costEdge_i(x^\star_i) + x_i^\star\frac{d\costEdge_i(x_i^\star)}{dx} + \frac{1}{\beta} \lr{1+\log(x_i^\star)}}\lr{ y_i-x_i^\star} \geq 0. 
\end{align}

Now recall that \(\fixedPointFlow(\fixedPointPrice)\) satisfies 
\begin{align*}
    \fixedPointFlow(\fixedPointPrice) = \argmin_{y\in F} \sum_{i\in[\numLinks]} \int_{0}^{y_i}\lr{\costEdge_i(z)+\fixedPointPrice_i } \textsf{d}z+\frac{1}{\beta}\sum_{i\in[\numLinks]} y_i\log(y_i).
\end{align*}
Note that we have already noted in proof of Lemma \ref{lemma:gStochasticEquilibrium} that the above optimization problem is strictly convex. The constrained optimality conditions ensure that for any \(y\in F\):
\begin{align}\label{eq: SelfishCostFirst}
    \sum_{i\in[\numLinks]}\lr{\costEdge_i(\fixedPointFlow_i(\fixedPointPrice)) + \fixedPointPrice_i + \frac{1}{\beta} \lr{1+\log(\fixedPointFlow_i(\fixedPointPrice))}}\lr{y_i-\fixedPointFlow_i(\fixedPointPrice)} \geq 0. 
\end{align}
Note that using \eqref{eq: PriceBeta} in \eqref{eq: SelfishCostFirst} we obtain that for any \(y\in F\): 
\begin{align}\label{eq: SocialCostSecond}
    \sum_{i\in[\numLinks]}\lr{\costEdge_i(\bar{x}) + \bar{x}_i \frac{d \costEdge_i(\bar{x}_i)}{dx} + \frac{1}{\beta} \lr{1+\log(\bar{x}_i)}}\lr{y_i-\bar{x}_i} \geq 0, 
\end{align}
where we have used \(\bar{x} = \fixedPointFlow(\fixedPointPrice)\) to simplify the expression. Comparing expression \eqref{eq: SocialCostFirst} and \eqref{eq: SocialCostSecond} we conclude that \(x^\star =\fixedPointFlow(\fixedPointPrice) \). This concludes the proof. 

\subsection{Proof of Lemma \ref{lemma: prep}}
We prove the claims in the lemma sequentially. 

Proof of \textbf{(C1)}: Using the independence of sequence \(\inflow(n),\outflow_i(n)\) we see that the conditional expection of \(\martingale_i(n+1)\) conditioned on the filtration \(\mc{F}_n\) is zero. That is, 
\begin{align*}
    \avg[\martingale_i(n+1)|\mc{F}_n] = \vectorFieldX_i(\flowDiscrete_i(n),\priceDiscrete_i(n)) \lr{\avg[\inflow(n+1)]-\meanInflow} - \flowDiscrete_i(n)\lr{\avg[\outflow_i(n+1)-\meanOutflow]} = 0.
\end{align*}

Proof of \textbf{(C2)}: Recall that we assume that the incoming loads and outgoing fraction have finite support. That is, for every \(i\in[\numLinks]\) and \(n\) we have \(\inflow(n)\in[\inflowLower,\inflowUpper] \subset (0,\infty)\) and \(\outflow_i(n)\in[\outflowLower, \outflowUpper] \subset (0,1)\). Note that \(X_i(0)\geq 0\) for all \(i\in [\numLinks]\) as it is impractical to have negative load on the network; therefore our update reflects the physical constraints of the network. Under this assumption, the discrete-time stochastic update \eqref{eq:x_original} can be written as 
\begin{align*}
    \flowDiscrete_i(n+1) &= (1-\outflow(n+1))\flowDiscrete_i(n) +  \frac{\exp(-\sueParameter \costPrice_i(\flowDiscrete_i(n), \priceDiscrete_i(n)))}{\sum_{j\in[R]}\exp(-\sueParameter \costPrice_j(\flowDiscrete_j(n), \priceDiscrete_j(n)))}\inflow(n),  \\
    &\leq (1-\outflowLower)\flowDiscrete_i(n)+ \inflow(n), \\ 
    &\leq (1-\outflowLower)\flowDiscrete_i(n) + \inflowUpper, \\
    &\leq (1-\outflowLower)^n\flowDiscrete_i(0)+\frac{\inflowUpper}{\outflowLower}.
\end{align*}
The preceding inequalities establish that \(\avg[\|\flowDiscrete_i(n)\|^2]<+\infty\). Consequently, it also ensure that \(\avg\left[ X_i(n)\frac{d \latency_i(n)}{dx}\right] < +\infty\) and is independent of \(n\), which in turn, from \eqref{eq: PricingDynamics} leads to \(\avg[\|P_i(n)\|^2] < +\infty\). 

Proof of \textbf{(C3)}: We see that:
\begin{align*}
    \avg[|\martingale_i(n+1)|^2|\filtration_n] & = \avg[|\vectorFieldX_i(\flowDiscrete_i(n), \priceDiscrete_i(n))(\inflow(n+1) - \meanInflow) - \flowDiscrete_i(n)\lr{\outflow_i(n+1)- \meanOutflow} |^2|\filtration_n] \\ & \leq \avg[ 2 |\vectorFieldX_i(\flowDiscrete_i(n), \priceDiscrete_i(n))(\inflow(n+1) - \meanInflow)|^2 + 2|\flowDiscrete_i(n)\lr{\outflow_i(n+1)- \meanOutflow} |^2|\filtration_n] \\ & \leq \avg[ 2 \frac{\meanInflow}{\meanOutflow}|(\inflow(n+1) - \meanInflow)|^2 + 2|\flowDiscrete_i(n)\lr{\outflow_i(n+1)- \meanOutflow} |^2|\filtration_n] \\ & \leq K_1 + K_2 \|\flowDiscrete_i(n)\|^2 \\ & \leq K\lr{1+|\flowDiscrete_i(n)|^2} <+\infty
\end{align*}
where $K_1 = \frac{2\meanInflow}{\meanOutflow}|\inflowUpper-\inflowLower|^2 $, $K_2 = 2|\outflowUpper-\outflowLower|^2$ and $K = \max(K_1, K_2)$. To obtain the preceding bound we used $\vectorFieldX_i(\flowDiscrete_i(n), \priceDiscrete_i(n)) \leq \frac{\meanInflow}{\meanOutflow}$.  

Proof of \textbf{(C4)}: To prove this result we shall use Theorem \ref{thm: HirshResult}. For that purpose we need to check conditions Theorem \ref{thm: HirshResult}\ref{enum: Assm1}-\ref{enum: Assm4}.

The condition \ref{enum: Assm1} is satisfied if we show that \(\frac{\partial \vectorFieldX_i(\flowContinuous,\priceContinuous)}{\partial \flowContinuous_j} \geq 0\). Indeed, by definition 
\begin{align*}
    \frac{\partial h_i(x,p)}{\partial x_j}  = \frac{\meanInflow}{\meanOutflow} \exp(-\beta \costPrice_i(x_i,p_i)) \frac{\beta\exp(-\beta \costPrice_j(x_j,p_j) )\frac{\partial \costPrice_j(x_j,p_j)}{\partial x_j}}{\lr{\sum_{j\in[\numLinks]}\exp\lr{-\beta \costPrice_j(x_j,p_j)}}^2} > 0.
\end{align*}

Furthermore, note that condition \ref{enum: Assm2} is also satisfied because the Jacobian matrix has all the off-diagonal terms positive and is therefore irreducible. Moreover, it follows from \eqref{eq: hVectorFieldDef} that  for any \(x,p\in\R^{\numLinks}\) , \(\vectorFieldX_i(x,p) \in \lr{0,\frac{\meanInflow}{\meanOutflow}}\) and therefore \ref{enum: Assm3}-\ref{enum: Assm4} are also satisfied. This completes the proof.

Proof of \textbf{(C5)}: We shall now show that \eqref{eq: PriceDynamicsTilde} satisfies conditions \ref{enum: Assm1}-\ref{enum: Assm4} in Theorem \ref{thm: HirshResult}. This ensures global convergence to the equilibrium set which is guaranteed to be singleton by Lemma \ref{lemma:unique_price}. 
For better presentation, for any \(i,j\in[\numLinks]\), we denote the derivative of \(\fixedPointFlow_i(\priceContinuous)\) with respect to \(\priceContinuous_j\) by \(\grad_j \fixedPointFlow(\priceContinuous)\)\footnote{
Note that in Lemma \ref{lemma:monotonicity}, we established that \(\fixedPointFlow(p)\) is continuously differentiable}.  
Using \eqref{eq: xEquilibrium} for any \(i\neq j\) we have
\begin{align}
    \exp(-\beta \costPrice_j(\fixedPointFlow_j(\priceContinuous),\priceContinuous_j)) \fixedPointFlow_i(\priceContinuous)= \exp(-\beta \costPrice_i(\fixedPointFlow_i(\priceContinuous),\priceContinuous_i)) \fixedPointFlow_j(\priceContinuous)
\end{align}
Taking derivative of the above equation with respect to \(\priceContinuous_k\) for \(k\neq i\neq j\): 
\begin{align*}
    & \exp(-\beta \costPrice_j(\fixedPointFlow_j(\priceContinuous),\priceContinuous_j))\grad_k\fixedPointFlow_i(\priceContinuous) \\&\quad + \fixedPointFlow_i(\priceContinuous)\exp(-\beta \costPrice_j(\fixedPointFlow_j(\priceContinuous),\priceContinuous_j))(-\beta \grad_x\costPrice_j(\fixedPointFlow_j(\priceContinuous),\priceContinuous_j) \grad_k \fixedPointFlow_j(\priceContinuous)) \\ 
     &= \exp(-\beta \costPrice_i(\fixedPointFlow_i(\priceContinuous),\priceContinuous_i))\grad_k\fixedPointFlow_j(\priceContinuous) \\ &\quad  + \fixedPointFlow_j(\priceContinuous)\exp(-\beta \costPrice_i(\fixedPointFlow_i(\priceContinuous),\priceContinuous_i))(-\beta \grad_x\costPrice_i(\fixedPointFlow_i(\priceContinuous),\priceContinuous_i) \grad_k \fixedPointFlow_i(\priceContinuous)).
\end{align*}
Collecting similar terms together we get 
\begin{align*}
    &\grad_k\fixedPointFlow_i(\priceContinuous)\lr{\exp(-\beta \costPrice_j(\fixedPointFlow_j(\priceContinuous),\priceContinuous_j))} \\&\quad + \grad_k\fixedPointFlow_i(\priceContinuous)\lr{\fixedPointFlow_j(\priceContinuous)\exp(-\beta \costPrice_i(\fixedPointFlow_i(\priceContinuous),\priceContinuous_i))(\beta \grad_x\costPrice_i(\fixedPointFlow_i(\priceContinuous),\priceContinuous_i) )} \\
    &= \grad_k\fixedPointFlow_j(\priceContinuous) \lr{\exp(-\beta \costPrice_i(\fixedPointFlow_i(\priceContinuous),\priceContinuous_i))} \\&\quad + \grad_k\fixedPointFlow_j(\priceContinuous) \lr{ \fixedPointFlow_i(\priceContinuous)\exp(-\beta \costPrice_j(\fixedPointFlow_j(\priceContinuous),\priceContinuous_j))(\beta \grad_x\costPrice_j(\fixedPointFlow_j(\priceContinuous),\priceContinuous_j) )} .
\end{align*}
This implies for \(i\neq j\neq k\) and for any \(p\in\R^{\numLinks}\) we have
\begin{align}\label{eq: SameSign}
\grad_k \fixedPointFlow_i(\priceContinuous) \cdot \grad_k \fixedPointFlow_j(\priceContinuous) > 0.
\end{align}
Moreover, by definition of fixed point in \eqref{eq: xEquilibrium} we have the constraint that
\[
\sum_{l\in[\numLinks]}\fixedPointFlow_l(p) = \frac{\lambda}{\mu}.
\]
Taking derivative with respect to \(\priceContinuous_k\) of the above equation we obtain
\begin{align}\label{eq: DerivativeConstraint}
\sum_{l\neq k} \grad_k\fixedPointFlow_l(p) = - \grad_k\fixedPointFlow_k(p) > 0,
\end{align}
where the last inequality follows from Lemma \ref{lemma:monotonicity}. Equation \eqref{eq: DerivativeConstraint} in conjunction with \eqref{eq: SameSign} implies that \(\grad_k \fixedPointFlow_i(p) > 0\) forall \(i\neq k\). This ensures satisfaction of \ref{enum: Assm1}-\ref{enum: Assm2}. The requirement \ref{enum: Assm3}-\ref{enum: Assm4} is also satisfied as for any \(p\in\R^{\numLinks}\), \(\fixedPointFlow(\priceContinuous)\in \lr{0,\frac{\meanInflow}{\meanOutflow}}\). This completes the proof. 
\subsection{Proof of Lemma \ref{lemma: borkar}}
Note that to invoke the results from two timescale stochastic approximation theory \cite{borkar2009stochastic}, in addition to Lemma \ref{lemma: prep} we also need to ensure the following 
\begin{enumerate}[label= (\roman*)]
    \item \label{enum: additional1}the function \(\fixedPointFlow(p)\) is Lipschitz;
    \item \label{enum: additional2}the function \(g(x,p) \defas h(x,p)-x\), which is the vector field in 
 \eqref{eq: FixedPointFlowDynamics},    is Lipschitz; 
    \item \label{enum: additional3}the function \(r_i(p) \defas \fixedPointFlow_i(p)\frac{d\ell_i(\fixedPointFlow_i(p))}{dx} - p_i \), which is the vector field in \eqref{eq: PriceDynamicsTilde}, is Lipschitz for all \(i\in[\numLinks]\).   
\end{enumerate}
If the above conditions hold, then \cite[Chapter 9]{borkar2009stochastic} ensures that Theorem \ref{theorem: fixed_point} hold. 


Note that \ref{enum: additional1} holds due the fact that \(\fixedPointFlow(p) \in (0,\lambda/\mu)\) and Lemma \ref{lemma:monotonicity} where we established that it is continuously differentiable. Moreover, \ref{enum: additional2} holds due to Lemma \ref{lem: LipschitzFunction}. At last, to show \ref{enum: additional3} we note that for any \(p,p'\in\R^{\numLinks}\) and \(i\in[\numLinks]\):
\begin{align*}
     &\|r_i(p)-r_i(p')\| =
     \big\|\fixedPointFlow_i(p)\frac{d\ell_i(\fixedPointFlow_i(p))}{dx} - \fixedPointFlow_i(p')\frac{d\ell_i(\fixedPointFlow_i(p'))}{dx} \big\| \\
    &\leq \big\|\fixedPointFlow_i(p)\frac{d\ell_i(\fixedPointFlow_i(p))}{dx} - \fixedPointFlow_i(p')\frac{d\ell_i(\fixedPointFlow_i(p))}{dx} \big\| + \big\|\fixedPointFlow_i(p')\frac{d\ell_i(\fixedPointFlow_i(p))}{dx} - \fixedPointFlow_i(p')\frac{d\ell_i(\fixedPointFlow_i(p'))}{dx} \big\| \\ 
    &\leq \big|\frac{d\ell_i(\fixedPointFlow_i(p))}{dx} \big| \|\fixedPointFlow_i(p)-\fixedPointFlow_i(p')\| + |\fixedPointFlow_i(p')|\big\|  \frac{d\ell_i(\fixedPointFlow_i(p))}{dx} - \frac{d\ell_i(\fixedPointFlow_i(p'))}{dx}\big\| \\ 
    &\leq K_1 \bar{L}\|p-p'\|+ K_2 \tilde{L}\|p-p'\|,
\end{align*}
where \(K_1 = \max_{i\in[\numLinks],x\in [0,\lambda/\mu]}\big| \frac{d\ell_i(x)}{dx}\big|\), \(\bar{L}\) is the Lipschitz constant for \(\fixedPointFlow(\cdot)\), \(K_2 = \lambda/\mu  \bar{L}\) and \(\tilde{L}\) is the Lipschitz constant for \(\frac{d \ell_i(x)}{dx}\) when \(x\in [0,\lambda/\mu]\).  


==> Dynamic_Routing_Regular (Arxiv)/result_revised.tex <==
\section{Main Results}
In Sec. \ref{subsec:fixed_point}, we present a continuous-time deterministic dynamics that is associated with the discrete-time stochastic dynamics \eqref{eq: CombinedDT}. We show that the continuous time dynamics has a unique fixed point. The fixed point flow vector is a \textcolor{red}{generalized stochastic user equilibrium} associated with the fixed point toll price, and it minimizes the social cost as $\beta \to \infty$. In Sec. \ref{ssec: Convergence}, we apply the two timescale stochastic approximation theory to show that the states of our discrete time dynamics $\left(\flowDiscrete(n), P(n)\right)$ \textcolor{red}{concentrate near} the unique fixed point. Therefore, the toll price in our dynamics eventually induces a \textcolor{red}{perturbed socially optimal flow vector}. %we prove the main result of the paper -- under the setup presented in \S\ref{sec: Model} the combined flow-toll price update \eqref{eq: CombinedDT} asymptotically concentrate in a neighborhood around the socially optimal flows and prices with high probability. One of the major contributions here is to show that the trajectories of the ``natural'' continuous time dynamical system, associated with the stochastic process  \eqref{eq: CombinedDT}, converges to the socially optimal flow and toll prices. We, then, employ the machinery from two-timescale constant step size stochastic approximation to bridge the connection between the continuous time dynamical system and discrete time stochastic process. 

\subsection{Continuous time dynamics and fixed point}\label{subsec:fixed_point}
We first introduce a \textcolor{red}{deterministic} continuous time dynamical system that \textcolor{red}{corresponds to} the discrete time stochastic process \eqref{eq: CombinedDT}. We define define $x(t)$ as the flow vector and $p(t)$ as the toll price vector at time $t \in [0, \infty)$ \textcolor{red}{(I suggest to use "time step" for discrete step $n$ and "time" for continuous time $t$)}. We also define \(\stepRatio \defas \frac{\stepPrice}{\meanOutflow} \), where $\meanOutflow$ (resp. $\stepPrice$) is the stepsize of the discrete dynamics of flow (resp. toll price). Since the toll price update is at a slower timescale compared to the flow update (i.e. $\stepPrice \ll \meanOutflow$), we have $\stepRatio \ll 1$. % between flow and toll prices. Furthermore, for any \(x,p\in \R^{\numLinks}\) define 

\tdBox{Define $x$ and $p$}

The continuous time dynamics of $(x(t), p(t))$ is given as follows: 
%Consider the following continuous time dynamical system, that we expect should closely follow \eqref{eq: CombinedDT}, 
\begin{equation}\label{eq: singularPerturbedODE}
    \begin{aligned}
    \dot{\flowContinuous}_i(t) &= \frac{1}{\stepRatio}\lr{\vectorFieldX_i(\flowContinuous(t),\priceContinuous(t)) - \flowContinuous_i(t)}, \\ 
    \dot{\priceContinuous}_i(t) &= -\priceContinuous_i(t) + \flowContinuous_i(t)
    \grad_x \costPrice_i(\flowContinuous_i(t), p_i(t)), \quad \forall \ t \geq 0.
    \end{aligned}
\end{equation}


\textcolor{red}{For the sake of completeness, I think you should briefly say what is "fixed point".}

We next present the fixed point of \eqref{eq: singularPerturbedODE} and their properties. To begin with, we introduce the following two definitions: 
\begin{definition}[Steady-State Stochastic User Equilibrium]\label{def:generalized_SUE}
 A flow vector $\fixedPointFlow(\priceContinuous)$ is a generalized stochastic user equilibrium corresponding to a \textcolor{red}{dispersion parameter} and a toll price vector $\priceContinuous$ if
 \begin{align}\label{eq: xEquilibrium}
    \fixedPointFlow_i(\priceContinuous) = \vectorFieldX_i(\fixedPointFlow(\priceContinuous),\priceContinuous) = \frac{\meanInflow}{\meanOutflow}\frac{\exp(-\sueParameter \costPrice_i(\fixedPointFlow_i(\priceContinuous),\priceContinuous_i))}{\sum_{j\in[R]}\exp(-\sueParameter \costPrice_j(\fixedPointFlow_j(\priceContinuous),\priceContinuous_j))}.
\end{align}

\end{definition}

\textcolor{red}{Add interpretation of this definition, build the link to generalized Wardrop equilibrium with $\beta \to \infty$.}

\begin{definition}[Perturbed socially optimal flow]\label{def:perturbed_opt}
A flow vector $\fixedPointFlow$ is a perturbed socially optimal flow if $\fixedPointFlow$ minimizes the following convex optimization problem: 
\begin{equation}\label{eq: SocialCostWE}
\begin{aligned}
    \min_{y\in \R^{\numLinks}} &\quad \sum_{i\in[\numLinks]} y_i\costEdge_i(y_i) + \frac{1}{\beta}\sum_{i\in[\numLinks]} y_i\log(y_i) \\
    \text{s.t} & \quad \sum_{i\in[\numLinks]} y_i = \frac{\meanInflow}{\meanOutflow}.
\end{aligned}
\end{equation}
\end{definition}
\textcolor{red}{Add interpretation of this definition, build the link to social optimality with $\beta \to \infty$.}
 %Owing to  the assumption \(\stepRatio<<1\) we see that \(\flowContinuous(\cdot)\) is a ``fast'' dynamics while \(\priceContinuous(\cdot)\) is a comparatively ``slower'' component. Therefore we can consider \(\priceContinuous(\cdot)\) ``static'' while analyzing the behavior of \(\flowContinuous(\cdot)\). We therefore first consider the following dynamical system for any fixed \(\priceContinuous\in\R^{\numLinks}\):
 
 
 \begin{theorem}\label{theorem: fixed_point}
 The continuous time dynamical system \eqref{eq: singularPerturbedODE} has a unique fixed point $(\fixedPointFlow(\fixedPointPrice), \fixedPointPrice)$ such that $\fixedPointFlow$ is a generalized stochastic user equilibrium corresponding to $\fixedPointPrice$, and 
 \begin{align}\label{eq: pEquilibrium}
    \fixedPointPrice_i = \fixedPointFlow_i(\fixedPointPrice) \grad \costEdge_i(\fixedPointFlow_i(\fixedPointPrice)).
\end{align}
Moreover, $\fixedPointFlow$ is a perturbed socially optimal flow. 
 \end{theorem}
 
 \textcolor{red}{Interpret Theorem \ref{theorem: fixed_point}.}
 
The proof of Theorem \ref{theorem: fixed_point} has three parts: 

\emph{Part 1:} We show that any fixed point of \eqref{eq: singularPerturbedODE} must satisfy that the flow vector is a generalized stochastic user equilibrium corresponding to the price vector, and the price vector satisfies \eqref{eq: pEquilibrium} (Lemma \ref{lemma:twotimescale}). This part relies on the fact that our dynamical system has two timescales. 

\emph{Part 2:} We prove that the fixed point $\left(\fixedPointFlow, \fixedPointPrice\right)$ is unique. In this part, we first show that for any price vector $\priceContinuous$, the generalized stochastic user equilibrium $\fixedPointFlow(\priceContinuous)$ is unique, and can be solved as the optimal solution of a convex optimization problem (Lemma \ref{lemma:gStochasticEquilibrium}). Secondly, we prove that there exists a unique fixed point price vector $\fixedPointPrice$ that satisfies \eqref{eq: pEquilibrium}. We note that in \eqref{eq: pEquilibrium}, the flow vector $\fixedPointFlow(\priceContinuous)$ is a generalized stochastic user equilibrium that depends on $\priceContinuous$. Thus, the key step of proving the uniqueness of $\priceContinuous$ is to show that the generalized stochastic equilibrium $\fixedPointFlow(\priceContinuous)$ is monotonic in $\priceContinuous$ (Lemmas \ref{lemma:monotonicity} and \ref{lemma:unique_price}). 


\emph{Part 3:} We conclude the theorem by proving that, given the fixed point price vector $\fixedPointPrice$, the corresponding fixed point flow vector $\fixedPointFlow$ is perturbed socially optimal (Lemma \ref{lemma:optimality}).  

We now present the lemmas in each part, and provide the proof ideas of these results. We include the formal proofs in the appendix due to the space limit. 

\begin{lemma}\label{lemma:twotimescale}
For any $\epsilon \ll 1$, a state $(\fixedPointFlow, \fixedPointPrice)$ is a fixed point of \eqref{eq: singularPerturbedODE} if and only if $\fixedPointFlow$ is a generalized stochastic user equilibrium corresponding to $\fixedPointPrice$, and $\fixedPointPrice$ satisfies \eqref{eq: pEquilibrium}. 
\end{lemma}

\begin{lemma}\label{lemma:gStochasticEquilibrium}
For every \(\priceContinuous\in \R^{\numLinks}\), \(\fixedPointFlow(\priceContinuous)\) is the unique optimal solution of the following convex optimization problem
% (also known as the stochastic user equilibrium (SUE) problem \cite{cominetti2012modern})
: 
 \begin{equation}\label{eq: OptimizationProblem}
\begin{aligned}
    \min_{y\in \R^{\numLinks}} & \quad  \sum_{i\in [\numLinks]} \int_{0}^{y_i} \costPrice_i(s,p_i)ds + \frac{1}{\beta} \sum_{i\in [\numLinks]} y_i \ln{y_i}, \\
    \text{s.t} & \quad \sum_{i\in[\numLinks]} y_i = \frac{\meanInflow}{\meanOutflow}%\quad k(y)\defas.
\end{aligned}
\end{equation}
\end{lemma}
%We shall refer \(\frac{\meanInflow}{\meanOutflow}\) as the \emph{equivalent demand in asymptotic limit}.


\begin{lemma}[\textbf{Monotonicity of $\fixedPointFlow(\priceContinuous)$}]\label{lemma:monotonicity}
For any \(p,p'\in\R^{\numLinks}\) we have 
\[\lara{ \fixedPointFlow(p)-\fixedPointFlow(p'),p-p' }<0. \]
Consequently, \(\frac{\partial \fixedPointFlow_i(\priceContinuous)}{\partial \priceContinuous_i} < 0\) for all \(i\in[\numLinks]\). 
\end{lemma}

\begin{lemma}[\textbf{Existence and uniqueness of $\fixedPointPrice$}]\label{lemma:unique_price}
The fixed point price vector $\fixedPointPrice$ is unique. 
\end{lemma}

\begin{lemma}
The fixed point flow vector $\fixedPointFlow$ is perturbed socially optimal. 
\end{lemma}

\subsection{Convergence}
In this section,we show that the states $(\flowDiscrete, \priceDiscrete)$ in the discrete stochastic dynamical system converges to a \textcolor{red}{neighborhood} of the unique fixed point $(\fixedPointFlow, \fixedPointPrice)$, \textcolor{red}{and the neighborhood depends on the average update stepsize $a$.} That is, the \textcolor{red}{two timescale dynamic pricing mechanism} eventually induces a perturbed socially optimal flow. 


\begin{theorem}\label{theorem:discrete_convergence}
\begin{align}
    \limsup_{n\ra+\infty}\avg[\|\flowDiscrete_n-\fixedPointFlow\|^2+\|\priceDiscrete_n-\fixedPointPrice\|^2] = \mathcal{O}(\meanOutflow)+\mathcal{O}\lr{\frac{a}{\meanOutflow}}.
\end{align}
\end{theorem}
\textcolor{red}{You need to explain this theorem: convergence in what sense, neighborhood in what sense, how do stepsizes affect things. You also need to loop back to the focus -- updates lead to optimality.}  




To prove Theorem \ref{theorem:discrete_convergence}, we \textcolor{red}{first... (Lemma \ref{}) In this part, we apply the theory of two-timescale stochastic approximation.} Then, we show that the the continuous time dynamical system \eqref{eq: singularPerturbedODE} converges to the unique fixed point $(\fixedPointFlow, \fixedPointPrice)$ (Lemma \ref{lemma: ConvergenceFlowCont}) . Therefore, \textcolor{red}{we can conclude that  ...}



\begin{lemma}\label{lemma: ConvergenceFlowCont}
The fixed point $(\fixedPointFlow, \fixedPointPrice)$ is a globally asymptotically stable state of \eqref{eq: singularPerturbedODE}, i.e. $\lim_{t \to \infty} (\flowContinuous(t), \priceContinuous(t)) = (\fixedPointFlow, \fixedPointPrice)$.
\end{lemma}

\color{red}
We proof this lemma by applying \textcolor{red}{the theory of cooperative dynamics} from \cite{hirsch1985systems}. We provide a brief review here for the sake of completeness. 

%  For this purpose we use results  which is also stated in Theorem \ref{thm: HirshResult} for the sake of completeness.
 
%  In this section we review a result from \cite{hirsch1985systems} which provides an easily verifiable requirement on the vector field which ensures convergence to equilibrium.  

Consider a \(C^1-\)vector field \(f:\R^n\rightarrow \R^n\) and the dynamical system 
\begin{align}\label{eq: DynSys}
\dot{x}(t) = f(x(t))
\end{align}
where
\begin{enumerate}%[label=(P-\roman*)]
    \item \label{enum: Assm1} for any \(i\neq j \in [n]\) and \(x\in \R^n\) we have \(\frac{\partial f_i(x)}{\partial x_j} \geq 0\); 
    \item \label{enum: Assm2} the Jacobian matrix \(\nabla f(x)\) is irreducible;\footnote{Define irreducible here}
    \item \label{enum: Assm3} for every \(i\in[n]\), \(f_i(0)\geq 0\);
    \item \label{enum: Assm4} for any \(x\in\Rp^n\) there exists \(y > x\) with \(f_i(y) < 0\) for all \(i\in[n]\)
 \end{enumerate}
 \begin{theorem}[{\cite[Theorem 5.1]{hirsch1985systems}}]\label{thm: HirshResult}
 Let the dynamical system \eqref{eq: DynSys} satisfy the assumptions \ref{enum: Assm1}-\ref{enum: Assm4}. Then \(\Rp^n\) is positively-invariant and trajectories starting almost everywhere in \(\Rp^n\) converge to the set \(\{x: f(x) = 0\}\).  
 \end{theorem}
 
 Based on Theorem \ref{thm: HirshResult}, we prove Lemma \ref{lemma: ConvergenceFlowCont} by verifying that both the continuous time dynamics \eqref{eq: singularPerturbedODE} satisfies assumptions \ref{enum: Assm1}-\ref{enum: Assm4}. 
 \color{black}





==> Dynamic_Routing_Regular (Arxiv)/results.tex <==
\section{Results}\label{sec: Results}




\begin{align}\label{eq: FixedPointFlowDynamics}
    \dot{\flowContinuousNew}_i(t) = \vectorFieldX_i(\flowContinuousNew(t),p) -\flowContinuousNew_i(t), \quad \quad \forall i \in [\numLinks], \forall \ t\geq 0.
\end{align}



For any \(\priceContinuous\in\R^{\numLinks}\) let the equilibrium of \eqref{eq: FixedPointFlowDynamics} be denoted by \(\fixedPointFlow(\priceContinuous)\). Note that  we will keep the parameter \(\beta\) in the equilibrium flow for exactness. By definition, for every \(i\in[\numLinks]\)


As the price dynamics in \eqref{eq: singularPerturbedODE} is on a slower timescale we expect that the flow trajectory \(\flowContinuousNew\) has converged to its equilibrium value.  That is, the price dynamics in \eqref{eq: singularPerturbedODE} closely track the following continuous time dynamical system 
\begin{align}\label{eq: PriceDynamics}
    \dot{\priceContinuousNew}_i(t) = -\priceContinuousNew_i(t)+\fixedPointFlow_i(\priceContinuousNew(t))\grad_x \costPrice_i(\fixedPointFlow_i(\priceContinuousNew(t)), \priceContinuousNew_i(t)), \quad \forall \ i\in[\numLinks], \forall \ t\geq 0.
\end{align}
We denote the equilibrium of \eqref{eq: PriceDynamics} by  \(\fixedPointPrice\). It follows that for every \(i\in[\numLinks]\)
% \begin{align}\label{eq: pEquilibrium}
%     \fixedPointPrice_i = \fixedPointFlow_i(\fixedPointPrice) \grad \costEdge_i(\fixedPointFlow_i(\fixedPointPrice)).
% \end{align}
At some places in the subsequent exposition, we shall denote \(\fixedPointPrice = \fixedPointPrice^{(\beta)}\) to emphasize the explicit dependence on \(\beta\). 
% A natural question at this stage is to ensure the existence of solutions to \eqref{eq: xEquilibrium} and \eqref{eq: pEquilibrium}. Furthermore our results guarantee uniqueness of the equilibrium points as well. 

% We posit a continuous time o.d.e. in variables $\flowContinuous \in \mathbb{R}^{\numLinks}$ and $\priceContinuous \in \mathbb{R}^{\numLinks}$ that the stochastic dynamics track. 
% Because we had assumed that the price evolves on a slower timescale, we are able to study the fixed points of the price dynamic $\fixedPointPrice$ and the induced fixed point flow $\fixedPointFlow(\fixedPointPrice)$; the fixed point equations for these quantities are introduced below.
We briefly summarize the results that are presented in this section. Moreover, we also state the main proof techniques involved in the itemized list below. Details are deferred to following subsections. 
\begin{enumerate}%[align=left, label=(\textsf{R}-\Roman*), leftmargin=*,widest=iii]
    \item \label{enum: Result1} We show existence, uniqueness $\fixedPointFlow(p)$. This is ensured by drawing connections with the literature on stochastic user equilibrium \cite{cominetti2012modern}. Furthermore, we establish that the trajectories of \eqref{eq: FixedPointFlowDynamics} converge to $\fixedPointFlow(p)$, for any \(p\in\R^{\numLinks}\). This is established by noting that the dynamics \eqref{eq: FixedPointFlowDynamics} is cooperative (\cite{hirsch1985systems}). 
    \item \label{enum: Result3} We show
    existence and uniqueness of $\fixedPointPrice$. Existence is attributed to Brouwer's fixed point theorem. Meanwhile, uniqueness of $\fixedPointPrice$ is ensured by monotonicity of $p\mapsto \fixedPointFlow(p)\in\R^{\numLinks}$. Furthermore, the convergence of the trajectories of \eqref{eq: PriceDynamics} to \(\fixedPointPrice\) is again established by noting that dynamics \eqref{eq: PriceDynamics} is cooperative. 
    \item \label{enum: Result4} We conclude by noting that the discrete time stochastic process \eqref{eq: CombinedDT} concentrates near \(\fixedPointFlow(\fixedPointPrice)\) and \(\fixedPointPrice\). Towards this end, we utilize results on two timescale constant step size stochastic approximation. 
\end{enumerate}


% In addition, we also make the following technical assumption on the second moment of the price and flow processes which are crucial for using results from stochastic approximation literature. 
% \begin{assumption}[\textbf{Stability Criterion}]
% We assume that \(\sup_{n}\avg[\|\priceDiscrete(n)\|^2]<+\infty\) and \(\sup_{n}\avg[\|\flowDiscrete(n)\|^2]< +\infty \) . 
% \end{assumption}
% \begin{remark}
% {\color{red} We can add a remark here saying this one would expect this sort of technical assumption to hold because our dynamics satisfied the conditions posed in \cite{lakshminarayanan2017stability}. We can do all the calculations that show that \cite[A4-A5]{lakshminarayanan2017stability} hold.}. \end{remark}
%\todo[inline]{Will think about relaxing this assumption at later point. It is good to keep in mind the following reference: \url{https://www.sciencedirect.com/science/article/abs/pii/S0005109816305222}.}

% In this section we shall zfirst present results on existence and uniqueness of {the} equilibrium point of the dynamical systems \eqref{eq: singularPerturbedODE}. Following this, we prove the convergence of the trajectories of \eqref{eq: singularPerturbedODE} to the corresponding equilibrium.  


\subsection{
Properties of fixed points}\label{ssec: PropFixedPoint}
We now discuss the existence and uniqueness of the fixed points $\fixedPointFlow(\cdot)$ and $\fixedPointPrice$. 

In this subsection, we shall first show that \(\fixedPointFlow(\cdot)\) in \eqref{eq: xEquilibrium} is a well-defined (single valued) function.  The following proposition formalizes this claim. 
\begin{proposition}[\textbf{Existence and uniqueness of $\fixedPointFlow(\priceContinuous)$}]\label{prop: xEqExist}
For every \(\priceContinuous\in \R^{\numLinks}\), \(\fixedPointFlow(\priceContinuous)\) exists and is unique. Furthermore, one can characterize \(\fixedPointFlow(\priceContinuous)\) as solution to the following convex optimization problem
% (also known as the stochastic user equilibrium (SUE) problem \cite{cominetti2012modern})
: 
 \begin{equation}\label{eq: OptimizationProblem}
\begin{aligned}
    \min_{y\in \R^{\numLinks}} & \quad  \sum_{i\in [\numLinks]} \int_{0}^{y_i} \costPrice_i(s,p_i)ds + \frac{1}{\beta} \sum_{i\in [\numLinks]} y_i \ln{y_i}, \\
    \text{s.t} & \quad \sum_{i\in[\numLinks]} y_i = \frac{\meanInflow}{\meanOutflow}%\quad k(y)\defas.
\end{aligned}
\end{equation}

We shall refer \(\frac{\meanInflow}{\meanOutflow}\) as the \emph{equivalent demand in asymptotic limit}.
\end{proposition}

To prove the above result we analyze the KKT conditions for the convex optimization problem and uniqueness is established by the strict convexity of the optimization objective in \eqref{eq: OptimizationProblem}. 
%The details of the proof are deferred to Appendix \ref{proof: Prop31}. 
\begin{proof}[Proof of Proposition \ref{prop: xEqExist}]
In the subsequent proof we shall show that the following claims hold: 

\begin{enumerate}[label= (C-\Roman*),widest=ii,leftmargin=*,align=left]
    \item \label{thm: claim1} For any \(p\in\R^{\numLinks}\), the optimizer of \eqref{eq: OptimizationProblem} is unique; call it \(y^\star(p)\);
    \item \label{thm: claim2} \(y^\star(p)\) is an optimal solution if and only if it satisfies \(h(y^\star(p),p) = y^\star\)
\end{enumerate}
Note that the above two claims ensure that \(\fixedPointFlow(p) = y^\star(p)\). The subsequent exposition establishes the validity of these claims.

To see that \ref{thm: claim1}  is true, we note that the feasible set of \eqref{eq: OptimizationProblem} is a compact convex set.  Moreover, from the convexity of $\costEdge$ it follows that \(k(y)\) is a strictly convex function. Strict convexity ensures the uniqueness of solution of a convex optimization problem on a convex compact set \cite{boyd2004convex}.


For \ref{thm: claim2}, we now employ KKT conditions of optimality: let \(\delta\in\R \) be the Lagrange multiplier corresponding to the equality constraint. Define the Lagrangian as follows:
\[
L(y,\delta,p) \defas \sum_{r\in [\numLinks]} \int_{0}^{y_r} \costPrice_r(s,p_r)ds + \frac{1}{\beta} \sum_{r\in \numLinks} y_r \ln{y_r} + \delta \lr{\sum_{r\in[\numLinks]} y_r - \frac{\meanInflow}{\meanOutflow}}
\]

The optimal solution $y^{\star}(p)$ and Lagrange multiplier $\delta^\star$ satisfy: \begin{enumerate}[widest=ii,leftmargin=*,align=left]
    \item \(\nabla_{y}L(y^{\star}(p),\delta^{\star},p) = 0\). This gives us \(\costPrice_r(y_r^{\star}(p),p_r) + \frac{1}{\beta}\lr{1+\ln(y_r^{\star}(p))} +\delta^{\star} = 0\), which can be also written as follows
    \begin{align}
    \label{eq: Opt_y}
    y_r^{\star}(p) = \exp(-1-\beta \costPrice_r(y_r^{\star}(p),p_r))\exp(-\beta \delta^\star), \quad \forall \ r\in[\numLinks].
    \end{align}
    \item \(\nabla_\delta L(y^{\star}(p),\delta^{\star},p) = 0\). That is, 
    \(
    \sum_{r\in \numLinks} y_r^{\star}(p)  = \frac{\meanInflow}{\meanOutflow}.
    \)
    \end{enumerate}
    Using \eqref{eq: Opt_y} we have 
    \[
    \exp(-\beta \delta -1 )  = \frac{\meanInflow}{\meanOutflow} \frac{1}{\sum_{r\in[\numLinks]}\exp(-\beta \costPrice_r(y_r^{\star}(p),p_r))}
    \]

The above conditions give us that \(y^\star(p)\) is an optimal solution of \eqref{eq: OptimizationProblem} if and only if it satisfies
\[
y_r^\star(p) = \frac{\meanInflow}{\meanOutflow} \frac{\exp(-\beta \costPrice_r(y_r^\star(p),p_r))}{\sum_{r\in[\numLinks]}\exp(-\beta \costPrice_r(y_r^\star(p),p_r))} = \vectorFieldX_r(y^\star(p),\priceContinuous), \quad \forall \ r\in[\numLinks].
\]
\end{proof}
\tdBox{May be remove this remark}
\begin{remark}
\label{rem: compactnessXEq}
Note that the set \(\{\fixedPointFlow(p):p\in\R^{\numLinks}\}\) is a subset of a simplex in \(\R^{\numLinks}\). This is because for any \(p\in\R^{\numLinks}\), \(\fixedPointFlow(p) \geq 0\) and \(\sum_{i\in[\numLinks]}\fixedPointFlow_i(p) = \frac{\meanInflow}{\meanOutflow}\). 
\end{remark}

We now proceed to show the existence and uniqueness of the solution of the nonlinear fixed point equation \eqref{eq: pEquilibrium}:
\begin{proposition}[\textbf{Existence and uniqueness of $\fixedPointPrice$}]\label{prop: pEqExists}
There exists a unique solution to \eqref{eq: pEquilibrium}. 
\end{proposition}
In the above result, we prove existence by using Brouwer's fixed point theorem. However, to establish uniqueness we first observe that \(\fixedPointFlow(\cdot)\) is monotonic \todo{Expand on this, as the proof will be in the appendix}. Following which we argue that if the solution to \eqref{eq: pEquilibrium} is not unique then the monotonic nature of \(\fixedPointFlow(\cdot)\) no longer holds. The aforementioned monotonic property is more formally stated in the next lemma. 

\begin{lemma}[\textbf{Monotonicity of $\fixedPointFlow(\priceContinuous)$}]\label{lem: MonotonicityFlow}
For any \(p,p'\in\R^{\numLinks}\) we have 
\[\lara{ \fixedPointFlow(p)-\fixedPointFlow(p'),p-p' }<0. \]
Consequently, \(\frac{\partial \fixedPointFlow_i(\priceContinuous)}{\partial \priceContinuous_i} < 0\) for all \(i\in[\numLinks]\).  
\end{lemma}
The proof of Lemma \ref{lem: MonotonicityFlow} follows by arguing about the variational inequalities associated with \eqref{eq: OptimizationProblem}. The details of the proof are deferred to Appendix \ref{proof: lemMonotonic}.
\begin{remark}
Note that the monotonicity of \(\fixedPointFlow(p)\) was considered as an assumption in \cite[cf Eq. (9)]{borkar2009cooperative}. In this article we have exploited the connection of our routing scheme with stochastic user equilibrium \cite{cominetti2012modern} to \emph{prove} the monotonicity property. 
\end{remark}
\begin{proof}[\textbf{Proof of Proposition \ref{prop: pEqExists}}]
We shall first show the existence and then prove the uniqueness of \(\fixedPointPrice\). 

For any \(p\in\R^{\numLinks}, r\in[\numLinks]\), define \(z_r(p) = \fixedPointFlow(p)\grad_x\costEdge_r(\fixedPointFlow_r(p))\). The equilibrium price \(\fixedPointPrice\) is then solution to the fixed point equation \(p=z(p)\).  Define a set \(K = \{y\in\R^{\numLinks}: y\geq 0, \|y\|_1 \leq \frac{\meanInflow}{\meanOutflow}\max_{r\in[\numLinks]}\grad_x c_r\lr{\frac{\meanInflow}{\meanOutflow}}\}\). Due to Remark \ref{rem: compactnessXEq} andthe convexity of the cost, we can see that \(z(\cdot)\) maps the convex compact set \(K\) to itself. Therefore, Brouwer's fixed point theorem \cite{sastry2013nonlinear} guarantees the existence of fixed point \(\fixedPointPrice\).

% Having shown the existence of equilibrium pricing, we shall now show the uniqueness of the solution of \eqref{eq: pEquilibrium}. But before we establish that result, we present a technical lemma that is key to the subsequent proofs. The following lemma formalizes the intuition that increasing prices on any link reduces flow on that link.




Now, we prove the uniqueness of the fixed point $\fixedPointPrice$ satisfying \eqref{eq: pEquilibrium}.  
We shall prove this via a contradiction argument. Assume that there are two distinct price profiles $\fixedPointPrice, \fixedPointPrice' \in \R^{\numLinks}$ that both satisfy the fixed point equation \eqref{eq: pEquilibrium}, therefore for every \(r\in[\numLinks]\):
\begin{align*}
    \fixedPointPrice_r &= \fixedPointFlow_r(\fixedPointPrice) \grad_x \costEdge_r(\fixedPointFlow_r(\fixedPointPrice)) \\ \fixedPointPrice_r' &= \fixedPointFlow_r(\fixedPointPrice') \grad_x \costEdge_r(\fixedPointFlow_r(\fixedPointPrice'))
\end{align*}
Taking the difference we get 
\begin{align*}
    \fixedPointPrice_r - \fixedPointPrice_r' &= \fixedPointFlow_r(\fixedPointPrice) \grad_x \costEdge_r(\fixedPointFlow_r(\fixedPointPrice)) - \fixedPointFlow_r(\fixedPointPrice') \grad_x \costEdge_r(\fixedPointFlow_r(\fixedPointPrice')) , \\ 
    &= \fixedPointFlow_r(\fixedPointPrice) \grad_x \costEdge_r(\fixedPointFlow_r(\fixedPointPrice)) - \fixedPointFlow_r(\fixedPointPrice') \grad_x \costEdge_r(\fixedPointFlow_r(\fixedPointPrice))\\
    &\quad \quad \quad + \fixedPointFlow_r(\fixedPointPrice') \grad_x \costEdge_r(\fixedPointFlow_r(\fixedPointPrice)) - \fixedPointFlow_r(\fixedPointPrice') \grad_x \costEdge_r(\fixedPointFlow_r(\fixedPointPrice')),  \\
    &= \lr{\fixedPointFlow_r( \fixedPointPrice)-\fixedPointFlow_r(\fixedPointPrice')}   \grad_x\costEdge_r(\fixedPointFlow_r(\fixedPointPrice))\\&\quad\quad\quad +\fixedPointFlow_r(\fixedPointPrice')\lr{\grad_x \costEdge_r(\fixedPointFlow_r(\fixedPointPrice))-\grad_x\costEdge_r(\fixedPointFlow_r(\fixedPointPrice'))},
\end{align*}
for every \(r\in[\numLinks]\). Multiplying \((\fixedPointFlow_r(\fixedPointPrice)-\fixedPointFlow_r(\fixedPointPrice'))\) in the preceding equation we obtain
\begin{equation}
\begin{aligned}\label{eq: pUniquenessContradiction}
    &(\fixedPointFlow_r(\fixedPointPrice)-\fixedPointFlow_r(\fixedPointPrice'))(\fixedPointPrice_r - \fixedPointPrice_r') = \lr{\fixedPointFlow_r(\fixedPointPrice)-\fixedPointFlow_r(\fixedPointPrice')}^2\grad_x \costEdge_r(\fixedPointFlow_r(\fixedPointPrice))\\&\quad\quad\quad +\fixedPointFlow_r(\fixedPointPrice') \lr{\grad_x \costEdge_r(\fixedPointFlow_r(\fixedPointPrice))-\grad_x \costEdge_r(\fixedPointFlow_r(\fixedPointPrice'))} (\fixedPointFlow_r(\fixedPointPrice)-\fixedPointFlow_r(\fixedPointPrice')), 
\end{aligned}
\end{equation}
for every \(r\in[\numLinks]\). Convexity of the edge cost function ensures that right hand side of \eqref{eq: pUniquenessContradiction} is always non-negative for every \(r\in[\numLinks]\). 
Summing over \(r\in[R]\) and using Lemma \ref{lem: MonotonicityFlow} we obtain:
\begin{align*}
    0>\lara{ \fixedPointFlow_r(\fixedPointPrice)-\fixedPointFlow_r(\fixedPointPrice'), \fixedPointPrice-\fixedPointPrice' } \geq 0.
\end{align*}
which contradicts our original hypothesis that there are two distinct price profiles satisfying \eqref{eq: pEquilibrium}. Therefore the existence result Proposition \ref{prop: pEqExists} ensures uniqueness. 
\end{proof}

The existence and uniqueness results presented above, interestingly, ensure that for any toll price \(p\), \(\fixedPointFlow(p)\) approaches the Wardrop(selfish) equilibrium as we let the perturbation parameter \(\beta\) to infinity. Furthermore, in the limit the equilibrium pricing ensures that the emergent flow on the network are socially optimal. This result is formalized in the result below. 

\todo{Should we make this a theorem? Also we want $\bar{p}$ to be the socially optimal marginal cost price.}
\begin{proposition}[\textbf{Social optimality of \(\fixedPointFlow(\fixedPointPrice^{(\beta)})\)}]\label{prop: ConnectionToWardrop}
For any \(\beta>0\), the equilibrium flow \(\fixedPointFlow(\fixedPointPrice^{(\beta)})\) is the minimizer of the following strictly convex optimization problem:

\end{proposition}
The proof of Proposition \ref{prop: ConnectionToWardrop} follows by comparing the variational inequalities associated with \eqref{eq: OptimizationProblem} ( at \(p=\fixedPointPrice^{(\beta)}\) ) and \eqref{eq: SocialCostWE}. 
The details of the proof can be found in Appendix \ref{proof: PropWardrop}. 
\begin{remark}
The cost function in \eqref{eq: SocialCostWE} is an entropy regularized social cost function. Note that in the limit \(\beta\uparrow \infty\), for any \(p\in \R^{\numLinks}\) the flow \(\fixedPointFlow(p)\) converges to the static Wardrop assignment \cite{cominetti2012modern}. Furthermore, as \(\beta\uparrow +\infty\), the equilibrium flow \(\fixedPointFlow(\fixedPointPrice^{(\beta)})\) converges to the socially optimal flow \cite{roughgarden2010algorithmic}.
\end{remark}



\subsection{Convergence}\label{ssec: Convergence}
We shall first show that for any fixed \(\priceContinuous\in\R^{\numLinks}\), the trajectories of the dynamical system \eqref{eq: FixedPointFlowDynamics} converges to the equilibrium \(\fixedPointFlow(\priceContinuous)\). For this purpose we use results from \cite{hirsch1985systems} which is also stated in Theorem \ref{thm: HirshResult} for the sake of completeness.
\begin{proposition}\label{prop: ConvergenceFlowCont}
For any fixed \(p\in\R^{\numLinks}\) the point \(\fixedPointFlow(\priceContinuous)\) is a globally asymptotically stable equilibrium of  \eqref{eq: FixedPointFlowDynamics}.  
\end{proposition}
\begin{proof}
To prove this result we shall use Theorem \ref{thm: HirshResult}. For that purpose we need to check conditions Theorem \ref{thm: HirshResult}\ref{enum: Assm1}-\ref{enum: Assm4}.

The condition \ref{enum: Assm1} is satisfied if we show that \(\frac{\partial \vectorFieldX_i(\flowContinuous,\priceContinuous)}{\partial \flowContinuous_j} \geq 0\). Indeed, by definition 
\begin{align*}
    \frac{\partial h_i(x,p)}{\partial x_j}  = \frac{\meanInflow}{\meanOutflow} \exp(-\beta \costPrice_i(x_i,p_i)) \frac{\beta\exp(-\beta \costPrice_j(x_j,p_j) )\frac{\partial \costPrice_j(x_j,p_j)}{\partial x_j}}{\lr{\sum_{j\in[\numLinks]}\exp\lr{-\beta \costPrice_j(x_j,p_j)}}^2} > 0.
\end{align*}
The condition \ref{enum: Assm2} is also satisfied trivially because the Jacobian matrix has all the off-diagonal terms positive and is therefore irreducible. Moreover, it follows from \eqref{eq: hVectorFieldDef} that  for any \(x,p\in\R^{\numLinks}\) , \(\vectorFieldX_i(x,p) \in \lr{0,\frac{\meanInflow}{\meanOutflow}}\) and therefore \ref{enum: Assm3}-\ref{enum: Assm4} are also satisfied. This completes the proof.
\end{proof}


Before presenting the next result, we define some notations that will be helpful for concise presentation. Define \(\diagC(x) \defas \diag\lr{\lr{\grad_x \costEdge_i(x)}_{i=1}^{\numLinks}} \) and \(\diagMarginal(x) \defas \diag\lr{\lr{x_i\grad_x \costEdge_i(x)}_{i=1}^{\numLinks}}\). We shall now discuss the convergence of \eqref{eq: PriceDynamics} to the equilibrium \(\fixedPointPrice\). 
\begin{proposition}\label{prop: ConvergencePriceCont}
The equilibrium \(\fixedPointPrice\) is the globally asymptotically stable equilibrium of \eqref{eq: PriceDynamics}.
\end{proposition}
\begin{proof}
First, we show that $\fixedPointFlow(\priceContinuous)$ is a differentiable function of $\priceContinuous$. To do this, we invoke the implicit function theorem for that map $\fixedGap(x, p) = x - h(x, p)$.
Note that for any fixed \(p\), \(\fixedPointFlow(p)\) is the zero of \(\fixedGap(\cdot,p)\). To satisfy the hypothesis in implicit function theorem: for any \(\priceContinuous\) we compute the Jacobian of the function $\fixedGap(x, p)$ with respect to \(x\) and evaluate it at $\fixedPointFlow(\priceContinuous)$. Using Lemma \ref{lem: LipschitzFunction} the Jacobian is given by: 
\begin{align*}
   \grad_x \fixedGap(\fixedPointFlow(p),p) &= I - \grad_x \vectorFieldX(\fixedPointFlow(p),p) \\
   & = I - \frac{\meanOutflow}{\meanInflow}\beta\fixedPointFlow(p)\fixedPointFlow(p)^\top \diagC(\fixedPointFlow(p)) + \beta\diagMarginal\lr{\fixedPointFlow(p)} \\ 
   & = \lr{\lr{\diagMarginal^{-1}(\fixedPointFlow(p)) + \beta I}-\beta v\mathbbm{1}^\top}\diagMarginal(\fixedPointFlow(p)) 
\end{align*}
where \(v \defas \frac{\meanOutflow}{\meanInflow}\fixedPointFlow(p)\). Note that from \eqref{eq: xEquilibrium} we have \(\mathbbm{1}^\top v = 1\).
We claim that \(\det(D_x \fixedGap(\fixedPointFlow(p),p)) \neq 0\). Indeed, 
\begin{align*}
    \det(D_x \fixedGap(\fixedPointFlow(p),p)) &= \det\lr{\diagMarginal(\fixedPointFlow(p)} \det\lr{\lr{\diagMarginal^{-1}(\fixedPointFlow(p)) + \beta I}-\beta v\mathbbm{1}^\top }\\ 
   &= \det\lr{\diagMarginal(\fixedPointFlow(p)}\cdot
    \det\lr{I-\beta v\mathbbm{1}^\top\lr{\diagMarginal^{-1}(\fixedPointFlow(p)) + \beta I}^{-1} }\\&\quad\quad \cdot \det\lr{\diagMarginal^{-1}(\fixedPointFlow(p)) + \beta I}^{-1}
\end{align*}
It is sufficient to show that \( \det\lr{I-\beta v\mathbbm{1}^\top\lr{\diagMarginal^{-1}(\fixedPointFlow(p)) + \beta I}^{-1} }\neq 0\). Using the Sherman-Morrison formula \cite{gentle2007matrix} it is necessary and sufficient to show that \(\beta\mathbbm{1}^\top\lr{\diagMarginal^{-1}(\fixedPointFlow(p)) + \beta I}^{-1} v \neq 1 \). 

We show it by contradiction. Suppose \(\beta\mathbbm{1}^\top\lr{\diagMarginal^{-1}(\fixedPointFlow(p)) + \beta I}^{-1} v = 1 \). Then 
\begin{align*}
&\implies \quad \sum_{i=1}^{\numLinks} v_i \frac{\beta}{\frac{1}{m_i}+\beta} = 1\\
&\implies \quad \sum_{i=1}^{\numLinks} v_i \frac{\beta}{\frac{1}{m_i}+\beta} = \sum_{i=1}^{\numLinks} v_i \\ 
&\implies \sum_{i=1}^{\numLinks} v_i\frac{\frac{1}{m_i}}{\beta+\frac{1}{m_i}} = 0
\end{align*}
This is not possible as the terms on the left hand side are all positive. 
% \begin{align}
%     J_{g, \flowContinuous}(\fixedPointFlow(\priceContinuous) , \priceContinuous) &= \begin{bmatrix} \frac{\partial \hat{g_i}(\fixedPointFlow(\priceContinuous), \priceContinuous)}{\partial \flowContinuous_j} \end{bmatrix} \\ & = I_{R \times R} - \begin{bmatrix} \frac{\partial h_i(\fixedPointFlow(\priceContinuous) , \priceContinuous)}{ \partial \flowContinuous_j}\end{bmatrix} \\ &=  I_{R \times R} - \frac{\meanInflow}{\meanOutflow} \begin{bmatrix} \begin{cases} \frac{\lr{\sum_{j\in[\numLinks]}\exp\lr{-\beta \costPrice_j(\fixedPointFlow_j(\priceContinuous),\priceContinuous_j)}}  \exp(-\beta \costPrice_i(\fixedPointFlow_i (\priceContinuous), \priceContinuous_i)}{\lr{\sum_{j\in[\numLinks]}\exp\lr{-\beta \costPrice_j(\fixedPointFlow_j(\priceContinuous),\priceContinuous_j)}}^2} \text{ if } i = j \\  \exp(-\beta \costPrice_i(\fixedPointFlow_i(\priceContinuous),\priceContinuous_i)) \frac{\beta\exp(-\beta \costPrice_j(\fixedPointFlow_j(\priceContinuous),\priceContinuous_j) )\frac{\partial \costPrice_j(\fixedPointFlow_j(\priceContinuous),\priceContinuous_j)}{\partial x_j}}{\lr{\sum_{j\in[\numLinks]}\exp\lr{-\beta \costPrice_j(\fixedPointFlow_j(\priceContinuous),\priceContinuous_j)}}^2} \text{ if } i \neq j \end{cases} \end{bmatrix}
% \end{align}    

% \todo[inline]{We need to show that the operator \(\R^R\ni p  \mapsto F(\fixedPointFlow(p)) \defas \fixedPointFlow(p)\odot \partial_x c(\fixedPointFlow(p))\in \R^R\) is monotone}

% \begin{align*}
% &\lara{ p-p',\fixedPointFlow(p)\odot\partial_x\costEdge(\fixedPointFlow(p)) -\fixedPointFlow(p')\odot\partial_x\costEdge(\fixedPointFlow(\fixedPointPrice))} = \sum_{r\in[R]}(p_r-p_r')((\fixedPointFlow_r(p))^4-(\fixedPointFlow_r(p'))^4)\\
% &= \sum_{r\in[R]}(p_r-p_r')((\fixedPointFlow_r(p)-\fixedPointFlow_r(p')(\fixedPointFlow_r(p)+\fixedPointFlow_r(p'))(\fixedPointFlow_r(p))^2+(\fixedPointFlow_r(p'))^2)
% \end{align*}

% Monotonicity 
% \[
% \sum_{r}(p_r-p_r')(\fixedPointFlow_r(p)-\fixedPointFlow_r(p')) < 0
% \]

% \todo[inline]{For the cooperative dynamics ideas to work it suffices to show that \(\partial \fixedPointFlow_i(p)/\partial p_j > 0\) for \(i\neq j\)}

% Alternatively: 

% \begin{itemize}
%     \item First show that $\frac{\partial \fixedPointFlow (p) \partial_x c(\fixedPointFlow(p))}{\partial x_j} > 0$ to guarantee the convergence of $p(t)$ to the set of equilibria with high probability. 
% \end{itemize}

% \textbf{Claim:} The minimizer $x^*$ of $S(x) = \sum_{i=1}^{R} x_i c_i(x_i)$ is unique because $S(x)$ is a convex function. 

% \textbf{Proof:} $S(x)$ is the sum of the product of nondecreasing convex functions $x_i$ and $c_i(x_i)$. 

% \textbf{Claim:} The marginal cost tax $p_i = x_i c_i'(x_i)$ such that for $(R , \zeta, c_i)$, the equilibrium flow $x^{*}$ of $(R , \zeta, c_i + p_i)$ minimizes $S(x)$ is unique. 

% \textbf{Recall:} The equilibrium $\bar{p}$ satisfies the fixed point equation $\bar{p}_i = \fixedPointFlow_i(\bar{p}) \partial_x c_i(\fixedPointFlow_i(\bar{p}))$

 

% \begin{equation}
% \begin{aligned}
%     \min_{y\in \R^{\numLinks}} &\quad \ell(y)\defas \sum_{r\in [\numLinks]} \int_{0}^{y_r} \costEdge_r(s)+p_rds + \frac{1}{\beta} \sum_{r\in [\numLinks]} y_r \ln{y_r} \\
%     \text{s.t} & \quad \sum_{r\in[\numLinks]} y_r = \frac{\meanInflow}{\meanOutflow}
% \end{aligned}
% \end{equation}

% \(\fixedPointFlow(p)\) is minimizer of above. \(p=\bar{p}\) then \(\fixedPointFlow(\bar{p})\) is minimizer of 
% \begin{equation}
% \begin{aligned}
%     \min_{y\in \R^{\numLinks}} &\quad \ell(y)\defas \sum_{r\in [\numLinks]} \int_{0}^{y_r} \costEdge_r(s)+\fixedPointFlow(\bar{p})\partial_xc_r(\fixedPointFlow(\bar{p}))ds + \frac{1}{\beta} \sum_{r\in [\numLinks]} y_r \ln{y_r} \\
%     \text{s.t} & \quad \sum_{r\in[\numLinks]} y_r = \frac{\meanInflow}{\meanOutflow}
% \end{aligned}

% \end{equation}


We shall now show that \eqref{eq: PriceDynamics} satisfies conditions \ref{enum: Assm1}-\ref{enum: Assm4} in Theorem \ref{thm: HirshResult}. This ensures global convergence to the equilibrium set which is guaranteed to be singleton by Proposition \ref{prop: pEqExists}. 
For better presentation, for any \(i,j\in[\numLinks]\), we shall concisely denote the gradient of \(\fixedPointFlow_i(\priceContinuous)\) with respect to \(\priceContinuous_j\) by \(\grad_j \fixedPointFlow(\priceContinuous)\).  
Using \eqref{eq: xEquilibrium} for any \(i\neq j\) we have
\begin{align}
    \exp(-\beta \costPrice_j(\fixedPointFlow_j(\priceContinuous),\priceContinuous_j)) \fixedPointFlow_i(\priceContinuous)= \exp(-\beta \costPrice_i(\fixedPointFlow_i(\priceContinuous),\priceContinuous_i)) \fixedPointFlow_j(\priceContinuous)
\end{align}
Taking derivative of the above equation with respect to \(\priceContinuous_k\) for \(k\neq i\neq j\): 
\begin{align*}
    & \exp(-\beta \costPrice_j(\fixedPointFlow_j(\priceContinuous),\priceContinuous_j))\grad_k\fixedPointFlow_i(\priceContinuous) \\&\quad + \fixedPointFlow_i(\priceContinuous)\exp(-\beta \costPrice_j(\fixedPointFlow_j(\priceContinuous),\priceContinuous_j))(-\beta \grad_x\costPrice_j(\fixedPointFlow_j(\priceContinuous),\priceContinuous_j) \grad_k \fixedPointFlow_j(\priceContinuous)) \\ 
     &= \exp(-\beta \costPrice_i(\fixedPointFlow_i(\priceContinuous),\priceContinuous_i))\grad_k\fixedPointFlow_j(\priceContinuous) \\ &\quad  + \fixedPointFlow_j(\priceContinuous)\exp(-\beta \costPrice_i(\fixedPointFlow_i(\priceContinuous),\priceContinuous_i))(-\beta \grad_x\costPrice_i(\fixedPointFlow_i(\priceContinuous),\priceContinuous_i) \grad_k \fixedPointFlow_i(\priceContinuous)).
\end{align*}
Collecting similar terms together we get 
\begin{align*}
    &\grad_k\fixedPointFlow_i(\priceContinuous)\lr{\exp(-\beta \costPrice_j(\fixedPointFlow_j(\priceContinuous),\priceContinuous_j))} \\&\quad + \grad_k\fixedPointFlow_i(\priceContinuous)\lr{\fixedPointFlow_j(\priceContinuous)\exp(-\beta \costPrice_i(\fixedPointFlow_i(\priceContinuous),\priceContinuous_i))(\beta \grad_x\costPrice_i(\fixedPointFlow_i(\priceContinuous),\priceContinuous_i) )} \\
    &= \grad_k\fixedPointFlow_j(\priceContinuous) \lr{\exp(-\beta \costPrice_i(\fixedPointFlow_i(\priceContinuous),\priceContinuous_i))} \\&\quad + \grad_k\fixedPointFlow_j(\priceContinuous) \lr{ \fixedPointFlow_i(\priceContinuous)\exp(-\beta \costPrice_j(\fixedPointFlow_j(\priceContinuous),\priceContinuous_j))(\beta \grad_x\costPrice_j(\fixedPointFlow_j(\priceContinuous),\priceContinuous_j) )} .
\end{align*}
This implies for \(i\neq j\neq k\) and for any \(p\in\R^{\numLinks}\) we have
\begin{align}\label{eq: SameSign}
\grad_k \fixedPointFlow_i(\priceContinuous) \cdot \grad_k \fixedPointFlow_j(\priceContinuous) > 0.
\end{align}
Moreover, by definition of fixed point in \eqref{eq: xEquilibrium} we have the constraint that
\[
\sum_{l\in[\numLinks]}\fixedPointFlow_l(p) = \frac{\lambda}{\mu}.
\]
Taking derivative with respect to \(\priceContinuous_k\) of the above equation we obtain
\begin{align}\label{eq: DerivativeConstraint}
\sum_{l\neq k} \grad_k\fixedPointFlow_l(p) = - \grad_k\fixedPointFlow_k(p) > 0,
\end{align}
where the last inequality follows from Lemma \ref{lem: MonotonicityFlow}. Equation \eqref{eq: DerivativeConstraint} in conjunction with \eqref{eq: SameSign} implies that \(\grad_k \fixedPointFlow_i(p) > 0\) forall \(i\neq k\). This ensures satisfaction of \ref{enum: Assm1}-\ref{enum: Assm2}. The requirement \ref{enum: Assm3}-\ref{enum: Assm4} is also satisfied as for any \(p\in\R^{\numLinks}\), \(\fixedPointFlow(\priceContinuous)\in \lr{0,\frac{\meanInflow}{\meanOutflow}}\). This completes the proof. 
\end{proof}

\todo[inline]{Merge this with section 3.2}
\subsection{Properties of discrete-time stochastic process \eqref{eq: CombinedDT}}\label{ssec: SATheoryConvergence}
% \tdBox{Need to think about the Lipschitz property of p dynamics \eqref{eq: PriceDynamics}. Somehow need to use the property that \(\|X(n)\|\) is bounded a.s. May be we can make arguments such as if we keep \(\mu\) small then process \(X(n)\) will track its asymptotically stable system closely and therefore we can get the Lipschitzness of the dynamics of p. Need to make this formal. May be the arguments of the form: 
% \[
% \Pr(\|X_n\|\geq R) \leq \frac{\avg[\|X_n\|^2]}{R^2} < \infty 
% \]

% \textbf{Update}: I think we should be fine here if we assume that support of \(\zeta\) is bounded and the support of \(\xi\) is contained strictly inside \((0,1)\). Then if we look at the discrete time dynamics in \(X\) then we obtain 
% \[
% X_{i}(n+1) = (1-\xi_i)X_i(n) + \zeta(n+1) h(X_n,P_n)+\mu M_{n}
% \]

% }
Observe that for any \(i\in[\numLinks]\),  \(\{\martingale_i(n+1)\}_n\) in \eqref{eq: MartingaleDefinition} is a martingale difference sequence with respect to the filtration \(\filtration_n = \sigma(\cup_{i\in[\numLinks]} \lr{\flowDiscrete_i(1),\inflow(1),\outflow_i(1),\dots,\flowDiscrete_i(n),\inflow(n),\outflow_i(n)} )\). Using the definition of martingale difference sequence \(\martingale_{i}(n+1)\) and assumptions on random variables $\{\inflow_i(n)\}_{n \in \mathbb{N}}$ and $\{\outflow(n)\}_{n \in \mathbb{N}}$ one can observe that there exists a finite scalar \(K>0\) such that 
\begin{align}\label{eq: martingaleBound}
    \avg[|\martingale_i(n+1)|^2|\filtration_n] \leq K\lr{1+\|\flowDiscrete_i(n)\|^2} \quad \forall i, n.
\end{align}


% The aim, now, is to understand whether the coupled stochastic process converges and to explicate its limiting behavior, with a goal towards showing asymptotic convergence to socially optimal flows. 

Our assumption that the random variables \(\inflow(n),\outflow(n)\)  have finite support ensures that  \(\flowDiscrete_n,\priceDiscrete_n\) in \eqref{eq: CombinedDT} are bounded almost surely. Specifically, \(\flowDiscrete_n\in\lr{0,\frac{\inflowUpper}{\outflowLower}}\) almost surely. This ensures that the vector fields in \eqref{eq: singularPerturbedODE}  are Lipschitz functions (as they take bounded sets to bounded sets).

We can therefore deploy the machinery of constant step-size two-timescale stochastic approximation presented in \cite[p. 112]{borkar2009stochastic}. 

\begin{theorem}\label{thm: BorkarSAConvergence}
The iterates of the stochastic process \eqref{eq: CombinedDT} will satisfy the following 
\begin{align}
    \limsup_{n\ra+\infty}\avg[\|\flowDiscrete_n-\fixedPointFlow(\fixedPointPrice)\|^2+\|\priceDiscrete_n-\fixedPointPrice\|^2] = \mathcal{O}(\meanOutflow)+\mathcal{O}\lr{\frac{a}{\meanOutflow}}.
\end{align}
\end{theorem}
\begin{proof}
The proof of the above theorem follows by observing that the modelling assumptions posited in \S\ref{sec: Model} and the properties of approximating continuous time dynamical system derived in \S\ref{ssec: PropFixedPoint}-\S\ref{ssec: Convergence} satisfies all the standard hypothesis of constant step size two time scale stochastic approximation theory (refer \cite[p. 112]{borkar2009stochastic}). 
\end{proof}



==> Dynamic_Routing_Regular (Arxiv)/results_arxiv.tex <==
\section{Main Results}\label{sec: Results}
In Sec. \ref{subsec:fixed_point}, we present a continuous-time deterministic dynamical system that is associated with the discrete-time updates \eqref{eq: FlowDynamics} and \eqref{eq: PricingDynamics}. We show that the flow of the continuous-time dynamical system has a unique fixed point that corresponds to the perturbed socially optimal load (refer Definition \ref{def:perturbed_opt}) and the socially optimal tolling. %\textcolor{red}{steady-state stochastic user equilibrium} 
% associated with the fixed point toll price, and it minimizes the social cost as $\beta \to \infty$. 
In Sec. \ref{ssec: ConvergenceDiscrete}, we apply the two timescale stochastic approximation theory to show that $\left(\flowDiscrete(n), P(n)\right)$ in the
%the states of our 
discrete-time stochastic updates concentrate on a neighborhood of the fixed point of the flow of the continuous-time dynamical system. Therefore, our dynamical tolling eventually induces a {perturbed socially optimal load vector} with high probability. %we prove the main result of the paper -- under the setup presented in \S\ref{sec: Model} the combined flow-toll price update \eqref{eq: CombinedDT} asymptotically concentrate in a neighborhood around the socially optimal flows and prices with high probability. One of the major contributions here is to show that the trajectories of the ``natural'' continuous-time dynamical system, associated with the stochastic process  \eqref{eq: CombinedDT}, converges to the socially optimal loadand toll prices. We, then, employ the machinery from two-timescale constant step size stochastic approximation to bridge the connection between the continuous-time dynamical system and discrete-time stochastic process. 

\subsection{Continuous-time dynamical system}\label{subsec:fixed_point}
We first introduce a \emph{deterministic} continuous-time dynamical system that {corresponds to} \eqref{eq: FlowDynamics} -- \eqref{eq: PricingDynamics}. The time evolution in continuous-time dynamical system is denoted by \(t\) and it is related with the discrete-time step \(n\) as \(t=an\), where \(a\) is the stepsize in \eqref{eq: PricingDynamics}. We define $x(t) \in \mathbb{R}^{\numLinks}$ as the load vector and $p(t) \in \mathbb{R}^{\numLinks}$ as the toll vector at time $t \in [0, \infty)$ 
%\textcolor{red}{(I suggest to use "time step" for discrete step $n$ and "time" for continuous-time $t$)}.
We also define \(\stepRatio \defas \frac{\stepPrice}{\meanOutflow} \), where $\meanOutflow$ (resp. $\stepPrice$) is the stepsize of the discrete-time load update (resp. toll update). Since the toll update occurs at a slower timescale compared to the load update (i.e. $\stepPrice \ll \meanOutflow$), we have $\stepRatio \ll 1$. % between loadand toll prices. Furthermore, for any \(x,p\in \R^{\numLinks}\) define 

The continuous-time dynamical system is as follows: 
%Consider the following continuous-time dynamical system, that we expect should closely follow \eqref{eq: CombinedDT}, 
\begin{equation}\label{eq: singularPerturbedODE}
    \begin{aligned}
    \dot{\flowContinuous}_i(t) &= \frac{1}{\stepRatio}\lr{\vectorFieldX_i(\flowContinuous(t),\priceContinuous(t)) - \flowContinuous_i(t)}, \\ 
    \dot{\priceContinuous}_i(t) &= -\priceContinuous_i(t) + \flowContinuous_i(t)
    \frac{d \ell_i(\flowContinuous_i(t))}{d x}, \quad \forall \ t \geq 0.
    \end{aligned}
\end{equation}
%The assumption \(\epsilon\ll 1\) ensures that \(x(t)\) is a fast transient while \(p(t)\) is the slow component. 


% \footnote{With slight abuse of terminology we refer to the fixed point of the flow here as the equilibrium of the continuous-time dynamical system.} 
% 
We introduce the following two definitions: 
\begin{definition}\label{def:generalized_SUE}{(\textbf{Stochastic user equilibrium})}
 For any fixed \(p\in \R^{\numLinks}\), a load vector $\fixedPointFlow(\priceContinuous)$\footnote{We explictly state the dependence on \(p,\beta\) in order relate the definition to later results.} is the stochastic user equilibrium corresponding to 
%  a {dispersion parameter} \(\beta\in[0,\infty)\) and 
the toll vector $\priceContinuous$ and demand $\frac{\meanInflow}{\meanOutflow}$ if for all \(i\in[\numLinks]\):
 \begin{align}\label{eq: xEquilibrium}
    \fixedPointFlow_i(\priceContinuous) = 
    %\vectorFieldX_i(\fixedPointFlow(\priceContinuous),\priceContinuous) =
    \frac{\meanInflow}{\meanOutflow}\frac{\exp(-\sueParameter \costPrice_i(\fixedPointFlow_i(\priceContinuous),\priceContinuous_i))}{\sum_{j\in[R]}\exp(-\sueParameter \costPrice_j(\fixedPointFlow_j(\priceContinuous),\priceContinuous_j))}.
\end{align}
\end{definition}
Given the stochastic user equilibrium in \eqref{eq: xEquilibrium}, all travelers with total demand of $\lambda/\mu$ make routing decisions in the network according to a perturbed best response given the latency functions on links and tolls $p$. We note that demand $\lambda/\mu$ is the expected value of the total demand in network at step $n$ when $n \uparrow \infty$. This is because in each step $n$, the expected value of the total demand in network is $\sum_{m=1}^{n}(1-\mu)^{n-m}\lambda$, where \((1-\mu)^{n-m}\lambda\) is the expected incoming demand in step $m$ that remains in the network in step $n$. Thus, as $n \uparrow \infty$, the expected value of the total demand is $\lambda/\mu$. 

%At any time step \(n\), the average load on network is \(\sum_{m=1}^{n}(1-\mu)^{m-1}\lambda\). Thus as \(n\uparrow \infty\) the total load on network is \(\frac{\lambda}{\mu}\). From the perspective of static one-shot routing the total load \(\frac{\meanInflow}{\meanOutflow}\) can be understood as incoming load that needs to be routed on an empty network. Thus, with slight abuse of terminology we refer \(\fixedPointFlow(p)\) as stochastic user equilibrium in our dynamic setting.

%Note that \(\fixedPointFlow(p)\) is the load corresponding to the static one-shot stochastic user equilibrium with incoming demand of \(\frac{\meanInflow}{\meanOutflow}\). This is also the \textit{stationary demand} on the network in the dynamic setting introduced above when the incoming load $\flowIn_i(n)$ and outgoing load $\flowOut_i(n)$ are the same. \textcolor{red}{mean incoming load \(\meanInflow\) and mean outgoing load $\meanOutflow$ are the same}. For any \(p\in\R^{\numLinks}\), the load \(\fixedPointFlow(p)\) allocates smaller load on the links with higher cost.
%Note that the Definition \ref{def:generalized_SUE} corresponds to the standard definition of stochastic user equilibrium \cite{cominetti2012modern} but with an \emph{equivalent demand} of \(\frac{\meanInflow}{\meanOutflow}\).
%We call it stochastic user equilibrium with stationary network throughput as it is the fixed point of the flow of the continuous-time dynamical system \eqref{eq: singularPerturbedODE}. 
%But for the subsequent exposition, for the sake of conciseness we shall simply call the  -- stochastic user equilibrium with stationary network throughput -- as stochastic user equilibrium. 
\begin{definition}\label{def:perturbed_opt}(\textbf{Perturbed socially optimal load})
A load vector $\bar{y}^{(\beta)}$ is a perturbed socially optimal load if $\bar{y}^{(\beta)}$ minimizes the following convex optimization problem: 
\begin{equation}\label{eq: SocialCostWE}
\begin{aligned}
    \min_{y\in \R^{\numLinks}} &\quad \sum_{i\in[\numLinks]} y_i\costEdge_i(y_i) + \frac{1}{\beta}\sum_{i\in[\numLinks]} y_i\log(y_i) \\
    \text{s.t} & \quad \sum_{i\in[\numLinks]} y_i = \frac{\meanInflow}{\meanOutflow}.
\end{aligned}
\end{equation}
\end{definition}
A commonly used notion to quantify the social objective is the total latency experienced on the network \cite{roughgarden2010algorithmic,farokhi2015piecewise}.  
Note that \eqref{eq: SocialCostWE} is an \emph{entropy} regularized social objective function where the regularization weight depends on \(\beta\). As \(\beta \uparrow \infty\), the perturbed socially optimal load \(\bar{y}^{(\beta)}\) becomes the socially optimal flow, which minimizes the total latency. 
 %Owing to  the assumption \(\stepRatio<<1\) we see that \(\flowContinuous(\cdot)\) is a ``fast'' dynamics while \(\priceContinuous(\cdot)\) is a comparatively ``slower'' component. Therefore we can consider \(\priceContinuous(\cdot)\) ``static'' while analyzing the behavior of \(\flowContinuous(\cdot)\). We therefore first consider the following dynamical system for any fixed \(\priceContinuous\in\R^{\numLinks}\):
 
 The following theorem shows that the flow of the continuous-time dynamical system has a unique fixed point, and this fixed point corresponds to the perturbed socially optimal load.
 \begin{theorem}\label{theorem: fixed_point}
 The flow of the continuous-time dynamical system \eqref{eq: singularPerturbedODE} has a \emph{unique} fixed point $(\fixedPointFlow(\fixedPointPrice), \fixedPointPrice)$ such that $\fixedPointFlow(\fixedPointPrice)$ is a stochastic user equilibrium corresponding to $\fixedPointPrice$, and 
 \begin{align}\label{eq: pEquilibrium}
    \fixedPointPrice_i = \fixedPointFlow_i(\fixedPointPrice) \frac{ d \costEdge_i(\fixedPointFlow_i(\fixedPointPrice))}{d x}.
\end{align}
Moreover, $\fixedPointFlow(\fixedPointPrice)$ is the perturbed socially optimal load. 
 \end{theorem}

At $(\fixedPointFlow_i(\fixedPointPrice), \fixedPointPrice)$, the load on the network is a stochastic user equilibrium given $\fixedPointPrice$ and demand $\lambda/\mu$. This implies that travelers' routing strategy, when averaged over all time steps, is a perturbed best response given $\fixedPointPrice$ and $\lambda/\mu$. Moreover, the unique price vector $\fixedPointPrice$ is the marginal latency cost, which ensures that the stochastic user equilibrium $\fixedPointFlow(\fixedPointPrice)$ is also a perturbed socially optimal load. As $\beta \to \infty$, $\fixedPointFlow(\fixedPointPrice)$ becomes a socially optimal load.  


%The fixed point of the flow of the continuous-time dynamical system \ref{eq: singularPerturbedODE} has a  game theoretic significance. Specifically, for every fixed $\fixedPointPrice$, the equilibrium $\fixedPointFlow_i(\fixedPointPrice)$ is such that loads are picked according to a stochastic user equilibrium under equivalent demand $\meanInflow/ \meanOutflow$. Further, the toll $\fixedPointPrice$ has as its fixed point the \textit{marginal cost price}.


We prove Theorem \ref{theorem: fixed_point} in three parts: Firstly, we show that for any toll vector $\priceContinuous\in \R^{\numLinks}$, the stochastic user equilibrium $\fixedPointFlow(\priceContinuous)$ exists and is unique, and can be solved as the optimal solution of a convex optimization problem (Lemma \ref{lemma:gStochasticEquilibrium}). Secondly, we show that there exists a unique toll vector $\fixedPointPrice$ that satisfies \eqref{eq: pEquilibrium} (Lemma \ref{lemma:unique_price}). This requires us to prove that the stochastic user equilibrium $\fixedPointFlow(\priceContinuous)$ is monotonic in $\priceContinuous$ (Lemma \ref{lemma:monotonicity} ). Finally, we conclude the theorem by proving that at $\fixedPointPrice$ the stochastic user equilibrium $\fixedPointFlow(\fixedPointPrice)$ is the perturbed socially optimal load (Lemma \ref{lemma:optimality}).  


We now present the lemmas that are referred in each of the parts above, and provide the proof ideas of these results. We include the formal proofs in Appendix \ref{appsec: ProofLemma}. 
% {\color{blue}
% \begin{lemma}\label{lemma:twotimescale}
% For any $\epsilon \ll 1$, a state $(\fixedPointFlow, \fixedPointPrice)$ is a fixed point of \eqref{eq: singularPerturbedODE} if and only if $\fixedPointFlow$ is a steady-state stochastic user equilibrium corresponding to $\fixedPointPrice$, and $\fixedPointPrice$ satisfies \eqref{eq: pEquilibrium}. 
% \end{lemma}
% }


\emph{Part 1:} For any $p$, the load vector $\fixedPointFlow(p)$ is the unique stochastic user equilibrium. 
\begin{lemma}\label{lemma:gStochasticEquilibrium}
For every \(\priceContinuous\in \R^{\numLinks}\), \(\fixedPointFlow(\priceContinuous)\) is the unique optimal solution to the following convex optimization problem:
% (also known as the stochastic user equilibrium (SUE) problem \cite{cominetti2012modern})
 \begin{equation}\label{eq: OptimizationProblemRevised}
\begin{aligned}
    \min_{y\in \R^{\numLinks}} & \quad  \sum_{i\in [\numLinks]} \int_{0}^{y_i} \costPrice_i(s,p_i)ds + \frac{1}{\beta} \sum_{i\in [\numLinks]} y_i \ln{y_i}, \\
    \text{s.t} & \quad \sum_{i\in[\numLinks]} y_i = \frac{\meanInflow}{\meanOutflow}%\quad k(y)\defas.
\end{aligned}
\end{equation}
\end{lemma}
 

The proof of Lemma \ref{lemma:gStochasticEquilibrium} follows by verifying that \(\fixedPointFlow(p)\) (refer Definition \ref{def:generalized_SUE}) satisfies the Karush–Kuhn–Tucker (KKT) conditions corresponding to \eqref{eq: OptimizationProblemRevised}, which is strictly convex problem and therefore has unique solution. We note that as $\beta \to \infty$, the stochastic user equilibrium $\fixedPointFlow(p)$ becomes a Wardrop equilibrium, where travelers only take routes with the minimum cost. 


\emph{Part 2:} We first show that the stochastic user equilibrium $\fixedPointFlow(p)$ is monotonic in $p$. This allows us to prove the existence and uniqueness of $\fixedPointPrice$ given by \eqref{eq: pEquilibrium}.  
\begin{lemma}\label{lemma:monotonicity}(\textbf{Monotonicity of $\fixedPointFlow(\priceContinuous)$})
For any \(p,p'\in\R^{\numLinks}\) we have 
\[\lara{ \fixedPointFlow(p)-\fixedPointFlow(p'),p-p' }<0. \]
Furthermore, \(\fixedPointFlow(p)\) is a continuously differentiable function. Consequently, \(\frac{\partial \fixedPointFlow_i(\priceContinuous)}{\partial \priceContinuous_i} < 0\) for all \(i\in[\numLinks]\). 
\end{lemma}
The proof of Lemma \ref{lemma:monotonicity} is proved by using the variational inequalities of stochastic user equilibrium, which are the first-order optimality condition associated with \eqref{eq: OptimizationProblemRevised}. Moreover, the monotonicity property relies on the fact that the latency on each link increases in the load. 
 
 

\begin{lemma}\label{lemma:unique_price}(\textbf{Existence and uniqueness of $\fixedPointPrice$})
The price vector $\fixedPointPrice$, defined in \eqref{eq: pEquilibrium}, exists and is unique. 
\end{lemma}
In Lemma \ref{lemma:unique_price} the  existence is proved by using the Brouwer's fixed point theorem. We prove uniqueness by contradiction. More formally, let \({p},{p}'\in \R^{\numLinks}\) be two distinct toll vectors that satisfy \eqref{eq: pEquilibrium}. Then, from \eqref{eq: pEquilibrium}, we know that for every \(i\in[\numLinks]\):
\begin{align}
    \fixedPointPrice_i - \fixedPointPrice_i' 
    &= \lr{\fixedPointFlow_i( p)-\fixedPointFlow_i(p')}   \frac{d \costEdge_i(\fixedPointFlow_i(p))}{dx}\notag\\&\quad\quad +\fixedPointFlow_i(p')\lr{\frac{ d \costEdge_i(\fixedPointFlow_i(p))}{dx}-\frac{d \costEdge_i(\fixedPointFlow_i(p'))}{dx}}.\label{eq:contradiction}
\end{align}
By multiplying  both sides of \eqref{eq:contradiction} by \((\fixedPointFlow_i(p)-\fixedPointFlow_i(p'))\),and summing over all \(i\in[\numLinks]\), we have
\begin{align*}
    \lara{ \fixedPointFlow(p)-\fixedPointFlow(p'), p-p' } \geq 0, 
\end{align*}
which contradicts the monotonicity condition proved in Lemma \ref{lemma:monotonicity}. Therefore, the price $\fixedPointPrice$ is unique. 

\emph{Part 3:} Finally, we prove that given $\fixedPointPrice$, $\fixedPointFlow(\fixedPointPrice)$ is a perturbed socially optimal load. 
\begin{lemma}\label{lemma:optimality}
The load vector $\fixedPointFlow(\fixedPointPrice)$ is the perturbed socially optimal load. 
\end{lemma}
We prove Lemma \ref{lemma:optimality} by showing that the variational inequality satisfied by the stochastic user equilibrium at \(\fixedPointPrice\) is identical to that satisfied by the perturbed socially optimal load. % associated with \eqref{eq: OptimizationProblemRevised} when evaluated at the toll \(\fixedPointPrice\) (which satisfies \eqref{eq: pEquilibrium}) is the same as the variational inequality associated with \eqref{eq: SocialCostWE}. 

Lemmas \ref{lemma:gStochasticEquilibrium} -- \ref{lemma:optimality} conclude Theorem \ref{theorem: fixed_point}. 
\subsection{Convergence}\label{ssec: ConvergenceDiscrete}
In this section, we show that $(\flowDiscrete_i(n), \priceDiscrete_i(n))$ induced by the discrete-time stochastic update converges to a {neighborhood} of $(\fixedPointFlow(\fixedPointPrice), \fixedPointPrice)$. The size of the neighborhood depends on the load update stepsize $\mu$ and the stepsize ratio between the two dynamics $a/\mu$. That is, the tolls eventually induce a perturbed socially optimal flow.


\begin{theorem}\label{theorem:discrete_convergence}
\begin{align}\label{eq: discreteNeighborhood}
    \limsup_{n\ra+\infty}\avg[\|\flowDiscrete_n-\fixedPointFlow(\fixedPointPrice)\|^2+\|\priceDiscrete_n-\fixedPointPrice\|^2] = \mc{O}\lr{\meanOutflow+\frac{a}{\meanOutflow}}.
\end{align}
Moreover, for any \(\delta>0\):
\begin{align}\label{eq:probability_neighborhood}
    \limsup_{n\ra+\infty}\Pr(\|\flowDiscrete_n-\fixedPointFlow(\fixedPointPrice)\|^2+\|\priceDiscrete_n-\fixedPointPrice\|^2 \geq \delta) \leq \mc{O}\lr{\frac{\mu}{\delta}+\frac{a}{\delta \mu}}. 
\end{align}
\end{theorem}

In Theorem \ref{theorem:discrete_convergence}, \eqref{eq: discreteNeighborhood} provides the neighborhood of the socially optimal load and tolls, where the discrete-time stochastic updates converge to in expectation. In particular, as the step size \(\mu\) and the stepsize ratio between the two updates \(\epsilon = a/\mu\) decreases (i.e. the discrete-time step for load update is small, and the toll update is much slower than the load update), the expected value of the distance between $(\flowDiscrete(n), \priceDiscrete(n))$ and $(\fixedPointFlow(\fixedPointPrice), \fixedPointPrice)$ decreases for $n \to \infty$. Moreover, by 
applying the Markov's inequality, \eqref{eq: discreteNeighborhood} also implies that for any neighborhood of $(\fixedPointFlow(\fixedPointPrice), \fixedPointPrice)$, $(\flowDiscrete(n), \priceDiscrete(n))$ converges to that neighborhood with high probability, and this probability increases as $\mu$ and $\epsilon$ decreases.  

%and as a result with high probability. Note that decreasing  provides tighter bound. 

To prove Theorem \ref{theorem:discrete_convergence}, we need to prove the following technical lemma: 
\begin{lemma}\label{lemma: prep}
\hfill %In \eqref{eq: FlowDynamics} -- \eqref{eq: PricingDynamics}, the following conditions are satisfied:
\begin{itemize} 
    \item[\textbf{(C1)}] For all \( i\in[\numLinks]\),  \(\{\martingale_i(n+1)\}_n\) in \eqref{eq: MartingaleDefinition} is a martingale difference sequence with respect to the filtration \(\filtration_n = \sigma(\cup_{i\in[\numLinks]} \lr{\flowDiscrete_i(1),\inflow(1),\outflow_i(1),\dots,\flowDiscrete_i(n),\inflow(n),\outflow_i(n)} )\)
    \item[\textbf{(C2)}] For all \( i\in[\numLinks]\),  \(X_i(n) \in \lr{0,\flowDiscrete_i(0)+\frac{\inflowUpper}{\outflowLower}}\). Consequently, \(\avg[\|X(n)\|^2]<+\infty\), \(\avg[\|P(n)\|^2] <+\infty\).
    \item[\textbf{(C3)}] There exists \( K >0\) such that for any $i \in [R]$ and any $n$,  \(\avg[|\martingale_i(n+1)|^2|\filtration_n] \leq K\lr{1+\|\flowDiscrete_i(n)\|^2} <+\infty.\)
    \item[\textbf{(C4)}] For any $p$, any $\tilde{x}(t): \mathbb{R}_{\geq 0} \to \mathbb{R}^{\numLinks}$ induced by following continuous-time dynamical system
    \begin{equation}
\begin{aligned}\label{eq: FixedPointFlowDynamics}
    \dot{\flowContinuousNew}_i(t) &= \vectorFieldX_i(\flowContinuousNew(t),p) -\flowContinuousNew_i(t), \quad \quad \forall i \in [\numLinks], \forall \ t\geq 0,
\end{aligned}
\end{equation}
satisfies $\lim_{t \to \infty}\tilde{x}(t)=\fixedPointFlow(p)$. Futhermore, \(\fixedPointFlow(p)\) is Lipschitz.
\item[\textbf{(C5)}] Any $\tilde{p}(t): \mathbb{R}_{\geq 0} \to \mathbb{R}^\numLinks$ induced by following continuous-time dynamical system
\begin{align}\label{eq: PriceDynamicsTilde}
    \dot{\priceContinuousNew}_i(t) = -\priceContinuousNew_i(t)+\fixedPointFlow_i(\priceContinuousNew(t))\frac{d  \costEdge_i(\fixedPointFlow_i(\priceContinuousNew(t)))}{d x}, \quad t\geq 0,
\end{align}
satisfies $\lim_{t \to \infty} \priceContinuousNew(t) = \fixedPointPrice$.
\end{itemize}
\end{lemma}

In Lemma \ref{lemma: prep}, condition \textbf{(C1)} relies on the fact that both the incoming and outgoing loads are i.i.d.. Condition \textbf{(C2)} ensures the boundedness of the loads and the tolls in the discrete-time stochastic updates, and it relies on the boundedness of $\inflow_n$ and $\outflow_n$. Condition \textbf{(C3)} ensures the boundedness of the martingale sequence $\{M_i(n+1)\}_n$, and it is built on condition \textbf{(C1)} and \textbf{(C2)}. 

In conditions \textbf{(C4)}, the continuous-time dynamical system \eqref{eq: FixedPointFlowDynamics} is associated with the discrete-time load update \eqref{eq: FlowDynamics} when the toll is set as a constant $p$. That is, due to the fact that toll update is at a slower timescale compared with the load update ($\epsilon \ll 1$), the continuous-time dynamical system of load evolves as if the toll is a constant $p$. We prove condition \textbf{(C4)} by showing that \eqref{eq: FixedPointFlowDynamics} is cooperative (see Theorem \ref{thm: HirshResult} in the appendix). Condition \textbf{(C4)} ensures that the load of the continuous-time dynamical system converges to the stochastic user equilibrium (Definition \ref{def:generalized_SUE}) with respect to \(p\). Recall from Lemma \ref{lemma:gStochasticEquilibrium}, the stochastic user equilibrium is unique. 


On the other hand, in condition \textbf{(C5)}, \eqref{eq: PriceDynamicsTilde} is associated with \eqref{eq: PricingDynamics} when the load -- which is updated at a faster timescale -- has already converged to the stochastic user equilibrium with respect to $p(t)$. Similar to condition \textbf{(C4)}, we show that \eqref{eq: PriceDynamicsTilde} is a cooperative dynamical system. The proof of this condition is built on the monotonicity of stochastic user equilibrium with respect to the toll (Lemma \ref{lemma:monotonicity}) and the uniqueness of $\fixedPointPrice$ (Lemma \ref{lemma:unique_price}). The proofs of \textbf{(C1)} -- \textbf{(C5)} are in Appendix \ref{appsec: ProofLemma}.  


 

%apply the theory of two timescale  stochastic approximation with constant stepsize \cite{borkar2009stochastic}. To begin with, we note that for any \(i\in[\numLinks]\),  \(\{\martingale_i(n+1)\}_n\) in the discrete-time stochastic updates \eqref{eq: MartingaleDefinition} is a martingale difference sequence with respect to the filtration \(\filtration_n = \sigma(\cup_{i\in[\numLinks]} \lr{\flowDiscrete_i(1),\inflow(1),\outflow_i(1),\dots,\flowDiscrete_i(n),\inflow(n),\outflow_i(n)} )\). Using the definition of martingale difference sequence \(\martingale_{i}(n+1)\) and assumptions on random variables $\{\inflow_i(n)\}_{n \in \mathbb{N}}$ and $\{\outflow(n)\}_{n \in \mathbb{N}}$ there exists a finite scalar \(K>0\) such that 
% \begin{align}\label{eq: martingaleBound}
%     \avg[|\martingale_i(n+1)|^2|\filtration_n] \leq K\lr{1+\|\flowDiscrete_i(n)\|^2} \quad \forall i, n.
% \end{align}
%Furthermore, note that for every \(i\in[\numLinks]\),  \(X_i(n) \in \lr{0,\frac{\inflowUpper}{\outflowLower}}\) and therefore \(\avg[\|X(n)\|^2]<+\infty\). Boundedness of \(X(n)\) in turn implies boundedness of \(P(n)\). Therefore, \(\avg[\|P(n)\|^2] < +\infty\). 

Based on Lemma \ref{lemma: prep}, we can apply the theory of two timescale stochastic approximation with constant stepsizes: 
\begin{lemma}[\cite{borkar2009stochastic}]\label{lemma: borkar}
Given $\epsilon \ll 1$, \eqref{eq: discreteNeighborhood} is satisfied under \textbf{(C1)} -- \textbf{(C5)}. 
\end{lemma}

Lemmas \ref{lemma: prep} and \ref{lemma: borkar} proves \eqref{eq: discreteNeighborhood}. Additionally, \eqref{eq:probability_neighborhood} can be directly derived from \eqref{eq: discreteNeighborhood} using the Markov's inequality. Thus, we can conclude Theorem \ref{theorem:discrete_convergence}. 


\begin{comment}
suggests that if the aforementioned properties of discrete-time stochastic updates hold then in order to establish the convergence of \((\flowDiscrete_i(n), \priceDiscrete_i(n))\) it is sufficient to study the convergence of the flow of \eqref{eq: singularPerturbedODE}. As we assume \(\epsilon\ll1\), we consider \(p(\cdot)\) to be quasi-static while analysing the behavior of \(x(\cdot)\). More formally, consider the following continuous-time dynamical system for any \(p\in \R^{\numLinks}\):
\begin{equation}
\begin{aligned}\label{eq: FixedPointFlowDynamics}
    \dot{\flowContinuousNew}_i(t) &= \vectorFieldX_i(\flowContinuousNew(t),p) -\flowContinuousNew_i(t), \quad \quad \forall i \in [\numLinks], \forall \ t\geq 0.
\end{aligned}
\end{equation}
Note that the fixed point of the flow of \eqref{eq: FixedPointFlowDynamics} is \(\fixedPointFlow(p)\). We show  that trajectories of \eqref{eq: FixedPointFlowDynamics} converges to \(\fixedPointFlow(p)\) (Lemma \ref{lemma: XdynamicsConvergence}). This suggests that the fast transient \(x(\cdot)\), in \eqref{eq: singularPerturbedODE}, will follow \(\fixedPointFlow(p(t))\) for $\epsilon \ll 1$.
%Furthermore, since \(\fixedPointFlow(p)\) is bounded and continuous it is Lipschitz. 

Thus to show convergence of \eqref{eq: singularPerturbedODE} it sufficient to argue about the convergence of the following continuous-time dynamical system:
\begin{align}\label{eq: PriceDynamicsTilde}
    \dot{\priceContinuousNew}_i(t) = -\priceContinuousNew_i(t)+\fixedPointFlow_i(\priceContinuousNew(t))\frac{d  \costEdge_i(\fixedPointFlow_i(\priceContinuousNew(t)))}{d x}, \quad t\geq 0,
\end{align}
for every \(i\in[\numLinks]\).
Note that the fixed point of the flow of \eqref{eq: PriceDynamicsTilde} is \(\fixedPointPrice\) (refer \eqref{eq: pEquilibrium}). We show that trajectories of \eqref{eq: PriceDynamicsTilde} converges to \(\fixedPointPrice\) (Lemma \ref{lemma: pDynamicsConvergence}). This establishes that the flow of \eqref{eq: singularPerturbedODE} will converge to its fixed points. This in turn imply that discrete-time stochastic updates will converge in neighborhood of these fixed points.  

% In summary, the assertion in Theorem \ref{theorem:discrete_convergence} holds, as all the hypotheses of \cite[Chapter 9]{borkar2009stochastic} hold true. 

We now present the lemmas that are referred in this subsection, and provide the proof ideas of these results. We include the formal proof in \cite{driveVersion} due to space considerations. 
% \textcolor{red}{first... (Lemma \ref{}) In this part, we apply the theory of two-timescale stochastic approximation.} Then, we show that the the continuous-time dynamical system \eqref{eq: singularPerturbedODE} converges to the unique fixed point $(\fixedPointFlow, \fixedPointPrice)$ (Lemma \ref{lemma: ConvergenceFlowCont}) . Therefore, \textcolor{red}{we can conclude that  ...}

\begin{lemma}\label{lemma: XdynamicsConvergence}
For any \(p\in\R^{\numLinks}\), the trajectories of \eqref{eq: FixedPointFlowDynamics},  starting from any initial conditions, satisfy $\lim_{t \to \infty} \flowContinuousNew(t) = \fixedPointFlow(p)$.
\end{lemma}
The proof of Lemma \ref{lemma: XdynamicsConvergence} follows by verifying that the dynamical system \eqref{eq: FixedPointFlowDynamics} is cooperative \cite{hirsch1985systems}(refer Appendix \ref{appsec: Cooperative} for theorem statement). 

\begin{lemma}\label{lemma: pDynamicsConvergence}
The trajectories of \eqref{eq: PriceDynamicsTilde},  starting from any initial conditions, satisfy $\lim_{t \to \infty} \priceContinuousNew(t) = \fixedPointPrice$.
\end{lemma}
The result in Lemma \ref{lemma: pDynamicsConvergence} also follows by showing that the dynamical system \eqref{eq: PriceDynamicsTilde} is cooperative. One of the crucial steps in attesting the cooperative nature of the dynamical system \eqref{eq: PriceDynamicsTilde} is to prove \(\frac{\partial \fixedPointFlow_i(p) }{\partial p_j} > 0\) for \(i\neq j \in [n]\). This is a non-trivial step as we do not have an explicit expression of \(\fixedPointFlow(p)\); it is implicitly defined in \eqref{eq: xEquilibrium}. The algebraic details of the proof are defered to \cite{driveVersion}. 

\end{comment}
% \color{red}
% We proof this lemma by applying \textcolor{red}{the theory of cooperative dynamics} from \cite{hirsch1985systems}. We provide a brief review here for the sake of completeness. 

% %  For this purpose we use results  which is also stated in Theorem \ref{thm: HirshResult} for the sake of completeness.
 
% %  In this section we review a result from \cite{hirsch1985systems} which provides an easily verifiable requirement on the vector field which ensures convergence to equilibrium.  

% Consider a \(C^1-\)vector field \(f:\R^n\rightarrow \R^n\) and the dynamical system 
% \begin{align}\label{eq: DynSys}
% \dot{x}(t) = f(x(t))
% \end{align}
% where
% \begin{enumerate}%[label=(P-\roman*)]
%     \item \label{enum: Assm1} for any \(i\neq j \in [n]\) and \(x\in \R^n\) we have \(\frac{\partial f_i(x)}{\partial x_j} \geq 0\); 
%     \item \label{enum: Assm2} the Jacobian matrix \(\nabla f(x)\) is irreducible;\footnote{Define irreducible here}
%     \item \label{enum: Assm3} for every \(i\in[n]\), \(f_i(0)\geq 0\);
%     \item \label{enum: Assm4} for any \(x\in\Rp^n\) there exists \(y > x\) with \(f_i(y) < 0\) for all \(i\in[n]\)
%  \end{enumerate}
%  \begin{theorem}[{\cite[Theorem 5.1]{hirsch1985systems}}]\label{thm: HirshResult}
%  Let the dynamical system \eqref{eq: DynSys} satisfy the assumptions \ref{enum: Assm1}-\ref{enum: Assm4}. Then \(\Rp^n\) is positively-invariant and trajectories starting almost everywhere in \(\Rp^n\) converge to the set \(\{x: f(x) = 0\}\).  
%  \end{theorem}
 
%  Based on Theorem \ref{thm: HirshResult}, we prove Lemma \ref{lemma: ConvergenceFlowCont} by verifying that both the continuous-time dynamics \eqref{eq: singularPerturbedODE} satisfies assumptions \ref{enum: Assm1}-\ref{enum: Assm4}. 
%  \color{black}





==> Dynamic_Routing_Regular (Arxiv)/setup.tex <==
\section{Setup}
We now introduce the time-dynamical model that models inflows and outflows on the network, along with an adaptive tolling scheme. We show that over time, the tolling scheme converges to a price that induces a socially optimal flow, as in the sense of minimizing the function in \ref{thm: SocialCost}.


There is an $\numLinks$-link parallel network and a pair of nodes connecting them. At every time $n \in \mathbb{N}$, there is $\flowDynamic_i(n)$ units of flow present on the $i$-th link. Each link is endowed with a cost function $\costLink_i(\cdot, \cdot) :\mathbb{R} \times \mathbb{R} \rightarrow \mathbb{R}$.  For any link \(i\in[\numLinks]\) and \(n\in\N\) the toll prices are denoted by $\priceDynamic_i(n) \in \mathbb{R}$. Therefore, $C_i$ is now a function of both the flow and the price on each link $i$.

\begin{assumption}
$C_i(\cdot, \cdot)$ is increasing in both arguments and convex in the first. 
\end{assumption}


\subsection{Routing Dynamics}
We consider the following routing dynamics and study the convergence of the flow process to a socially optimal profile. : 
\begin{align}
\flowDynamic_i(n+1) & = 
\flowDynamic_i(n) + 
\frac{\exp(-\beta 
\costLink_i(\flowDynamic_i(n), 
\priceDynamic_i(n)))}{\sum_{j=1}^{R}  \exp (-\beta 
\costLink_j(\flowDynamic_j(n), 
\priceDynamic_j(n)))} \zeta(n+1) - 
\xi_i(n+1) \flowDynamic_i(n) \\ &= 
\flowDynamic_i(n) + \mu \left( 
\frac{\lambda}{\mu} 
\frac{\exp(-\beta 
\costLink_i(\flowDynamic_i(n), 
\priceDynamic_i(n)))}{\sum_{j=1}^{R}  \exp (-\beta\costLink_j( 
\flowDynamic_j(n), 
\priceDynamic_j(n)))} - 
\flowDynamic_i(n) \right) + \mu M_i(n+1) \\
\priceDynamic_i(n+1) &= (1-a)\priceDynamic_i(n) + a  \flowDynamic_i(n) \frac{\partial C_i}{\partial x_i}(\flowDynamic_i(n), \priceDynamic_i(n))
\end{align}
We define the basic quantities used in the routing dynamic:

\begin{definition} 
The function
\begin{align}
    (X_i(n), P_i(n)) \rightarrow \frac{\exp(- \beta C_i(X_i(n), P_i(n))}{\sum_{j=1}^{R} \exp(-\beta C_i(X_i(n), P_i(n)))}
\end{align}
is the \emph{route choice model}. $\zeta(n)$, the \emph{inflow rate}, is an i.i.d. random variable with mean $\mu$. $\xi_i(n)$, the \emph{completion rate on link $i$}, is an i.i.d. random variable with mean $\lambda. $
\end{definition}

We assume $\mu < \lambda R$ to ensure stability (the inflow rate is smaller than the net outflow rate).

\begin{proposition}
When $a = 0$, and $\beta \nearrow \infty$, $X_i(n) \rightarrow \bar{X}$ where $\bar{X}$ is the (unique) Wardrop equilibrium. 
\end{proposition}

\begin{proposition}
When $a << \mu$, $x_i(n) \rightarrow x^{*}$, where $x^{*}$ is an optimal flow for the social cost function $S(x) = x_i C_i(x_i)$ for $\beta \rightarrow \infty$.
\end{proposition}

\begin{lemma}
$\bar{X}(p)$ is monotone in $p$. 
\end{lemma}

\begin{assumption}\label{assm: CostAssumption}
We assume that for any \(i \in [\numLinks]\),  \(\costPrice_i(x_i,p_i) \defas \costLink_i(x_i)+p_i\). Moreover, for every \(i\in [\numLinks]\)  \(\frac{\partial \costLink_i(x)}{\partial x} > 0. \)
\end{assumption}
For any \(p\in \R^{\numLinks}\), let's define the following continuous time ode 
\begin{align}
\label{eq: continuousDyn}
    \dot{x}_i(t) = \frac{\meanOutflow}{\meanInflow} \frac{\exp\lr{-\beta \costPrice_i(x_i(t),p_i)}}{\sum_{j\in[\numLinks]}\exp\lr{-\beta \costPrice_j(x_j(t),p_j)}} - x_i(t), \quad \forall i \in [\numLinks] 
\end{align}

Define \(h_i(x;p) \defas  \frac{\meanOutflow}{\meanInflow} \frac{\exp\lr{-\beta \costPrice_i(x_i,p_i)}}{\sum_{j\in[\numLinks]}\exp\lr{-\beta \costPrice_j(x_j,p_j)}}\) for \(i\in [\numLinks]\). We claim that \(\frac{\partial h_i(x;p)}{\partial x_j} > 0\) for all \(i\neq j\). Indeed 

where the inequality follows from Assumption \ref{assm: CostAssumption}.
It now follows from \cite[Theorem 5.1]{hirsch1985systems} that for any \(p\in \R^{\numLinks}\) the trajectories of \ref{eq: continuousDyn} converges to the set \(\EXSet(p) \defas \{x\in \R^{\numLinks}: h(x;p) = x\}\). We claim that for every \(p\in\R^{\numLinks}\), \(E(p)\) is a singleton set. 

We further check that the forward orbit $O_{+}(x)$, which is the image of the curve $t \rightarrow \phi_t(x)$, $t \in I(x)$, and $\phi_t(x)$ is the flow of the differential equation $\dot{x} = h(x;p)$, has a compact closure. To do this we check conditions from  \cite[Theorem 5.1]{hirsch1985systems}. Namely:

\begin{enumerate}
    \item The ode is cooperative and irreducible (i.e. the matrix $[\frac{\partial h_i}{\partial x_j}](x;p)$ is irreducible for every $x$ and $p$).
    \item $h_i(0) \geq 0$ \\
    \item For any $x \in \mathbb{R}^R_{+}$ there exists $y > x$ (entrywise) with $h_i(y;p) < 0$ for all $i$.  
\end{enumerate}

(1) is checked earlier. (2) is trivial because $h_i(0) = \frac{\lambda}{\mu} \frac{\exp(-\beta \tilde{C}(0,p_i)}{\sum_{j \in [\numLinks]} \exp(-\beta \costPrice(0, p_j)} \geq 0$. (3) holds because 




Define \(g(x;p) \defas h(x;p) -x\). Naturally, we can write \eqref{eq: continuousDyn} as \(\dot{x} = g(x;p)\). For any \(x\in \R^{\numLinks}\), we define 
\[
g_{\infty}(x;p) \defas \lim_{s\ra\infty}\frac{g(sx;p)}{s} = \lim_{s\ra\infty} \frac{h(sx;p)}{s} - x = -x 
\]
The equality follows because \(h(\cdot;p)\) is bounded for any \(p\in\R^{\numLinks}\). Therefore, the ode \(\dot{y}(t)  =g_{\infty}(y(t);p)\) has origin as its globally asymptotically (exponentially, to be precise) stable equilibrium. 


\begin{align}
\label{eq: continuousDyn}
     \frac{\meanOutflow}{\meanInflow} \frac{\exp\lr{-\beta \costPrice_i(x_i(p),p_i)}}{\sum_{j\in[\numLinks]}\exp\lr{-\beta \costPrice_j(x_j(p),p_j)}} &= x_i(p), &&\quad \forall i \in [\numLinks] \\
    x_i(p) \frac{\partial C_i(x_i(p),p_i)}{\partial x_i} &= p_i&&\quad \forall i \in [\numLinks]
\end{align}


\section{Outline of lemmas}
\begin{enumerate}
    \item Existence of $p*$ through Brouwer fixed point theorem ($\bar{X}(p) \frac{\partial C}{\partial x}(\bar{X}(p), p)$ takes bounded sets to bounded sets). 
    \item Product of nonnegative monotonic functions is monotonic. 
    \item Show that \(\bar{X}(p,\beta)\) is monotonic in p 
    \item Use Lyapunov argument 
\end{enumerate}

==> FigPlots.tex <==
\begin{figure}
\begin{subfigure}{.4\textwidth}
  \centering
  % include first image
  \includegraphics[scale = 0.4]{Figures/3LinkSetting13FlowWPrice.eps}  
  \caption{Parameter setting \ref{enum: Setting1}}
  \label{fig:3LinkFlowProfileL1}
\end{subfigure}
\begin{subfigure}{.4\textwidth}
  \centering
  % include second image
  \includegraphics[scale = 0.4]{Figures/3LinkSetting13Price.eps}
  \caption{Parameter setting \ref{enum: Setting1}}
  \label{fig:3LinkPriceProfileL1}
\end{subfigure}
\begin{subfigure}{.4\textwidth}
  \centering
  % include first image
  \includegraphics[scale = 0.4]{Figures/3LinkSetting3FlowWPrice.eps}  
  \caption{Parameter Setting \ref{enum: Setting2}}
  \label{fig:3LinkFlowProfileL2}
\end{subfigure}
\begin{subfigure}{.4\textwidth}
  \centering
  % include first image
  \includegraphics[scale = 0.4]{Figures/3LinkSetting3Price.eps}  
  \caption{Parameter setting \ref{enum: Setting2}}
  \label{fig:3LinkPriceProfileL2}
\end{subfigure}
\caption{Comparison between the trajectories of discrete time stochastic process \eqref{eq: CombinedDT} (dotted trajectories) and the continuous time approximation to it \eqref{eq: singularPerturbedODE}(solid trajectories) for the case when $\numLinks = 3$, $\meanInflow= 0.1$, $\meanOutflow = 0.1$ and \(a=0.0015\) (i.e. \ref{enum: Setting1}) in \textsf{(A),(B)} while $\meanInflow= 0.1$, $\meanOutflow = 0.05$ and \(a=0.0015\) (i.e. \ref{enum: Setting2}) \textsf{(C),(D)}. For discrete time trajectories above we have averaged out the trajectories from \(20\) independent rollouts. }
\label{fig:3LinkSetting}
\end{figure}


\begin{figure}
\begin{subfigure}{.4\textwidth}
  \centering
  % include first image
  \includegraphics[scale = 0.4]{Figures/3LinkSetting13FlowWOPrice.eps}  
  \caption{Paramter setting \ref{enum: Setting3}}
  \label{fig:3LinkFlowPriceProfileL1NoToll}
\end{subfigure}
\begin{subfigure}{.4\textwidth}
  \centering
  % include second image
  \includegraphics[scale = 0.4]{Figures/3LinkSetting3FlowWOPrice.eps}
  \caption{Paramter setting \ref{enum: Setting4}}
  \label{fig:3LinkPriceProfileL2NoToll}
\end{subfigure}
\caption{Comparison between flow obtained without toll pricing (solid lines) and socially optimal level (dashed line). The vertical axis represents flow on corresponding link. The horizontal axis represents the time scale which normalized between the continuous trajectory and discrete time trajectory for comparison.  For discrete time trajectories (solid lines) above we have averaged out the trajectories from \(20\) independent rollouts.} 
    \label{fig:3LinkNoPrice}
\end{figure}


\begin{figure}
\begin{subfigure}{.4\textwidth}
  \centering
  % include first image
  \includegraphics[scale = 0.4]{Figures/6LinkSetting14FlowWPrice.eps}  
  \caption{Paramter setting \ref{enum: Setting5}}
  \label{fig:6LinkFlowProfileL1}
\end{subfigure}
\begin{subfigure}{.4\textwidth}
  \centering
  % include second image
  \includegraphics[scale = 0.4]{Figures/6LinkSetting14Price.eps}
  \caption{Paramter setting \ref{enum: Setting5}}
  \label{fig:6LinkPriceProfileL1}
\end{subfigure}
\begin{subfigure}{.4\textwidth}
  \centering
  % include first image
  \includegraphics[scale = 0.4]{Figures/6LinkSetting4FlowWPrice.eps}  
  \caption{Paramter setting \ref{enum: Setting6}}
  \label{fig:6LinkFlowProfileL2}
\end{subfigure}
\begin{subfigure}{.4\textwidth}
  \centering
  % include first image
  \includegraphics[scale = 0.4]{Figures/6LinkSetting4Price.eps}  
  \caption{Parameter setting \ref{enum: Setting6}}
  \label{fig:6LinkPriceProfileL2}
\end{subfigure}
\caption{  Comparison between the trajectories of discrete time stochastic process \eqref{eq: CombinedDiscreteDyn} (dotted trajectories) and the continuous time approximation to it \eqref{eq: singularPerturbedODE}(solid trajectories) for the case when $\numLinks = 6$, $\meanInflow= 0.1$, $\meanOutflow = 0.05$ and \(a=0.0015\) in \textsf{(A),(B)} (i.e. \ref{enum: Setting5})  and $\numLinks = 6$,$\meanInflow= 0.18$, $\meanOutflow = 0.05$ and \(a=0.0015\) \textsf{(C),(D)} (i.e. \ref{enum: Setting6}). For discrete time trajectories above we have averaged out the trajectories from \(20\) independent rollouts. }
\label{fig:6LinkSetting1}
\end{figure}




\begin{figure}
\begin{subfigure}{.4\textwidth}
  \centering
  % include first image
  \includegraphics[scale = 0.4]{Figures/6LinkSetting14FlowWOPrice.eps}  
  \caption{Parameters setting \ref{enum: Setting7}}
  \label{fig:6LinkPriceProfileL1NoToll}
\end{subfigure}
\begin{subfigure}{.4\textwidth}
  \centering
  % include second image
  \includegraphics[scale = 0.4]{Figures/6LinkSetting4FlowWOPrice.eps}
  \caption{Parameters setting \ref{enum: Setting8}}
  \label{fig:6LinkPriceProfileL2NoToll}
\end{subfigure}
\caption{Comparison between flow obtained without toll pricing (solid lines) and socially optimal level (dashed line). The vertical axis represents flow on corresponding link. The horizontal axis represents the time scale which normalized between the continuous trajectory and discrete time trajectory for comparison. For discrete time trajectories (solid lines) above we have averaged out the trajectories from \(20\) independent rollouts. } 
    \label{fig:6LinkNoPrice}
\end{figure}

==> Preliminaries.tex <==
\section{Preliminaries}

\subsection{Static Routing}

Consider a parallel traffic network with a single source and single destination. These are connected with each other through \(\numLinks\) parallel links\footnote{We fix an enumeration of routes to be used as reference throughout the article, $i = \{1, \dots, R\}$}. The total demand that needs to be routed through the network is \(\demand\in \R\). Let \(\flowLink\in\R^{\numLinks}\) be the flow profile on the network such that \(\flowLink_i\) denotes
the flow on link \(i\in[\numLinks]\).

The congestion cost on a link \(i\in[\numLinks]\) with flow \(\flowLink_i\) is denoted by \(\costLink_i(\flowLink_i)\). Above is the situation.


For ease of exposition, we further define \(\costLink(\flowLink)\defas (\costLink_1(\flowLink_1),\dots,\costLink_\numLinks(\flowLink_\numLinks)) \in \R^{\numLinks} \). The aforementioned routing game setup will be concisely represented as \((\numLinks,\demand,\costLink)\) going forward.  

\begin{assumption}
The functions $C_i(\cdot)$ are increasing and convex. 
\end{assumption}
\begin{definition}
A flow \(x\in\R^{\numLinks}\) is called \emph{feasible} if 
\[
\sum_{i\in[\numLinks]} \flowLink_i = \demand.
\]
We denote the set of feasible flows by \(\feasibleFlow\).
\end{definition} 
\begin{definition}[Wardrop equilibrium]
A feasible flow profile \(\flowLink\in\R^\numLinks\) is a \emph{Wardrop equilibrium} of $(\numLinks,\demand,\costLink)$ if for any \(i\in[\numLinks]\) such that \(\flowLink_i>0\) we have 
\[
\costLink_i(\flowLink_i) \leq \costLink_j(\flowLink_j) \quad \forall \ i\neq j 
\].
\end{definition}

\begin{definition}[Stochastic user equilibrium \cite{cominetti2012modern}]
A feasible flow profile \(\flowLink\in\R^{\numLinks}\) is a \emph{stochastic user equilibrium} of \((\numLinks,\demand,\costLink)\) if the flow on route \(i\) satisfies 
\[
\flowLink_i = \demand\Pr[\costLink_i(x_i)+\noise_i \leq \min_{j\in [\numLinks]}\costLink_j(x_j)+\noise_j] \quad \forall \ i,
\]
where \(\{\noise_i\}_{i\in [R]}\) are zero mean random variables. 
\end{definition}

Further, there is an equivalent convex optimization problem that characterizes the stochastic user equilibrium
\begin{theorem}[\cite{cominetti2012modern}]\label{thm: EqOptProb} An equivalent convex optimization based characterization of Wardrop and stochastic user equilibrium:
\begin{enumerate}
    \item A flow profile \(\flowLink\in\R^{\numLinks}\) is a Wardrop equilibrium \emph{if and only if} it solves the following optimization problem:
    \begin{align*}
    \min_{\flowLink\in\feasibleFlow} \sum_{i\in\numLinks} \int_{0}^{\flowLink_i} \costLink_i(z) \dd z
    \end{align*}
    
    \item A flow profile \(\flowLink\in\R^{\numLinks}\), with \(\{\noise_i\}_{i\in[\numLinks]}\) a zero-mean \(\gumbel(\beta)\) distribution\footnote{Write about Gumbel dist} for some \(\beta>0\), is a stochastic user equilibrium \emph{if and only if} it solves the following optimization problem:
\begin{align*}
    \min_{\flowLink\in F} \sum_{i\in[\numLinks]}\int_{0}^{x_i} \costLink_i(z)\dd z + \frac{1}{\beta} \sum_{i\in[\numLinks]} \flowLink_i \ln{\flowLink_i}.
\end{align*}
\end{enumerate}
\end{theorem}

\begin{corollary}
[\cite{cominetti2012modern}]\label{thm: UniqueSUE} By the strict convexity of the optimization problem (2) in \ref{thm: EqOptProb} there exists a unique stochastic user equilibrium for every \((\numLinks,\demand,\costLink)\).
\end{corollary}
\begin{remark}
An immediate conclusion from the optimization problems presented in Theorem \ref{thm: EqOptProb} is that if \(\beta\rightarrow +\infty\) then stochastic user equilibrium and Wardrop equilibrium coincide. 
\end{remark}

\subsection{Socially Optimal Routing}
We now give a summary of behavior that a central planner would like to induce for the routing game. 

\begin{definition}\label{thm: SocialCost}
The function 
\[
\socialCost(\flowLink) \defas \sum_{i=1}^{\numLinks} \flowLink_i \costLink_i(\flowLink_i).
\]
is called the \emph{social cost function} (SCF) and its minimizer over the feasible set \(\feasibleFlow\), \(\minSocial\), is called the \emph{socially optimal flow}. 
\end{definition}

\begin{definition}
Let \(\marginalCost(x)\) denote the \emph{marginal cost function} (MCF) corresponding to $C$ defined as \[
\marginalCost_i(\flowLink_i) \defas \marginalCost_i(\flowLink_i) + \flowLink_i\grad_x \costLink_i(\flowLink_i)
\]

\end{definition} 
% \begin{definition}
% We define the \textbf{social cost function} 
% \begin{align}
    
% \end{align}
% and we call any feasible flow that minimizes the social cost function an \textbf{optimal flow}.
% \end{definition}

% \begin{definition}
% We define the \textbf{marginal cost function}
% \begin{align}
%     \tilde{C}_i(x_i) = C_i(x_i) + x_i C_i'(x_i)
% \end{align}
% \end{definition}

Given these definitions, we have the following proposition from \cite{roughgarden2010algorithmic}.

\begin{proposition}
[\cite{roughgarden2010algorithmic}] A feasible flow $x \in \feasibleFlow$ is a minimizer of the social cost function for $(\numLinks,\demand,\costLink)$ \emph{if and only if} it is a Wardrop equilibrium for $(\numLinks,\demand, \marginalCost)$, where $\marginalCost$ is the marginal cost function corresponding to $\costLink$.
\end{proposition} 

\subsection{Stochastic Approximation}
In this section we shall recall some of the relevant results from stochastic approximation \cite{borkar2009stochastic}. 

Consider a \(d-\) dimensional stochastic process defined as 
\begin{align}\label{eq: StochasticProcess}
X(n+1) = X(n)+ a\ls{h(X(n)) + M(n+1)}, \quad n \geq 0
\end{align}
where \(h:\R^d \ra \R^d\), \(\{a > 0\}\) is the step sizes and \(\{M(n):n\in \N\}\) is uncorrelated and zero mean. Let \(\mc{F}_n \defas \sigma(X(i),M(i),i\leq n)\). 

\begin{assumption}\label{assm: SA Assumption}
We impose the following assumptions on the stochastic process mentioned in \eqref{eq: StochasticProcess}:
\begin{enumerate}[leftmargin = *]
    \item The function \(h\) is Lipschitz continuous and  there exists function \(h_{\infty}:\R^d\ra\R^d\) defined as 
    \[
    h_\infty(x) \defas \lim_{s\ra\infty} \frac{h(sx)}{s}, \quad \forall x\in \R^d 
    \]
    such that origin is an asymptotically stable equilibrium of the ode \(\dot{x}(t) = h_\infty(x(t))\). 
    \item Let \(\{M(n)\}_{n\in\N}\) be \(\mc{F}_n-\)adapted martingale difference sequence. Furthermore, for some \(C_0 < \infty\) and any initial state \(X(0)\) we posit 
    \[
    \avg[\|M(n+1)\|^2|\mc{F}_n] \leq C_0 \lr{1+\|X(n)\|^2}, \quad n \in \N.
    \]
\end{enumerate}
\end{assumption}

Under the above set of assumptions, one can ensure that the mean squared iterate will be bounded. That is, 
\begin{theorem}
Under the Assumption \ref{assm: SA Assumption}, there exists \(a^\star\) such that for all \(0<a<a^\star\) and \(X(0)\in \R^d\) we have \[
\limsup_{n\ra \infty} \avg[\|X(n)\|^2] \leq C_1
\]
\end{theorem}

==> experiments.tex <==
\section{Numerical Experiments}\label{sec: NumExp}
In this section we present an extensive numerical study of the results presented in \S\ref{sec: Results}. 
Specifically, 
\begin{enumerate}[align=left,leftmargin=*]
    \item we compare the evolution of the stochastic process \eqref{eq: CombinedDT} and the continuous time dynamical system \eqref{eq: singularPerturbedODE} under different parameter settings when toll pricing is implemented;
    \item we compare the evolution of stochastic process \eqref{eq: CombinedDT} with the socially optimal flow when \(a=0\) (i.e. no toll pricing). 
\end{enumerate}

In all the experiments, we set $\beta = 100$ which ensures that we are reasonably close to Wardrop equilibrium (ref Proposition \ref{prop: ConnectionToWardrop}). Furthermore, we set the edge cost function to take the following form: 
\begin{align}
    \costEdge_i(x) = i x^2 + i, \quad \quad i \in [\numLinks].
\end{align}
We implement the stochastic process for \(N=2000\) iterations. In order to plot the continuous time dynamical system and stochastic process we identify \(n\) iterations of stochastic process with \(n\meanOutflow\) units of flow of the continuous time dynamical system.  

We conduct the experiments in the following eight settings of parameters: 
\begin{enumerate}[label = (\textsf{S}-\Roman*), widest=viii, align=left, leftmargin=*]
    \item \label{enum: Setting1} $\numLinks = 3$,  $\meanInflow= 0.1$, $\meanOutflow = 0.1$ and \(a=0.0015\);
    \item \label{enum: Setting2}$\numLinks = 3$, $\meanInflow= 0.1$, $\meanOutflow = 0.05$ and \(a=0.0015\);
    \item \label{enum: Setting3} $\numLinks = 3$,  $\meanInflow= 0.1$, $\meanOutflow = 0.1$ and \(a=0\);
    \item \label{enum: Setting4}$\numLinks = 3$, $\meanInflow= 0.1$, $\meanOutflow = 0.05$ and \(a=0\);
    \item \label{enum: Setting5} $\numLinks = 6$,  $\meanInflow= 0.1$, $\meanOutflow = 0.05$ and \(a=0.0015\);
    \item \label{enum: Setting6} $\numLinks = 6$, $\meanInflow= 0.18$, $\meanOutflow = 0.05$ and \(a=0.0015\);
    \item \label{enum: Setting7} $\numLinks = 6$,  $\meanInflow= 0.1$, $\meanOutflow = 0.05$ and \(a=0\);
    \item \label{enum: Setting8} $\numLinks = 6$, $\meanInflow= 0.18$, $\meanOutflow = 0.05$ and \(a=0\).
\end{enumerate}

We now present the main observations from the numerical study.
In Fig. \ref{fig:3LinkSetting}, Fig. \ref{fig:6LinkSetting1} we observe that introducing the tolling dynamics allows the flow to converge to a neighborhood of the socially optimal flow. Note that socially optimal flow and price are the ones obtained by asymptotic limit of the continuous time dynamical systems \eqref{eq: singularPerturbedODE} (represented by solid lines in the plots).

 Note that the difference between setting \ref{enum: Setting1} and \ref{enum: Setting2} is different values of mean outflow \(\meanOutflow\). This naturally changes the ratio of mean inflow to mean outflow. This ratio, \(\meanInflow/\meanOutflow\), is the {equivalent demand} in the asymptotic limit (as stated in Proposition \ref{prop: xEqExist}) and the equilibrium flow is the flow obtained by performing static one shot routing using this equivalent demand. The significance of this equivalent demand is illustrated in 
     Fig. \ref{fig:3LinkFlowProfileL1} and Fig. \ref{fig:3LinkFlowProfileL2}. Observe that increasing this equivalent demand fills up the blue link (in Fig. \ref{fig:3LinkFlowProfileL2}) which was un-utilized in Fig. \ref{fig:3LinkFlowProfileL1}. 
     
    The settings \ref{enum: Setting5} and \ref{enum: Setting6} are also designed to capture the effect of variable equivalent demand on bigger network.  Interestingly, between these settings we have kept the mean outflow constant but changed mean inflow. This will naturally also change the equivalent demand, whose effect is seen in Fig. \ref{fig:6LinkFlowProfileL1} and Fig. \ref{fig:6LinkFlowProfileL2}. As we increase the equivalent demand the black and magenta link in Fig. \ref{fig:6LinkFlowProfileL2} starts filling up. These were un-utilized in Fig. \ref{fig:6LinkFlowProfileL1}. The effect of increasing the number of links is that some of the links may remain unfilled for quite a long time before starting to fill up (compare Fig.\ref{fig:3LinkFlowProfileL1}-Fig.\ref{fig:3LinkFlowProfileL2} 
     with 
     Fig.\ref{fig:6LinkFlowProfileL1}-Fig.\ref{fig:6LinkFlowProfileL2}
     ). 
     
     Next, we compare the changes in flow evolution when tolling is inactive (i.e. \(a=0\)). For the case of three link network, in Fig. \ref{fig:3LinkFlowPriceProfileL1NoToll} and Fig.\ref{fig:3LinkPriceProfileL2NoToll} we represent the socially optimal flow by dashed lines while flow obtained by stochastic rule \eqref{eq: CombinedDT} by solid lines. The flow allocation is inefficient in such settings. Low cost links are disproportionately over-utilized. Furthermore increasing the equivalent demand exacerbates the situation (compare Fig.\ref{fig:3LinkFlowPriceProfileL1NoToll} and Fig.\ref{fig:3LinkPriceProfileL2NoToll}). Similarly, when the number of links are increased a lot many links remain un-utilized when tolling is absent (refer Fig.\ref{fig:6LinkPriceProfileL1NoToll}-Fig.\ref{fig:6LinkPriceProfileL2NoToll}).


It is also interesting to mention the transient behavior observed when tolling is active (i.e. \(a>0\)). Since the pricing dynamics is slowly updated, during the initial phase of trajectory the flow evolution takes place as if there is no tolling and tries to reach near Wardrop equilibrium. But this phase does not last very long and the pricing dynamics diverts flow from the overutilized links to underutilized links. This effect is very distincly visible, for instance, in Fig.\ref{fig:6LinkFlowProfileL2}. The green link tries to reach its Wardrop point (similar to Fig. \ref{fig:6LinkPriceProfileL2NoToll}) but the pricing dynamics suppress this grown and diverts the flow to magenta and black link.

Note that it takes longer for the price trajectories (refer Fig. \ref{fig:3LinkPriceProfileL1},Fig.\ref{fig:3LinkPriceProfileL2}, Fig.\ref{fig:6LinkPriceProfileL1}, Fig.\ref{fig:6LinkPriceProfileL2}) to converge to their equilibrium as  compared to the flow trajectories. This is attributed to their evolution on slower time scale (recall \(a<<\mu\)).
\input{FigPlots}


==> intro.tex <==
\section{Introduction}\label{sec: Intro}

% \begin{itemize}
%     \item 
%     \item 
%     \item We are proposing a new tolling mechanism that have two time scales -- one is ..., the other is ... why one is slower than the other
% \end{itemize}


% \tdBox{Main point to include in the intro
% 1. Brief account of real world cases where the congestion pricingi is implemented. Practical issues with this

% 2. Bringing out computationaly efficiency of scheme 


% }
%%%% Motivation of the problem

Efficient traffic routing is an increasingly important problem as congestion aggravates on urban transportation networks. Many cities around the world have implemented congestion pricing (tolling) to regulate the demand of travelers (\cite{latimes2021,nyt2021}). Tolling, when properly set in response to real-time traffic conditions, can effectively alleviate congestion and even induce socially optimal loads \cite{sharon2017real, paccagnan2019incentivizing}. 

One challenge of setting tolls is that travelers continuously arrive at and depart from the network, which creates a dynamic involvement of traffic loads in the network. Additionally, travelers are selfish in that they prefer to choose the routes with the minimum cost - travel time cost and the tolls combined. A dynamic tolling mechanism that induces efficient traffic load must account for the dynamic nature of traffic demand and the selfish nature of individuals' routing decisions. In particular, the mechanism must enable the tolls to \textit{adaptively} change in response to changing traffic conditions. 


%In real world traffic networks, users arrive dynamically and make routing decisions based on the existing congestion of the network, and the natural equilibria in routing games (Wardrop, stochastic user (\cite{cominetti2012modern}), etc.) are inefficient in the sense that they are not minimizers of the social cost function \cite{roughgarden2002bad}. how should we set tolls dynamically such that the joint evolution of the load and price converges to social optimality? 

% Para 1 on modeling 
We propose a discrete-time stochastic dynamics to capture the joint evolution of the loads and tolls in a parallel-route network. In each time step of the dynamics, non-atomic travelers arrive at the origin of the network, and they make routing decisions according to a perturbed best response based on the travel time cost and toll of each route in that step. Additionally, a fraction of load on each route is discharged from the network. Both the incoming and outgoing demand are randomly realized from an identical and independent distribution. Therefore, the sequence of link loads forms a Markov process, and the discrete-time stochastic dynamics of loads is governed by the total arriving demand, the stochastic user equilibrium, and the load discharge rate. Furthermore, in each time step, a traffic authority adjusts the toll on each route by interpolating between the current toll and a new increment dependent on the marginal cost of travel time given the load in that step. 

We assume that the dynamics of the toll evolves at a slower time-scale compared to that of the load dynamics. This assumption avoids the situation that tolls change during the trip of individual travelers, which is undesirable in practice (\cite{farokhi2015piecewise}). Therefore, travelers view the tolls as static when they make routing decisions at the arrival. %Therefore, price does not change during their trip. That is, when travelers make routing decisions at , extending the extensive literature on tolling in static routing (\cite{brown2016robustness}, \cite{yang1998principle}, \cite{yang2004trial}). 

%This model builds upon existing work in dynamic traffic routing in two main ways: 1) We incorporate a ``two-timescale'' toll update, in which tolls evolve slowly as compared to the loads, and 2) our model allows for stochasticity in the incoming demand and outgoing loads.
%, and therefore, we are able to analyze the dynamics as a random process. 

% Para 1 of Results: Convergence results

 


We show that the loads and tolls in the discrete-time stochastic dynamics asymptotically concentrate in a neighborhood of a unique fixed point with high probability. The fixed point load is \emph{socially optimal} in that it minimizes the total travel time costs on all routes in the network when the total arriving and discharging traffic demand reach a \emph{steady state}, and the fixed point toll on each route equals to the marginal cost. That is, our dynamic tolling eventually induces the socially optimal loads that account for the incoming and discharging travelers and their selfish routing behavior. Furthermore, we emphasize that our dynamic tolling is \emph{distributed} in that the traffic authority only uses the information of the cost and load on each route to update its toll.  % (\cite{roughgarden2010algorithmic, farokhi2015piecewise}). The socially optimal load corresponds to the {\color{red}``steady-state''} equilibrium of our dynamics when the tolls are set at the socially optimal values. 

% Para 2 of Results: Link between the discrete time and continuous time 

Our technical approach to proving the main result involves: \emph{(i)} Constructing a continuous-time deterministic dynamical system associated with the two timescale discrete-time stochastic dynamics; \emph{(ii)} Demonstrating that the flow of the continuous-time dynamical system has a unique fixed point that corresponds to the socially optimal load and tolls; \emph{(iii)} Proving that the unique fixed point of the flow of the continuous time dynamics is globally stable. In particular, we apply the theory of two time-scale stochastic approximation to show that the loads and tolls under the stochastic dynamics concentrates with high probability in the neighborhood of the fixed point of the flow of continuous time dynamics constructed in \emph{(i)} (\cite{borkar2009stochastic}). Additionally, our proof in \emph{(ii)} on the uniqueness and optimality of fixed point of the flow of continuous time dynamics builds on a variational inequality, and extends the analysis of stochastic user equilibrium in static routing games to account for the steady state of the network given the arriving and discharging traffic (\cite{cominetti2012modern}). Furthermore, we show that the continuous time dynamical system is cooperative, and thus its flow must converge to its fixed point (\cite{hirsch1985systems}). 


%In order to prove the main result we consider an underlying continuous-time deterministic dynamical system that ``closely'' approximates the discrete-time stochastic dynamical system. Such a continuous-time dynamical system is obtained by leveraging the slower update of toll-price dynamics. This property is popularly referred as the ``two-timescale'' property \cite{borkar2009stochastic}.  We show that the continuous-time dynamical system admits unique fixed points that are the same as the socially optimal loads and tolls respectively.  Furthermore, we show that the trajectories of the continuous-time dynamical system in fact converge to the fixed points, which in turn ensures that the discrete-time dynamics concentrates in a neighborhood of socially optimal load with high probability.

% Para 3 of Results: Discuss the techniques
%We design the discrete-time dynamics such that the fixed point of the underlying continuous-time load dynamics, at any \emph{fixed} toll-price, is a game theoretically motivated quantity -- namely it is the ``steady-state'' stochastic user equilibrium at that toll under an \emph{equivalent demand} dependent on the inload and outload. One of our main technical results we establish that such fixed points are monotonic in toll-prices. Broadly speaking, this property ensures that increasing toll-prices on particular link reduces the load on that link.  The convergence of the underlying continuous-time dynamics is established by exploiting this monotonicity in conjunction with the results from \emph{cooperative dynamical systems theory} \cite{hirsch1985systems}. 

Our model and results contribute to the rich literature on designing tolling mechanisms for inducing socially optimal route loads. Classical literature on static routing games has focused on measuring the inefficiency of selfish routing by bounding the "price of anarchy", and designing marginal cost tolling to induce socially optimal route loads (\cite{christodoulou2005price, roughgarden2002bad, roughgarden2010algorithmic}). In static routing games, optimal tolling does not account for the dynamic arrival and departure of travelers. The computation of optimal tolls relies on knowledge of the entire network structure and the equilibrium route flows, which are challenging to compute. 

Dynamic toll pricing has been studied in a variety of settings to account for the continuous arrival and discharge of travelers in the network. The paper \cite{borkar2009cooperative} analyzed a discrete-time stochastic dynamics of the arrival and discharge of non-atomic travelers, and discussed the impact of tolling on routing strategies. We consider an adaptive adjustment of tolls using marginal toll pricing, and analyze the long-run outcomes of the joint evolution of the route loads and tolls. We prove that the tolls updated in our dynamics converge, and eventually induce a socially optimal traffic load associated with the steady state of the network. Additionally, we have removed the assumption in \cite{borkar2009cooperative} that the equilibrium routing strategy is monotonic in tolls. In fact, we \emph{prove} that the monotonicity condition is a feature of the equilibrium routing strategy. 

Moreover, \cite{como2021distributed} proposed a continuous-time dynamical system to study socially optimal tolling when strategic travelers continuously arrive and make selfish routing decisions. In their model, the arrival and discharged loads are balanced so that the aggregate load in the network is a constant. In our setting, both the total arrival load and discharged load are random variables. Therefore, our fixed point analysis needs to account for the total load at the steady state of the network. Moreover, \cite{como2021distributed} assumes that the tolls are adjusted at a faster time scale than their traveler's route preferences, while we assume that the update of tolls is at a slower timescale compared to the change of routing decisions.  

Finally, this article is also related to the literature on learning in routing games, and learning for tolling with unknown network condition. In particular, a variety of algorithms have been proposed to study how travelers learn an equilibrium by repeatedly adjusting their routing decisions based on the observed travel time in the network (e.g. \cite{cominetti2010payoff, krichene2014convergence, kleinberg2009multiplicative}). Additionally, papers \cite{farokhi2015piecewise, poveda2017class, meigs2017learning, wu2020bayesian} have analyzed how the traffic authority adaptively updates the tolls while learning the unknown network condition using crowd-sourced data on traffic load and time costs.




%We note that much of the literature on dynamics in traffic routing focuses on learning dynamics such as those found in \cite{krichene2014convergence}, or casts the problem of dynamic traffic routing as a repeated game \cite{la2002optimal}. This literature does not take into account the \textit{residual loads} and \textit{delays} that are present in real-world traffic networks.

%The works closest to ours in philosophy are \cite{borkar2009cooperative}, \cite{pietrabissa2018discrete}, and \cite{como2021distributed}. These build in a dynamic load adjustment at the network level scheme based on conservation laws whose steady states are Wardrop equilibria, and thus the strategic decisions made by loads are accounted for. However, \cite{borkar2009cooperative} and \cite{pietrabissa2018discrete} do not address the issue of dynamic pricing to social optima, and \cite{como2021distributed} addresses the question of fast-changing pricing (and correspondingly slow-changing preferences) for a large class of dynamic feedback control policies. In contrast we study \textit{slow-changing marginal cost tolls} which are more preferable to users \cite{farokhi2015piecewise}.

This article is organized as follows: we introduce the dynamic tolling model and the discrete time stochastic dynamics in Sec. \ref{sec: Model}. We present the main result in Sec. \ref{sec: Results}, and numerical examples in Sec. \ref{sec: NumExp}. We conclude our work in Sec. \ref{sec: Conclusion}. We only present the key ideas of our prove techniques in the Sec. \ref{sec: Results}, and include all proofs in Appendix \ref{appsec: ProofLemma}. 
%We also note that our scheme allows for computationally tractable marginal cost tolls, as the central authority can \textit{adaptively} compute the tolls based on only the available state information. This is in contrast with the literature on static traffic assignment and tolling, in which the authority would need to compute the traffic equilibrium (known to be computationally intractable problem \cite{papadimitriou2007complexity}) in order to impose tolls. 

%Dynamic traffic routing and tolling presents a novel problem as technologies like navigation apps have enabled flexible routing both spatially and temporally \cite{aswani2011game}. As road congestion worsens as a result of selfish game-theoretic behavior from traffic, it is important to study the effect of interventions like tolling on network state. 



\begin{comment}
{\color{red} Beyond this point it is yet to be updated}
In this article, we use techniques from \emph{cooperative} dynamical systems theory \cite{hirsch1985systems} and two-timescale stochastic approximation \cite{borkar2009stochastic} to prove the convergence of these stochastic dynamics to socially optimal tolls and loads. We show that the discrete-time dynamics asymptotically track a continuous time o.d.e., and that the o.d.e. converges to the socially optimal loads and tolls given a particular construction of the tolls that uses the \textit{marginal cost} incurred on each link. 
We prove a novel monotonicity result 

% \todo[inline]{Model description, comments, and discussion/techniques: Add our contributions here. Second paragraph should focus on model, begin paragraph with ``We propose a discrete time stochastic dynamics that addresses the joint evolution of load and tolls. The introduction should tell about the model. People arrive at origin and make decisions; tolls are set by central authority. Comment on dynamics of $x$ and $p$. End with question: how should we set tolls in this dynamics such that the dynamic converges to social optimality. We also need to justify two time-scale in the next paragraph.

% Also a paragraph to emphasize the novelty of the model.}
% \tdBox{Results around 3 paragraph: Dynamics converge to the socially optimal load. Find continuous dynamics approximating this dynamics. Find continuous dynamics is equilibirium}
% \tdBox{Comment about the techniques: Hirsch and monotonicity. DONT give sense that it is direct deployment. Point out game theoretic aspect. }
Correspondingly, time dynamical routing and its convergence to game theoretic equilibria has been studied in \cite{borkar2009cooperative}. This routing framework allows one to keep track of loads dynamically as they travel through a network, in contrast to the static or repeated routing schemes traditionally found in the literature.  

The challenge is that there is a need for a new mechanism to set tolls adaptively in response to the dynamically evolving traffic conditions, which are determined by the coming and going of traffic in the network and also by the \textit{selfish} routing decisions made by the travelers.
%This paper extends previous work by including a pricing dynamic that ensures link loads minimizes a utilitarian measure of social optimality. 
Taking inspiration from marginal cost pricing \cite{roughgarden2010algorithmic}, we construct an adaptive pricing scheme that ensures that the emergent traffic behavior minimizes a utilitarian measure of social optimality in long run. To this end, we construct a \emph{two-timescale} discrete-time routing algorithm that makes use of this converged price to tax the links and therefore drive them toward the socially optimal loads. This turns the selfish equilibria achieved through dynamic routing into socially optimal ones. 

We also note that our scheme allows for computationally tractable marginal cost tolls, as the central authority can \textit{adaptively} compute the tolls based on only the available state information. This is in contrast with the literature on static traffic assignment and tolling, in which the authority would need to compute the traffic equilibrium (known to be computationally intractable problem \cite{papadimitriou2007complexity}) in order to impose tolls. 


\todo[inline]{We may not be able to cite this as we are only studying parallel links.}

\subsection*{Relevant Work}
\todo[inline]{We don't need a specific section on relevant work.}
It has been known that the natural equilibria in routing games (Wardrop, stochastic user (\cite{cominetti2012modern}), etc.) are inefficient in the sense that they are not minimizers of the social cost function \cite{roughgarden2002bad}. Going back to \cite{pigou1924economics}, there have been attempts at developing tolling schemes to alleviate this problem. In particular, \cite{beckmann1956studies} mathematically demonstrated the efficacy of tolls at rates that would measure the cost to others caused by the average road user, which led to the notion of ``marginal cost tolling". Since then, there has been an extensive literature on tolling in static routing (\cite{brown2016robustness}, \cite{yang1998principle}, \cite{yang2004trial}). 
Dynamic pricing has also been studied in the repeated games setting, as in \cite{farokhi2015piecewise}. 

Dynamic pricing for ramp metering applications, especially the stabilization of traffic loads, have been studied in \cite{papageorgiou1991alinea}, \cite{yin2009dynamic}. These schemes use techniques from feedback control to control traffic load. We provide two critiques for such schemes: they are computationally intractable for the same reason as static tolling, in that they require the computation of a reference load in equilibrium that one would like the trajectory to track. Further, they do not achieve optimality of the social cost function in general without the Wardrop equilibrium to track. 

There are also corresponding optimization based schemes, such as \cite{toledo2015simulation}, {\color{red}[INCOMPLETE]}

\todo[inline]{Combine with game theoretic relevance of results.}
Further, there has been a line of work on converting the static equilibrium concepts found in \cite{wardrop1952road} into a dynamic system. Much of the literature focuses on learning dynamics such as the  found in \cite{krichene2014convergence}, or casts the problem of dynamic traffic routing as a repeated game \cite{la2002optimal}. This literature does not take into account the residual loads and delays that are present in real-world traffic networks. Therefore, the timescale of such algorithms is in days.

\todo[inline]{Maybe not needed.}
We should also mention that there are various natural ways of extending the static routing framework into a dynamic one based on conservation laws at the link level. The cell-transmission model  discretizes links into cells and models traffic as a fluid \cite{daganzo1994cell}, and there is a line of work going back to \cite{lighthill1955kinematic} that studies traffic through partial differential equations (PDEs) and load conservation. We note that these models do not preserve the game theoretic relevance that we desire to model the \textit{strategic} interactions in traffic on networks. 

\todo[inline]{Move before.}
The works closest to ours in philosophy are \cite{borkar2009cooperative}, \cite{pietrabissa2018discrete}, and \cite{como2021distributed}. These build in a dynamic load adjustment at the network level scheme based on conservation laws whose steady states are Wardrop equilibria. Therefore, the strategic decisions made by loads are accounted for. However, \cite{borkar2009cooperative} and \cite{pietrabissa2018discrete} do not address the issue of dynamic pricing to social optima, and \cite{como2021distributed} addresses the question of fast-changing pricing (and correspondingly slow-changing preferences) for a large class of dynamic feedback control policies, in contrast to our study specifically of \textit{slow-changing marginal cost tolls}. There is evidence in the economics literature that users prefer slow-changing taxes \cite{farokhi2015piecewise}.


\end{comment}

\begin{comment}
\begin{center}
    \begin{tabular}{|c|l|}
    \hline 
    Notation & Description \\
    \hline 
      \(\flowDiscrete_i(n)\)  & load on link \(i\) at time \(n\)\\
         \(\priceDiscrete_i(n)\) & price on the link \(i\) at time \(n\)\\ \(\costEdge_i(\cdot)\) & congestion cost as a function of load on that edge \\ 
         \(\costPrice_i(\cdot,\cdot)\) & congestion cost as a function of load and the price assigned \\ 
         \(\sueParameter\) & the parameter which parametrizes the assignment ratios \\ 
         \(\meanInflow\) & mean inflow rate \\
         \(\meanOutflow\) & mean outflow rate \\ 
         \(\inflow_i(n)\) & random variable that decides inflow on link \(i\) at time \(n\) \\ 
         \(\outflow_i(n)\) & random variable that decides the outflow ratio on link \(i\) at time \(n\) \\ 
         \(\flowContinuous_i(t)\) & flow on link \(i\) at time \(t\) in the ode \\
         \(\priceContinuous_i(t)\) & price on link \(i\) at time \(t\) in the ode \\
         \(\numLinks\) & number of links in the network\\
         \(\stepPrice\)& step size used to update the pricing dynamics\\
         \hline 
     \end{tabular}
\end{center}
\end{comment}


\subsection*{Notations}
We denote the set of non-negative real numbers by \(\Rp\). For any natural number \(R\), we succinctly write \([R] = \{1,2,\dots,R\}\). For any vector \(x\in \R^n\), we define \(\diag(x)\in\R^{n\times n}\) to be a diagonal matrix with its diagonals filled with entries of \(x\). 








==> model.tex <==
\section{Model}\label{sec: Model}
  Consider a parallel link network with \(\numLinks\) links connecting a single source-destination pair. The network is occupied by the \emph{non-atomic} population of travellers that continuously arrive at the source node at each time $n =0, 1, 2, \dots$, and are routed through links \(\numLinks\) to the destination node. 
  
  At each time $n$, the flow (i.e. amount of travellers) on link \(i\in [\numLinks]\) is \(\flowDiscrete_i(n)\). The average latency experienced by the travellers on any link \(i \in [\numLinks]\) is a function of flow on the link \(\latency_i: \Rp \ra\Rp\). We assume the latency function is \emph{strictly-increasing} and \emph{convex}, which reflect the congestive nature of links and the fact that the latency increases faster when the flow is higher. 
  
  
  A traffic authority sets toll prices on links, denoted as $\priceDiscrete(n)=\left(\priceDiscrete_i(n)\right)_{i \in \R}$, where $\priceDiscrete_i(n)$ is the toll price on link $i$ at time $n$. The \emph{cost} of an individual traveller who uses any link \(i\in[\numLinks]\) at time $n$, denoted $\costPrice_i(\flowDiscrete_i(n), \priceDiscrete_i(n))$, equals to the experienced travel time cost, which is sum of the average latency function \(\latency_i(\flowDiscrete_i(n))\), a noise term $\upsilon_i(n)$ with zero mean, and the charged toll price: 
  \begin{align*}
      \costPrice_i(\flowDiscrete_i(n), \priceDiscrete_i(n)) \defas \latency_i(\flowDiscrete_i(n)) + \priceDiscrete_i(n)+\textcolor{red}{ \upsilon_i(n)}.
  \end{align*} 
  A schematic summarizing the aforementioned setup is presented in Fig. \ref{fig: SchematicFigure}.
  
  %Further, each link gets tolled by a price of $\priceDiscrete_i(n)$ at every time $n$ with the goal of achieving socially optimal routing of the travellers. To be precise, we demand that the flows on the links asymptotically correspond to the minimizer of the utilitarian \emph{social cost function}$S: \R^{\numLinks} \ra  \R$ where $ S(x) \defas \sum_{i\in [R]} x_i \latency_i(x_i)$. 
  
  
 

 
\begin{figure}[h]
\begin{tikzpicture}[main/.style = {draw, circle}] 
\node[main] (1) {$\mc{S}$}; 
\node[main] (2) [right= 8cm of 1] {$\mc{D}$}; 
\draw[->] (1) to [out=70,in=110,looseness=1.2] node[midway,above] {$\costPrice_1(\flowDiscrete_1(n), \priceDiscrete_1(n))$} (2);
\draw[->] (1) to [out=45,in=135,looseness=0.8] node[midway,above] {$\costPrice_2(\flowDiscrete_2(n) ,\priceDiscrete_2(n)$} (2);
\draw[->] (1) to [out=0,in=180,looseness=0.8] node[midway,above] {$\dots$} (2);
\draw[->] (1) to [out=-45,in=225,looseness=0.8] node[midway,below] {$\costPrice_{R-1}(\flowDiscrete_{R-1}(n), \priceDiscrete_{R-1}(n))$} (2);
\draw[->] (1) to [out=-70,in=-110,looseness=1.2] node[midway,below] {$\costPrice_{R}(\flowDiscrete_R(n), \priceDiscrete_R(n))$} (2);
\end{tikzpicture} 
\caption{Schematic of a \(\numLinks-\)link parallel network with source node \(\mc{S}\) and the destination node \(\mc{D}\) with the corresponding cost to travellers at time \(n\).}
\label{fig: SchematicFigure}
\end{figure}


  
  The demand of travellers arriving at the source node at time \(n\) is a random variable $\inflow(n)$. We assume that  \(\{\inflow(n)\}_{n\in\N}\) are independently and identically distributed (i.i.d) with bounded support $[\inflowLower,\inflowUpper]$ and a finite mean $\lambda$ (i.e. \(\avg[\inflow(n)] = \meanInflow\)). Travelers make routing decisions based on the latest cost vector $\costPrice(n-1)$ at time $n-1$. We denote travelers' routing strategy at time $n$ as $\flowIn(n) = \left(\flowIn_i(n)\right)_{i \in \R}$, where $\flowIn_i(n)$ is the demand of travelers who choose link $i$. We assume that $\flowIn(n)$ is a \emph{stochastic user equilibrium} defined as follows:  %Further, the fraction of flow leaving link $i$ at time $n$ is $\outflow_i(n)$, and $\{\outflow_i(n)\}_{n \in N}$ are i.i.d. as well, with a finite mean $\avg[\outflow_i(n)] = \meanOutflow \in (0,1)$. We also assume that $\inflow_i(n)$ and $\outflow_i(n)$ have bounded support. Specifically, for every \(i\in[\numLinks]\) and       \(n\in\N\), \(\inflow(n) \in [\inflowLower,\inflowUpper]\) almost surely and \(\outflow_i(n) \in [\outflowLower,\outflowUpper]\) almost surely. Moreover \(\outflowLower > 0\) and \(\outflowUpper < 1\).
  
  %The demand at the source node is allocated to different links in accordance to the allocations under \emph{stochastic user equilibrium}. Stochastic user equilibrium is a commonly used routing paradigm that captures the behavioral aspect of traveller's decision making in response to stochastic perception of travel cost associated with different links. 
 \begin{definition}[\textbf{Stochastic User Equilibrium} (\cite{})]\label{assm: InflowAssumption}
  At any time \(n\in \N\), a routing strategy $\flowIn(n)$ is a stochastic user equilibrium if 
  \begin{align}\label{eq: InflowEquation}
     \flowIn_i(n) \defas \frac{\exp(-\sueParameter \costPrice_i(\flowDiscrete_i(n-1), \priceDiscrete_i(n-1)))}{\sum_{j\in[R]}\exp(-\sueParameter \costPrice_j(\flowDiscrete_j(n-1), \priceDiscrete_j(n-1)))}\inflow(n), \quad \forall i \in \R,  
 \end{align}
 where $\beta \in [0, \infty)$. 
  \end{definition}
  
  \textcolor{red}{Here, the parameter $\sueParameter$ characterizes the relative weight the traveller assigns between higher and lower costs. As $\sueParameter \downarrow 0$, the inflows  $\flowIn_i(n) = \flowIn_j(n)$ for all $i,j$. However, as $\sueParameter \uparrow \infty$, $\flowIn_i(n) = \max_{j} (\flowIn_j(n))$ and $\flowIn_i(n) = 0$ for all $i \not\in\{ j : \flowIn_i(n) = \max_{j}(\flowIn_i(n))\}$.}
  
  
   \textcolor{red}{The route choice model represents a \emph{myopic, selfish}, and \textit{perturbed} best-response strategy for picking flow splitting, for $\beta$ finite and nonzero. That is, the flows pick the links with low cost (and leave higher cost links empty), but experience a perturbed version of the cost. Therefore, as $\beta \uparrow \infty$, the inflow approximates the route choice corresponding to Wardrop equilibrium \cite{cominetti2012modern}}.
   \todo[inline]{Borrow formal language}
  
Furthermore, for any \(i\in[\numLinks]\) the proportion of existing flow leaving that link at time \(n\) is given by the random variable \(\outflow_i(n) \in [0,1]\). Thus the flow actually leaving out from link \(i\in[\numLinks]\) at time \(n\in\N\) is given by \begin{align}\label{eq:outflow}
    \flowOut_i(n) \defas \flowDiscrete_i(n-1)\outflow_i(n).
\end{align}
  

\subsection{Discrete time stochastic dynamics} 
We characterize the evolution of the flow on each link in the network by the following discrete time stochastic dynamics: 
\begin{align}\label{eq:x_original}
    \flowDiscrete_i(n+1) &= \flowDiscrete_i(n) +  \flowIn_i(n+1) - \flowOut_i(n+1) .
\end{align}
We note that the stochasticity of the flow dynamics arises from the randomness in demand arrival $\flowIn(n)$ and the outflow rate $\flowOut(n)$. By combining \eqref{eq: InflowEquation} -- \eqref{eq:outflow}, We re-write \eqref{eq:x_original} as follows: 
\begin{equation}\label{eq: FlowDynamics}
\begin{aligned}
    \flowDiscrete_i(n+1) &=  \flowDiscrete_i(n) + \frac{\exp(-\sueParameter \costPrice_i(\flowDiscrete_i(n-1), \priceDiscrete_i(n-1)))}{\sum_{j\in[R]}\exp(-\sueParameter \costPrice_j(\flowDiscrete_j(n-1), \priceDiscrete_j(n-1)))}\inflow(n) -  \flowDiscrete_i(n-1)\outflow_i(n)\\
    &=(1-\meanOutflow) \flowDiscrete_i(n) + \textcolor{red}{\frac{\exp(-\sueParameter \costPrice_i(\flowDiscrete_i(n),\priceDiscrete_i(n)))}{\sum_{j\in[R]}\exp(-\sueParameter \costPrice_j(\flowDiscrete_j(n),\priceDiscrete_j(n)))}\meanInflow} + \meanOutflow\martingale_i(n+1),
\end{aligned}
\end{equation}

\begin{align}\label{eq: hVectorFieldDef}
\vectorFieldX_i(x,p) \defas \frac{\meanInflow}{\meanOutflow}\frac{\exp(-\sueParameter \costPrice_i(x,p))}{\sum_{j\in[R]}\exp(-\sueParameter \costPrice_j(x,p))}. 
\end{align}


where $\meanInflow$ and $\meanOutflow$ are the mean of the random variables $\flowIn(n)$ and $\flowOut(n)$, respectively, and
\begin{align}\label{eq: MartingaleDefinition}
\martingale_i(n+1) \defas \frac{1}{\meanOutflow} \lr{ \frac{\exp(-\sueParameter \costPrice_i(\flowDiscrete_i(n),\priceDiscrete_i(n) ))}{\sum_{j\in[R]}\exp(-\sueParameter \costPrice_j(\flowDiscrete_j(n), \priceDiscrete_j(n)))}\lr{\inflow_i(n+1) - \meanInflow } - \flowDiscrete_i(n)\lr{\outflow_i(n+1)- \meanOutflow} }. 
\end{align}


%The advantage of latter version of flow update is that it allows us to think about \(\meanOutflow\) as a step size.

Furthermore, the central authority updates the toll price vector $\priceDiscrete(n)$ in each time $n$ as follows: 
\begin{align}\label{eq: PricingDynamics}
\priceDiscrete_i(n+1) = (1-a)\priceDiscrete_i(n) + a \flowDiscrete_i(n)\grad_x\costPrice_i(\flowDiscrete_i(n), \priceDiscrete_i(n)) \quad \forall i \in [\numLinks], n\in \N, 
\end{align}
\color{red}where \(a>0\) is the step size.
That is, the toll price updates towards a small step in the direction of \emph{marginal cost} from its current value at time \(n\). We note that the toll update on each link $i$ only depends on the flow and cost of $i$ at time $n$ instead of the entire network. That is, the tolls are updated in a \emph{distributed} manner.  

We posit that the toll prices and latency additively realize the total cost on any link. That is,  $\costPrice_i(\flowDiscrete_i(n), \priceDiscrete_i(n)= \latency(\flowDiscrete_i(n)) + \priceDiscrete_i(n)$. This is consistent with the theory from tolling in static routing \cite{roughgarden2010algorithmic}, in which marginal cost prices also enter the cost functions of every link additively. 

For later reference, we present below the combined flow and price update dynamics \begin{equation}\label{eq: CombinedDT}
    \begin{aligned}
     \flowDiscrete_i(n+1) &=  \flowDiscrete_i(n) + \meanOutflow\lr{\frac{\meanInflow}{\meanOutflow}\frac{\exp(-\sueParameter \costPrice_i(\flowDiscrete_i(n),\priceDiscrete_i(n)))}{\sum_{j\in[R]}\exp(-\sueParameter \costPrice_j(\flowDiscrete_j(n),\priceDiscrete_j(n)))} - \flowDiscrete_i(n)} + \meanOutflow\martingale_i(n+1),\\
     \priceDiscrete_i(n+1) &= (1-a)\priceDiscrete_i(n) + a \flowDiscrete_i(n)\grad_x\costEdge_i(\flowDiscrete_i(n)) \quad \forall i \in [\numLinks], n\in \N.
    \end{aligned}
\end{equation}

% This model follows a class of dynamics in the spirit of \cite{borkar2009cooperative} and \cite{pietrabissa2018discrete}. In particular, we note that the dynamic is distinguished from classical dynamics in routing games (gradient descent, multiplicative weights, etc.) in that it explicitly accounts for the inflow and outflow of vehicles through a conservation law.

At last, we assume that in \eqref{eq: CombinedDT} the price dynamics update on a slower time scale than the flow dynamics. That is, \(a << \meanOutflow\). Slow price updation is a desirable feature to have from the traveller's perspective \cite{farokhi2015piecewise} as it gives them appropriate time to respond. 
\color{black}
% \textcolor{red}{
% \begin{itemize}
%     \item \sout{Introduce tolls in the beginning. Add toll prices in the cost function when it is first introduced in route choices rather than later }
%     \item \sout{Rephrase "assumptions" as setups, and put them in line}
%     \item \sout{You need to introduce two timescale here, and justify it}
%     \item Put technical parts in the technical section 
%     \item Avoid loose English and casual use of terminologies that you don't define 
%     \item \sout{Name the dynamics as X-update, p-update (or something else that makes sense to you). It is easier for readers to remember them since they are referred repeatedly throughout}
% \end{itemize}}

==> result_revised.tex <==
\section{Main Results}
In Sec. \ref{subsec:fixed_point}, we present a continuous-time deterministic dynamics that is associated with the discrete-time stochastic dynamics \eqref{eq: CombinedDT}. We show that the continuous time dynamics has a unique fixed point. The fixed point flow vector is a \textcolor{red}{generalized stochastic user equilibrium} associated with the fixed point toll price, and it minimizes the social cost as $\beta \to \infty$. In Sec. \ref{ssec: Convergence}, we apply the two timescale stochastic approximation theory to show that the states of our discrete time dynamics $\left(\flowDiscrete(n), P(n)\right)$ \textcolor{red}{concentrate near} the unique fixed point. Therefore, the toll price in our dynamics eventually induces a \textcolor{red}{perturbed socially optimal flow vector}. %we prove the main result of the paper -- under the setup presented in \S\ref{sec: Model} the combined flow-toll price update \eqref{eq: CombinedDT} asymptotically concentrate in a neighborhood around the socially optimal flows and prices with high probability. One of the major contributions here is to show that the trajectories of the ``natural'' continuous time dynamical system, associated with the stochastic process  \eqref{eq: CombinedDT}, converges to the socially optimal flow and toll prices. We, then, employ the machinery from two-timescale constant step size stochastic approximation to bridge the connection between the continuous time dynamical system and discrete time stochastic process. 

\subsection{Continuous time dynamics and fixed point}\label{subsec:fixed_point}
We first introduce a \textcolor{red}{deterministic} continuous time dynamical system that \textcolor{red}{corresponds to} the discrete time stochastic process \eqref{eq: CombinedDT}. We define define $x(t)$ as the flow vector and $p(t)$ as the toll price vector at time $t \in [0, \infty)$ \textcolor{red}{(I suggest to use "time step" for discrete step $n$ and "time" for continuous time $t$)}. We also define \(\stepRatio \defas \frac{\stepPrice}{\meanOutflow} \), where $\meanOutflow$ (resp. $\stepPrice$) is the stepsize of the discrete dynamics of flow (resp. toll price). Since the toll price update is at a slower timescale compared to the flow update (i.e. $\stepPrice \ll \meanOutflow$), we have $\stepRatio \ll 1$. % between flow and toll prices. Furthermore, for any \(x,p\in \R^{\numLinks}\) define 

\tdBox{Define $x$ and $p$}

The continuous time dynamics of $(x(t), p(t))$ is given as follows: 
%Consider the following continuous time dynamical system, that we expect should closely follow \eqref{eq: CombinedDT}, 
\begin{equation}\label{eq: singularPerturbedODE}
    \begin{aligned}
    \dot{\flowContinuous}_i(t) &= \frac{1}{\stepRatio}\lr{\vectorFieldX_i(\flowContinuous(t),\priceContinuous(t)) - \flowContinuous_i(t)}, \\ 
    \dot{\priceContinuous}_i(t) &= -\priceContinuous_i(t) + \flowContinuous_i(t)
    \grad_x \costPrice_i(\flowContinuous_i(t), p_i(t)), \quad \forall \ t \geq 0.
    \end{aligned}
\end{equation}


\textcolor{red}{For the sake of completeness, I think you should briefly say what is "fixed point".}

We next present the fixed point of \eqref{eq: singularPerturbedODE} and their properties. To begin with, we introduce the following two definitions: 
\begin{definition}[Steady-State Stochastic User Equilibrium]\label{def:generalized_SUE}
 A flow vector $\fixedPointFlow(\priceContinuous)$ is a generalized stochastic user equilibrium corresponding to a \textcolor{red}{dispersion parameter} and a toll price vector $\priceContinuous$ if
 \begin{align}\label{eq: xEquilibrium}
    \fixedPointFlow_i(\priceContinuous) = \vectorFieldX_i(\fixedPointFlow(\priceContinuous),\priceContinuous) = \frac{\meanInflow}{\meanOutflow}\frac{\exp(-\sueParameter \costPrice_i(\fixedPointFlow_i(\priceContinuous),\priceContinuous_i))}{\sum_{j\in[R]}\exp(-\sueParameter \costPrice_j(\fixedPointFlow_j(\priceContinuous),\priceContinuous_j))}.
\end{align}

\end{definition}

\textcolor{red}{Add interpretation of this definition, build the link to generalized Wardrop equilibrium with $\beta \to \infty$.}

\begin{definition}[Perturbed socially optimal flow]\label{def:perturbed_opt}
A flow vector $\fixedPointFlow$ is a perturbed socially optimal flow if $\fixedPointFlow$ minimizes the following convex optimization problem: 
\begin{equation}\label{eq: SocialCostWE}
\begin{aligned}
    \min_{y\in \R^{\numLinks}} &\quad \sum_{i\in[\numLinks]} y_i\costEdge_i(y_i) + \frac{1}{\beta}\sum_{i\in[\numLinks]} y_i\log(y_i) \\
    \text{s.t} & \quad \sum_{i\in[\numLinks]} y_i = \frac{\meanInflow}{\meanOutflow}.
\end{aligned}
\end{equation}
\end{definition}
\textcolor{red}{Add interpretation of this definition, build the link to social optimality with $\beta \to \infty$.}
 %Owing to  the assumption \(\stepRatio<<1\) we see that \(\flowContinuous(\cdot)\) is a ``fast'' dynamics while \(\priceContinuous(\cdot)\) is a comparatively ``slower'' component. Therefore we can consider \(\priceContinuous(\cdot)\) ``static'' while analyzing the behavior of \(\flowContinuous(\cdot)\). We therefore first consider the following dynamical system for any fixed \(\priceContinuous\in\R^{\numLinks}\):
 
 
 \begin{theorem}\label{theorem: fixed_point}
 The continuous time dynamical system \eqref{eq: singularPerturbedODE} has a unique fixed point $(\fixedPointFlow(\fixedPointPrice), \fixedPointPrice)$ such that $\fixedPointFlow$ is a generalized stochastic user equilibrium corresponding to $\fixedPointPrice$, and 
 \begin{align}\label{eq: pEquilibrium}
    \fixedPointPrice_i = \fixedPointFlow_i(\fixedPointPrice) \grad \costEdge_i(\fixedPointFlow_i(\fixedPointPrice)).
\end{align}
Moreover, $\fixedPointFlow$ is a perturbed socially optimal flow. 
 \end{theorem}
 
 \textcolor{red}{Interpret Theorem \ref{theorem: fixed_point}.}
 
The proof of Theorem \ref{theorem: fixed_point} has three parts: 

\emph{Part 1:} We show that any fixed point of \eqref{eq: singularPerturbedODE} must satisfy that the flow vector is a generalized stochastic user equilibrium corresponding to the price vector, and the price vector satisfies \eqref{eq: pEquilibrium} (Lemma \ref{lemma:twotimescale}). This part relies on the fact that our dynamical system has two timescales. 

\emph{Part 2:} We prove that the fixed point $\left(\fixedPointFlow, \fixedPointPrice\right)$ is unique. In this part, we first show that for any price vector $\priceContinuous$, the generalized stochastic user equilibrium $\fixedPointFlow(\priceContinuous)$ is unique, and can be solved as the optimal solution of a convex optimization problem (Lemma \ref{lemma:gStochasticEquilibrium}). Secondly, we prove that there exists a unique fixed point price vector $\fixedPointPrice$ that satisfies \eqref{eq: pEquilibrium}. We note that in \eqref{eq: pEquilibrium}, the flow vector $\fixedPointFlow(\priceContinuous)$ is a generalized stochastic user equilibrium that depends on $\priceContinuous$. Thus, the key step of proving the uniqueness of $\priceContinuous$ is to show that the generalized stochastic equilibrium $\fixedPointFlow(\priceContinuous)$ is monotonic in $\priceContinuous$ (Lemmas \ref{lemma:monotonicity} and \ref{lemma:unique_price}). 


\emph{Part 3:} We conclude the theorem by proving that, given the fixed point price vector $\fixedPointPrice$, the corresponding fixed point flow vector $\fixedPointFlow$ is perturbed socially optimal (Lemma \ref{lemma:optimality}).  

We now present the lemmas in each part, and provide the proof ideas of these results. We include the formal proofs in the appendix due to the space limit. 

\begin{lemma}\label{lemma:twotimescale}
For any $\epsilon \ll 1$, a state $(\fixedPointFlow, \fixedPointPrice)$ is a fixed point of \eqref{eq: singularPerturbedODE} if and only if $\fixedPointFlow$ is a generalized stochastic user equilibrium corresponding to $\fixedPointPrice$, and $\fixedPointPrice$ satisfies \eqref{eq: pEquilibrium}. 
\end{lemma}

\begin{lemma}\label{lemma:gStochasticEquilibrium}
For every \(\priceContinuous\in \R^{\numLinks}\), \(\fixedPointFlow(\priceContinuous)\) is the unique optimal solution of the following convex optimization problem
% (also known as the stochastic user equilibrium (SUE) problem \cite{cominetti2012modern})
: 
 \begin{equation}\label{eq: OptimizationProblem}
\begin{aligned}
    \min_{y\in \R^{\numLinks}} & \quad  \sum_{i\in [\numLinks]} \int_{0}^{y_i} \costPrice_i(s,p_i)ds + \frac{1}{\beta} \sum_{i\in [\numLinks]} y_i \ln{y_i}, \\
    \text{s.t} & \quad \sum_{i\in[\numLinks]} y_i = \frac{\meanInflow}{\meanOutflow}%\quad k(y)\defas.
\end{aligned}
\end{equation}
\end{lemma}
%We shall refer \(\frac{\meanInflow}{\meanOutflow}\) as the \emph{equivalent demand in asymptotic limit}.


\begin{lemma}[\textbf{Monotonicity of $\fixedPointFlow(\priceContinuous)$}]\label{lemma:monotonicity}
For any \(p,p'\in\R^{\numLinks}\) we have 
\[\lara{ \fixedPointFlow(p)-\fixedPointFlow(p'),p-p' }<0. \]
Consequently, \(\frac{\partial \fixedPointFlow_i(\priceContinuous)}{\partial \priceContinuous_i} < 0\) for all \(i\in[\numLinks]\). 
\end{lemma}

\begin{lemma}[\textbf{Existence and uniqueness of $\fixedPointPrice$}]\label{lemma:unique_price}
The fixed point price vector $\fixedPointPrice$ is unique. 
\end{lemma}

\begin{lemma}
The fixed point flow vector $\fixedPointFlow$ is perturbed socially optimal. 
\end{lemma}

\subsection{Convergence}
In this section,we show that the states $(\flowDiscrete, \priceDiscrete)$ in the discrete stochastic dynamical system converges to a \textcolor{red}{neighborhood} of the unique fixed point $(\fixedPointFlow, \fixedPointPrice)$, \textcolor{red}{and the neighborhood depends on the average update stepsize $a$.} That is, the \textcolor{red}{two timescale dynamic pricing mechanism} eventually induces a perturbed socially optimal flow. 


\begin{theorem}\label{theorem:discrete_convergence}
\begin{align}
    \limsup_{n\ra+\infty}\avg[\|\flowDiscrete_n-\fixedPointFlow\|^2+\|\priceDiscrete_n-\fixedPointPrice\|^2] = \mathcal{O}(\meanOutflow)+\mathcal{O}\lr{\frac{a}{\meanOutflow}}.
\end{align}
\end{theorem}
\textcolor{red}{You need to explain this theorem: convergence in what sense, neighborhood in what sense, how do stepsizes affect things. You also need to loop back to the focus -- updates lead to optimality.}  




To prove Theorem \ref{theorem:discrete_convergence}, we \textcolor{red}{first... (Lemma \ref{}) In this part, we apply the theory of two-timescale stochastic approximation.} Then, we show that the the continuous time dynamical system \eqref{eq: singularPerturbedODE} converges to the unique fixed point $(\fixedPointFlow, \fixedPointPrice)$ (Lemma \ref{lemma: ConvergenceFlowCont}) . Therefore, \textcolor{red}{we can conclude that  ...}



\begin{lemma}\label{lemma: ConvergenceFlowCont}
The fixed point $(\fixedPointFlow, \fixedPointPrice)$ is a globally asymptotically stable state of \eqref{eq: singularPerturbedODE}, i.e. $\lim_{t \to \infty} (\flowContinuous(t), \priceContinuous(t)) = (\fixedPointFlow, \fixedPointPrice)$.
\end{lemma}

\color{red}
We proof this lemma by applying \textcolor{red}{the theory of cooperative dynamics} from \cite{hirsch1985systems}. We provide a brief review here for the sake of completeness. 

%  For this purpose we use results  which is also stated in Theorem \ref{thm: HirshResult} for the sake of completeness.
 
%  In this section we review a result from \cite{hirsch1985systems} which provides an easily verifiable requirement on the vector field which ensures convergence to equilibrium.  

Consider a \(C^1-\)vector field \(f:\R^n\rightarrow \R^n\) and the dynamical system 
\begin{align}\label{eq: DynSys}
\dot{x}(t) = f(x(t))
\end{align}
where
\begin{enumerate}%[label=(P-\roman*)]
    \item \label{enum: Assm1} for any \(i\neq j \in [n]\) and \(x\in \R^n\) we have \(\frac{\partial f_i(x)}{\partial x_j} \geq 0\); 
    \item \label{enum: Assm2} the Jacobian matrix \(\nabla f(x)\) is irreducible;\footnote{Define irreducible here}
    \item \label{enum: Assm3} for every \(i\in[n]\), \(f_i(0)\geq 0\);
    \item \label{enum: Assm4} for any \(x\in\Rp^n\) there exists \(y > x\) with \(f_i(y) < 0\) for all \(i\in[n]\)
 \end{enumerate}
 \begin{theorem}[{\cite[Theorem 5.1]{hirsch1985systems}}]\label{thm: HirshResult}
 Let the dynamical system \eqref{eq: DynSys} satisfy the assumptions \ref{enum: Assm1}-\ref{enum: Assm4}. Then \(\Rp^n\) is positively-invariant and trajectories starting almost everywhere in \(\Rp^n\) converge to the set \(\{x: f(x) = 0\}\).  
 \end{theorem}
 
 Based on Theorem \ref{thm: HirshResult}, we prove Lemma \ref{lemma: ConvergenceFlowCont} by verifying that both the continuous time dynamics \eqref{eq: singularPerturbedODE} satisfies assumptions \ref{enum: Assm1}-\ref{enum: Assm4}. 
 \color{black}





==> results.tex <==
\section{Results}\label{sec: Results}




\begin{align}\label{eq: FixedPointFlowDynamics}
    \dot{\flowContinuousNew}_i(t) = \vectorFieldX_i(\flowContinuousNew(t),p) -\flowContinuousNew_i(t), \quad \quad \forall i \in [\numLinks], \forall \ t\geq 0.
\end{align}



For any \(\priceContinuous\in\R^{\numLinks}\) let the equilibrium of \eqref{eq: FixedPointFlowDynamics} be denoted by \(\fixedPointFlow(\priceContinuous)\). Note that  we will keep the parameter \(\beta\) in the equilibrium flow for exactness. By definition, for every \(i\in[\numLinks]\)


As the price dynamics in \eqref{eq: singularPerturbedODE} is on a slower timescale we expect that the flow trajectory \(\flowContinuousNew\) has converged to its equilibrium value.  That is, the price dynamics in \eqref{eq: singularPerturbedODE} closely track the following continuous time dynamical system 
\begin{align}\label{eq: PriceDynamics}
    \dot{\priceContinuousNew}_i(t) = -\priceContinuousNew_i(t)+\fixedPointFlow_i(\priceContinuousNew(t))\grad_x \costPrice_i(\fixedPointFlow_i(\priceContinuousNew(t)), \priceContinuousNew_i(t)), \quad \forall \ i\in[\numLinks], \forall \ t\geq 0.
\end{align}
We denote the equilibrium of \eqref{eq: PriceDynamics} by  \(\fixedPointPrice\). It follows that for every \(i\in[\numLinks]\)
% \begin{align}\label{eq: pEquilibrium}
%     \fixedPointPrice_i = \fixedPointFlow_i(\fixedPointPrice) \grad \costEdge_i(\fixedPointFlow_i(\fixedPointPrice)).
% \end{align}
At some places in the subsequent exposition, we shall denote \(\fixedPointPrice = \fixedPointPrice^{(\beta)}\) to emphasize the explicit dependence on \(\beta\). 
% A natural question at this stage is to ensure the existence of solutions to \eqref{eq: xEquilibrium} and \eqref{eq: pEquilibrium}. Furthermore our results guarantee uniqueness of the equilibrium points as well. 

% We posit a continuous time o.d.e. in variables $\flowContinuous \in \mathbb{R}^{\numLinks}$ and $\priceContinuous \in \mathbb{R}^{\numLinks}$ that the stochastic dynamics track. 
% Because we had assumed that the price evolves on a slower timescale, we are able to study the fixed points of the price dynamic $\fixedPointPrice$ and the induced fixed point flow $\fixedPointFlow(\fixedPointPrice)$; the fixed point equations for these quantities are introduced below.
We briefly summarize the results that are presented in this section. Moreover, we also state the main proof techniques involved in the itemized list below. Details are deferred to following subsections. 
\begin{enumerate}%[align=left, label=(\textsf{R}-\Roman*), leftmargin=*,widest=iii]
    \item \label{enum: Result1} We show existence, uniqueness $\fixedPointFlow(p)$. This is ensured by drawing connections with the literature on stochastic user equilibrium \cite{cominetti2012modern}. Furthermore, we establish that the trajectories of \eqref{eq: FixedPointFlowDynamics} converge to $\fixedPointFlow(p)$, for any \(p\in\R^{\numLinks}\). This is established by noting that the dynamics \eqref{eq: FixedPointFlowDynamics} is cooperative (\cite{hirsch1985systems}). 
    \item \label{enum: Result3} We show
    existence and uniqueness of $\fixedPointPrice$. Existence is attributed to Brouwer's fixed point theorem. Meanwhile, uniqueness of $\fixedPointPrice$ is ensured by monotonicity of $p\mapsto \fixedPointFlow(p)\in\R^{\numLinks}$. Furthermore, the convergence of the trajectories of \eqref{eq: PriceDynamics} to \(\fixedPointPrice\) is again established by noting that dynamics \eqref{eq: PriceDynamics} is cooperative. 
    \item \label{enum: Result4} We conclude by noting that the discrete time stochastic process \eqref{eq: CombinedDT} concentrates near \(\fixedPointFlow(\fixedPointPrice)\) and \(\fixedPointPrice\). Towards this end, we utilize results on two timescale constant step size stochastic approximation. 
\end{enumerate}


% In addition, we also make the following technical assumption on the second moment of the price and flow processes which are crucial for using results from stochastic approximation literature. 
% \begin{assumption}[\textbf{Stability Criterion}]
% We assume that \(\sup_{n}\avg[\|\priceDiscrete(n)\|^2]<+\infty\) and \(\sup_{n}\avg[\|\flowDiscrete(n)\|^2]< +\infty \) . 
% \end{assumption}
% \begin{remark}
% {\color{red} We can add a remark here saying this one would expect this sort of technical assumption to hold because our dynamics satisfied the conditions posed in \cite{lakshminarayanan2017stability}. We can do all the calculations that show that \cite[A4-A5]{lakshminarayanan2017stability} hold.}. \end{remark}
%\todo[inline]{Will think about relaxing this assumption at later point. It is good to keep in mind the following reference: \url{https://www.sciencedirect.com/science/article/abs/pii/S0005109816305222}.}

% In this section we shall zfirst present results on existence and uniqueness of {the} equilibrium point of the dynamical systems \eqref{eq: singularPerturbedODE}. Following this, we prove the convergence of the trajectories of \eqref{eq: singularPerturbedODE} to the corresponding equilibrium.  


\subsection{
Properties of fixed points}\label{ssec: PropFixedPoint}
We now discuss the existence and uniqueness of the fixed points $\fixedPointFlow(\cdot)$ and $\fixedPointPrice$. 

In this subsection, we shall first show that \(\fixedPointFlow(\cdot)\) in \eqref{eq: xEquilibrium} is a well-defined (single valued) function.  The following proposition formalizes this claim. 
\begin{proposition}[\textbf{Existence and uniqueness of $\fixedPointFlow(\priceContinuous)$}]\label{prop: xEqExist}
For every \(\priceContinuous\in \R^{\numLinks}\), \(\fixedPointFlow(\priceContinuous)\) exists and is unique. Furthermore, one can characterize \(\fixedPointFlow(\priceContinuous)\) as solution to the following convex optimization problem
% (also known as the stochastic user equilibrium (SUE) problem \cite{cominetti2012modern})
: 
 \begin{equation}\label{eq: OptimizationProblem}
\begin{aligned}
    \min_{y\in \R^{\numLinks}} & \quad  \sum_{i\in [\numLinks]} \int_{0}^{y_i} \costPrice_i(s,p_i)ds + \frac{1}{\beta} \sum_{i\in [\numLinks]} y_i \ln{y_i}, \\
    \text{s.t} & \quad \sum_{i\in[\numLinks]} y_i = \frac{\meanInflow}{\meanOutflow}%\quad k(y)\defas.
\end{aligned}
\end{equation}

We shall refer \(\frac{\meanInflow}{\meanOutflow}\) as the \emph{equivalent demand in asymptotic limit}.
\end{proposition}

To prove the above result we analyze the KKT conditions for the convex optimization problem and uniqueness is established by the strict convexity of the optimization objective in \eqref{eq: OptimizationProblem}. 
%The details of the proof are deferred to Appendix \ref{proof: Prop31}. 
\begin{proof}[Proof of Proposition \ref{prop: xEqExist}]
In the subsequent proof we shall show that the following claims hold: 

\begin{enumerate}[label= (C-\Roman*),widest=ii,leftmargin=*,align=left]
    \item \label{thm: claim1} For any \(p\in\R^{\numLinks}\), the optimizer of \eqref{eq: OptimizationProblem} is unique; call it \(y^\star(p)\);
    \item \label{thm: claim2} \(y^\star(p)\) is an optimal solution if and only if it satisfies \(h(y^\star(p),p) = y^\star\)
\end{enumerate}
Note that the above two claims ensure that \(\fixedPointFlow(p) = y^\star(p)\). The subsequent exposition establishes the validity of these claims.

To see that \ref{thm: claim1}  is true, we note that the feasible set of \eqref{eq: OptimizationProblem} is a compact convex set.  Moreover, from the convexity of $\costEdge$ it follows that \(k(y)\) is a strictly convex function. Strict convexity ensures the uniqueness of solution of a convex optimization problem on a convex compact set \cite{boyd2004convex}.


For \ref{thm: claim2}, we now employ KKT conditions of optimality: let \(\delta\in\R \) be the Lagrange multiplier corresponding to the equality constraint. Define the Lagrangian as follows:
\[
L(y,\delta,p) \defas \sum_{r\in [\numLinks]} \int_{0}^{y_r} \costPrice_r(s,p_r)ds + \frac{1}{\beta} \sum_{r\in \numLinks} y_r \ln{y_r} + \delta \lr{\sum_{r\in[\numLinks]} y_r - \frac{\meanInflow}{\meanOutflow}}
\]

The optimal solution $y^{\star}(p)$ and Lagrange multiplier $\delta^\star$ satisfy: \begin{enumerate}[widest=ii,leftmargin=*,align=left]
    \item \(\nabla_{y}L(y^{\star}(p),\delta^{\star},p) = 0\). This gives us \(\costPrice_r(y_r^{\star}(p),p_r) + \frac{1}{\beta}\lr{1+\ln(y_r^{\star}(p))} +\delta^{\star} = 0\), which can be also written as follows
    \begin{align}
    \label{eq: Opt_y}
    y_r^{\star}(p) = \exp(-1-\beta \costPrice_r(y_r^{\star}(p),p_r))\exp(-\beta \delta^\star), \quad \forall \ r\in[\numLinks].
    \end{align}
    \item \(\nabla_\delta L(y^{\star}(p),\delta^{\star},p) = 0\). That is, 
    \(
    \sum_{r\in \numLinks} y_r^{\star}(p)  = \frac{\meanInflow}{\meanOutflow}.
    \)
    \end{enumerate}
    Using \eqref{eq: Opt_y} we have 
    \[
    \exp(-\beta \delta -1 )  = \frac{\meanInflow}{\meanOutflow} \frac{1}{\sum_{r\in[\numLinks]}\exp(-\beta \costPrice_r(y_r^{\star}(p),p_r))}
    \]

The above conditions give us that \(y^\star(p)\) is an optimal solution of \eqref{eq: OptimizationProblem} if and only if it satisfies
\[
y_r^\star(p) = \frac{\meanInflow}{\meanOutflow} \frac{\exp(-\beta \costPrice_r(y_r^\star(p),p_r))}{\sum_{r\in[\numLinks]}\exp(-\beta \costPrice_r(y_r^\star(p),p_r))} = \vectorFieldX_r(y^\star(p),\priceContinuous), \quad \forall \ r\in[\numLinks].
\]
\end{proof}
\tdBox{May be remove this remark}
\begin{remark}
\label{rem: compactnessXEq}
Note that the set \(\{\fixedPointFlow(p):p\in\R^{\numLinks}\}\) is a subset of a simplex in \(\R^{\numLinks}\). This is because for any \(p\in\R^{\numLinks}\), \(\fixedPointFlow(p) \geq 0\) and \(\sum_{i\in[\numLinks]}\fixedPointFlow_i(p) = \frac{\meanInflow}{\meanOutflow}\). 
\end{remark}

We now proceed to show the existence and uniqueness of the solution of the nonlinear fixed point equation \eqref{eq: pEquilibrium}:
\begin{proposition}[\textbf{Existence and uniqueness of $\fixedPointPrice$}]\label{prop: pEqExists}
There exists a unique solution to \eqref{eq: pEquilibrium}. 
\end{proposition}
In the above result, we prove existence by using Brouwer's fixed point theorem. However, to establish uniqueness we first observe that \(\fixedPointFlow(\cdot)\) is monotonic \todo{Expand on this, as the proof will be in the appendix}. Following which we argue that if the solution to \eqref{eq: pEquilibrium} is not unique then the monotonic nature of \(\fixedPointFlow(\cdot)\) no longer holds. The aforementioned monotonic property is more formally stated in the next lemma. 

\begin{lemma}[\textbf{Monotonicity of $\fixedPointFlow(\priceContinuous)$}]\label{lem: MonotonicityFlow}
For any \(p,p'\in\R^{\numLinks}\) we have 
\[\lara{ \fixedPointFlow(p)-\fixedPointFlow(p'),p-p' }<0. \]
Consequently, \(\frac{\partial \fixedPointFlow_i(\priceContinuous)}{\partial \priceContinuous_i} < 0\) for all \(i\in[\numLinks]\).  
\end{lemma}
The proof of Lemma \ref{lem: MonotonicityFlow} follows by arguing about the variational inequalities associated with \eqref{eq: OptimizationProblem}. The details of the proof are deferred to Appendix \ref{proof: lemMonotonic}.
\begin{remark}
Note that the monotonicity of \(\fixedPointFlow(p)\) was considered as an assumption in \cite[cf Eq. (9)]{borkar2009cooperative}. In this article we have exploited the connection of our routing scheme with stochastic user equilibrium \cite{cominetti2012modern} to \emph{prove} the monotonicity property. 
\end{remark}
\begin{proof}[\textbf{Proof of Proposition \ref{prop: pEqExists}}]
We shall first show the existence and then prove the uniqueness of \(\fixedPointPrice\). 

For any \(p\in\R^{\numLinks}, r\in[\numLinks]\), define \(z_r(p) = \fixedPointFlow(p)\grad_x\costEdge_r(\fixedPointFlow_r(p))\). The equilibrium price \(\fixedPointPrice\) is then solution to the fixed point equation \(p=z(p)\).  Define a set \(K = \{y\in\R^{\numLinks}: y\geq 0, \|y\|_1 \leq \frac{\meanInflow}{\meanOutflow}\max_{r\in[\numLinks]}\grad_x c_r\lr{\frac{\meanInflow}{\meanOutflow}}\}\). Due to Remark \ref{rem: compactnessXEq} andthe convexity of the cost, we can see that \(z(\cdot)\) maps the convex compact set \(K\) to itself. Therefore, Brouwer's fixed point theorem \cite{sastry2013nonlinear} guarantees the existence of fixed point \(\fixedPointPrice\).

% Having shown the existence of equilibrium pricing, we shall now show the uniqueness of the solution of \eqref{eq: pEquilibrium}. But before we establish that result, we present a technical lemma that is key to the subsequent proofs. The following lemma formalizes the intuition that increasing prices on any link reduces flow on that link.




Now, we prove the uniqueness of the fixed point $\fixedPointPrice$ satisfying \eqref{eq: pEquilibrium}.  
We shall prove this via a contradiction argument. Assume that there are two distinct price profiles $\fixedPointPrice, \fixedPointPrice' \in \R^{\numLinks}$ that both satisfy the fixed point equation \eqref{eq: pEquilibrium}, therefore for every \(r\in[\numLinks]\):
\begin{align*}
    \fixedPointPrice_r &= \fixedPointFlow_r(\fixedPointPrice) \grad_x \costEdge_r(\fixedPointFlow_r(\fixedPointPrice)) \\ \fixedPointPrice_r' &= \fixedPointFlow_r(\fixedPointPrice') \grad_x \costEdge_r(\fixedPointFlow_r(\fixedPointPrice'))
\end{align*}
Taking the difference we get 
\begin{align*}
    \fixedPointPrice_r - \fixedPointPrice_r' &= \fixedPointFlow_r(\fixedPointPrice) \grad_x \costEdge_r(\fixedPointFlow_r(\fixedPointPrice)) - \fixedPointFlow_r(\fixedPointPrice') \grad_x \costEdge_r(\fixedPointFlow_r(\fixedPointPrice')) , \\ 
    &= \fixedPointFlow_r(\fixedPointPrice) \grad_x \costEdge_r(\fixedPointFlow_r(\fixedPointPrice)) - \fixedPointFlow_r(\fixedPointPrice') \grad_x \costEdge_r(\fixedPointFlow_r(\fixedPointPrice))\\
    &\quad \quad \quad + \fixedPointFlow_r(\fixedPointPrice') \grad_x \costEdge_r(\fixedPointFlow_r(\fixedPointPrice)) - \fixedPointFlow_r(\fixedPointPrice') \grad_x \costEdge_r(\fixedPointFlow_r(\fixedPointPrice')),  \\
    &= \lr{\fixedPointFlow_r( \fixedPointPrice)-\fixedPointFlow_r(\fixedPointPrice')}   \grad_x\costEdge_r(\fixedPointFlow_r(\fixedPointPrice))\\&\quad\quad\quad +\fixedPointFlow_r(\fixedPointPrice')\lr{\grad_x \costEdge_r(\fixedPointFlow_r(\fixedPointPrice))-\grad_x\costEdge_r(\fixedPointFlow_r(\fixedPointPrice'))},
\end{align*}
for every \(r\in[\numLinks]\). Multiplying \((\fixedPointFlow_r(\fixedPointPrice)-\fixedPointFlow_r(\fixedPointPrice'))\) in the preceding equation we obtain
\begin{equation}
\begin{aligned}\label{eq: pUniquenessContradiction}
    &(\fixedPointFlow_r(\fixedPointPrice)-\fixedPointFlow_r(\fixedPointPrice'))(\fixedPointPrice_r - \fixedPointPrice_r') = \lr{\fixedPointFlow_r(\fixedPointPrice)-\fixedPointFlow_r(\fixedPointPrice')}^2\grad_x \costEdge_r(\fixedPointFlow_r(\fixedPointPrice))\\&\quad\quad\quad +\fixedPointFlow_r(\fixedPointPrice') \lr{\grad_x \costEdge_r(\fixedPointFlow_r(\fixedPointPrice))-\grad_x \costEdge_r(\fixedPointFlow_r(\fixedPointPrice'))} (\fixedPointFlow_r(\fixedPointPrice)-\fixedPointFlow_r(\fixedPointPrice')), 
\end{aligned}
\end{equation}
for every \(r\in[\numLinks]\). Convexity of the edge cost function ensures that right hand side of \eqref{eq: pUniquenessContradiction} is always non-negative for every \(r\in[\numLinks]\). 
Summing over \(r\in[R]\) and using Lemma \ref{lem: MonotonicityFlow} we obtain:
\begin{align*}
    0>\lara{ \fixedPointFlow_r(\fixedPointPrice)-\fixedPointFlow_r(\fixedPointPrice'), \fixedPointPrice-\fixedPointPrice' } \geq 0.
\end{align*}
which contradicts our original hypothesis that there are two distinct price profiles satisfying \eqref{eq: pEquilibrium}. Therefore the existence result Proposition \ref{prop: pEqExists} ensures uniqueness. 
\end{proof}

The existence and uniqueness results presented above, interestingly, ensure that for any toll price \(p\), \(\fixedPointFlow(p)\) approaches the Wardrop(selfish) equilibrium as we let the perturbation parameter \(\beta\) to infinity. Furthermore, in the limit the equilibrium pricing ensures that the emergent flow on the network are socially optimal. This result is formalized in the result below. 

\todo{Should we make this a theorem? Also we want $\bar{p}$ to be the socially optimal marginal cost price.}
\begin{proposition}[\textbf{Social optimality of \(\fixedPointFlow(\fixedPointPrice^{(\beta)})\)}]\label{prop: ConnectionToWardrop}
For any \(\beta>0\), the equilibrium flow \(\fixedPointFlow(\fixedPointPrice^{(\beta)})\) is the minimizer of the following strictly convex optimization problem:

\end{proposition}
The proof of Proposition \ref{prop: ConnectionToWardrop} follows by comparing the variational inequalities associated with \eqref{eq: OptimizationProblem} ( at \(p=\fixedPointPrice^{(\beta)}\) ) and \eqref{eq: SocialCostWE}. 
The details of the proof can be found in Appendix \ref{proof: PropWardrop}. 
\begin{remark}
The cost function in \eqref{eq: SocialCostWE} is an entropy regularized social cost function. Note that in the limit \(\beta\uparrow \infty\), for any \(p\in \R^{\numLinks}\) the flow \(\fixedPointFlow(p)\) converges to the static Wardrop assignment \cite{cominetti2012modern}. Furthermore, as \(\beta\uparrow +\infty\), the equilibrium flow \(\fixedPointFlow(\fixedPointPrice^{(\beta)})\) converges to the socially optimal flow \cite{roughgarden2010algorithmic}.
\end{remark}



\subsection{Convergence}\label{ssec: Convergence}
We shall first show that for any fixed \(\priceContinuous\in\R^{\numLinks}\), the trajectories of the dynamical system \eqref{eq: FixedPointFlowDynamics} converges to the equilibrium \(\fixedPointFlow(\priceContinuous)\). For this purpose we use results from \cite{hirsch1985systems} which is also stated in Theorem \ref{thm: HirshResult} for the sake of completeness.
\begin{proposition}\label{prop: ConvergenceFlowCont}
For any fixed \(p\in\R^{\numLinks}\) the point \(\fixedPointFlow(\priceContinuous)\) is a globally asymptotically stable equilibrium of  \eqref{eq: FixedPointFlowDynamics}.  
\end{proposition}
\begin{proof}
To prove this result we shall use Theorem \ref{thm: HirshResult}. For that purpose we need to check conditions Theorem \ref{thm: HirshResult}\ref{enum: Assm1}-\ref{enum: Assm4}.

The condition \ref{enum: Assm1} is satisfied if we show that \(\frac{\partial \vectorFieldX_i(\flowContinuous,\priceContinuous)}{\partial \flowContinuous_j} \geq 0\). Indeed, by definition 
\begin{align*}
    \frac{\partial h_i(x,p)}{\partial x_j}  = \frac{\meanInflow}{\meanOutflow} \exp(-\beta \costPrice_i(x_i,p_i)) \frac{\beta\exp(-\beta \costPrice_j(x_j,p_j) )\frac{\partial \costPrice_j(x_j,p_j)}{\partial x_j}}{\lr{\sum_{j\in[\numLinks]}\exp\lr{-\beta \costPrice_j(x_j,p_j)}}^2} > 0.
\end{align*}
The condition \ref{enum: Assm2} is also satisfied trivially because the Jacobian matrix has all the off-diagonal terms positive and is therefore irreducible. Moreover, it follows from \eqref{eq: hVectorFieldDef} that  for any \(x,p\in\R^{\numLinks}\) , \(\vectorFieldX_i(x,p) \in \lr{0,\frac{\meanInflow}{\meanOutflow}}\) and therefore \ref{enum: Assm3}-\ref{enum: Assm4} are also satisfied. This completes the proof.
\end{proof}


Before presenting the next result, we define some notations that will be helpful for concise presentation. Define \(\diagC(x) \defas \diag\lr{\lr{\grad_x \costEdge_i(x)}_{i=1}^{\numLinks}} \) and \(\diagMarginal(x) \defas \diag\lr{\lr{x_i\grad_x \costEdge_i(x)}_{i=1}^{\numLinks}}\). We shall now discuss the convergence of \eqref{eq: PriceDynamics} to the equilibrium \(\fixedPointPrice\). 
\begin{proposition}\label{prop: ConvergencePriceCont}
The equilibrium \(\fixedPointPrice\) is the globally asymptotically stable equilibrium of \eqref{eq: PriceDynamics}.
\end{proposition}
\begin{proof}
First, we show that $\fixedPointFlow(\priceContinuous)$ is a differentiable function of $\priceContinuous$. To do this, we invoke the implicit function theorem for that map $\fixedGap(x, p) = x - h(x, p)$.
Note that for any fixed \(p\), \(\fixedPointFlow(p)\) is the zero of \(\fixedGap(\cdot,p)\). To satisfy the hypothesis in implicit function theorem: for any \(\priceContinuous\) we compute the Jacobian of the function $\fixedGap(x, p)$ with respect to \(x\) and evaluate it at $\fixedPointFlow(\priceContinuous)$. Using Lemma \ref{lem: LipschitzFunction} the Jacobian is given by: 
\begin{align*}
   \grad_x \fixedGap(\fixedPointFlow(p),p) &= I - \grad_x \vectorFieldX(\fixedPointFlow(p),p) \\
   & = I - \frac{\meanOutflow}{\meanInflow}\beta\fixedPointFlow(p)\fixedPointFlow(p)^\top \diagC(\fixedPointFlow(p)) + \beta\diagMarginal\lr{\fixedPointFlow(p)} \\ 
   & = \lr{\lr{\diagMarginal^{-1}(\fixedPointFlow(p)) + \beta I}-\beta v\mathbbm{1}^\top}\diagMarginal(\fixedPointFlow(p)) 
\end{align*}
where \(v \defas \frac{\meanOutflow}{\meanInflow}\fixedPointFlow(p)\). Note that from \eqref{eq: xEquilibrium} we have \(\mathbbm{1}^\top v = 1\).
We claim that \(\det(D_x \fixedGap(\fixedPointFlow(p),p)) \neq 0\). Indeed, 
\begin{align*}
    \det(D_x \fixedGap(\fixedPointFlow(p),p)) &= \det\lr{\diagMarginal(\fixedPointFlow(p)} \det\lr{\lr{\diagMarginal^{-1}(\fixedPointFlow(p)) + \beta I}-\beta v\mathbbm{1}^\top }\\ 
   &= \det\lr{\diagMarginal(\fixedPointFlow(p)}\cdot
    \det\lr{I-\beta v\mathbbm{1}^\top\lr{\diagMarginal^{-1}(\fixedPointFlow(p)) + \beta I}^{-1} }\\&\quad\quad \cdot \det\lr{\diagMarginal^{-1}(\fixedPointFlow(p)) + \beta I}^{-1}
\end{align*}
It is sufficient to show that \( \det\lr{I-\beta v\mathbbm{1}^\top\lr{\diagMarginal^{-1}(\fixedPointFlow(p)) + \beta I}^{-1} }\neq 0\). Using the Sherman-Morrison formula \cite{gentle2007matrix} it is necessary and sufficient to show that \(\beta\mathbbm{1}^\top\lr{\diagMarginal^{-1}(\fixedPointFlow(p)) + \beta I}^{-1} v \neq 1 \). 

We show it by contradiction. Suppose \(\beta\mathbbm{1}^\top\lr{\diagMarginal^{-1}(\fixedPointFlow(p)) + \beta I}^{-1} v = 1 \). Then 
\begin{align*}
&\implies \quad \sum_{i=1}^{\numLinks} v_i \frac{\beta}{\frac{1}{m_i}+\beta} = 1\\
&\implies \quad \sum_{i=1}^{\numLinks} v_i \frac{\beta}{\frac{1}{m_i}+\beta} = \sum_{i=1}^{\numLinks} v_i \\ 
&\implies \sum_{i=1}^{\numLinks} v_i\frac{\frac{1}{m_i}}{\beta+\frac{1}{m_i}} = 0
\end{align*}
This is not possible as the terms on the left hand side are all positive. 
% \begin{align}
%     J_{g, \flowContinuous}(\fixedPointFlow(\priceContinuous) , \priceContinuous) &= \begin{bmatrix} \frac{\partial \hat{g_i}(\fixedPointFlow(\priceContinuous), \priceContinuous)}{\partial \flowContinuous_j} \end{bmatrix} \\ & = I_{R \times R} - \begin{bmatrix} \frac{\partial h_i(\fixedPointFlow(\priceContinuous) , \priceContinuous)}{ \partial \flowContinuous_j}\end{bmatrix} \\ &=  I_{R \times R} - \frac{\meanInflow}{\meanOutflow} \begin{bmatrix} \begin{cases} \frac{\lr{\sum_{j\in[\numLinks]}\exp\lr{-\beta \costPrice_j(\fixedPointFlow_j(\priceContinuous),\priceContinuous_j)}}  \exp(-\beta \costPrice_i(\fixedPointFlow_i (\priceContinuous), \priceContinuous_i)}{\lr{\sum_{j\in[\numLinks]}\exp\lr{-\beta \costPrice_j(\fixedPointFlow_j(\priceContinuous),\priceContinuous_j)}}^2} \text{ if } i = j \\  \exp(-\beta \costPrice_i(\fixedPointFlow_i(\priceContinuous),\priceContinuous_i)) \frac{\beta\exp(-\beta \costPrice_j(\fixedPointFlow_j(\priceContinuous),\priceContinuous_j) )\frac{\partial \costPrice_j(\fixedPointFlow_j(\priceContinuous),\priceContinuous_j)}{\partial x_j}}{\lr{\sum_{j\in[\numLinks]}\exp\lr{-\beta \costPrice_j(\fixedPointFlow_j(\priceContinuous),\priceContinuous_j)}}^2} \text{ if } i \neq j \end{cases} \end{bmatrix}
% \end{align}    

% \todo[inline]{We need to show that the operator \(\R^R\ni p  \mapsto F(\fixedPointFlow(p)) \defas \fixedPointFlow(p)\odot \partial_x c(\fixedPointFlow(p))\in \R^R\) is monotone}

% \begin{align*}
% &\lara{ p-p',\fixedPointFlow(p)\odot\partial_x\costEdge(\fixedPointFlow(p)) -\fixedPointFlow(p')\odot\partial_x\costEdge(\fixedPointFlow(\fixedPointPrice))} = \sum_{r\in[R]}(p_r-p_r')((\fixedPointFlow_r(p))^4-(\fixedPointFlow_r(p'))^4)\\
% &= \sum_{r\in[R]}(p_r-p_r')((\fixedPointFlow_r(p)-\fixedPointFlow_r(p')(\fixedPointFlow_r(p)+\fixedPointFlow_r(p'))(\fixedPointFlow_r(p))^2+(\fixedPointFlow_r(p'))^2)
% \end{align*}

% Monotonicity 
% \[
% \sum_{r}(p_r-p_r')(\fixedPointFlow_r(p)-\fixedPointFlow_r(p')) < 0
% \]

% \todo[inline]{For the cooperative dynamics ideas to work it suffices to show that \(\partial \fixedPointFlow_i(p)/\partial p_j > 0\) for \(i\neq j\)}

% Alternatively: 

% \begin{itemize}
%     \item First show that $\frac{\partial \fixedPointFlow (p) \partial_x c(\fixedPointFlow(p))}{\partial x_j} > 0$ to guarantee the convergence of $p(t)$ to the set of equilibria with high probability. 
% \end{itemize}

% \textbf{Claim:} The minimizer $x^*$ of $S(x) = \sum_{i=1}^{R} x_i c_i(x_i)$ is unique because $S(x)$ is a convex function. 

% \textbf{Proof:} $S(x)$ is the sum of the product of nondecreasing convex functions $x_i$ and $c_i(x_i)$. 

% \textbf{Claim:} The marginal cost tax $p_i = x_i c_i'(x_i)$ such that for $(R , \zeta, c_i)$, the equilibrium flow $x^{*}$ of $(R , \zeta, c_i + p_i)$ minimizes $S(x)$ is unique. 

% \textbf{Recall:} The equilibrium $\bar{p}$ satisfies the fixed point equation $\bar{p}_i = \fixedPointFlow_i(\bar{p}) \partial_x c_i(\fixedPointFlow_i(\bar{p}))$

 

% \begin{equation}
% \begin{aligned}
%     \min_{y\in \R^{\numLinks}} &\quad \ell(y)\defas \sum_{r\in [\numLinks]} \int_{0}^{y_r} \costEdge_r(s)+p_rds + \frac{1}{\beta} \sum_{r\in [\numLinks]} y_r \ln{y_r} \\
%     \text{s.t} & \quad \sum_{r\in[\numLinks]} y_r = \frac{\meanInflow}{\meanOutflow}
% \end{aligned}
% \end{equation}

% \(\fixedPointFlow(p)\) is minimizer of above. \(p=\bar{p}\) then \(\fixedPointFlow(\bar{p})\) is minimizer of 
% \begin{equation}
% \begin{aligned}
%     \min_{y\in \R^{\numLinks}} &\quad \ell(y)\defas \sum_{r\in [\numLinks]} \int_{0}^{y_r} \costEdge_r(s)+\fixedPointFlow(\bar{p})\partial_xc_r(\fixedPointFlow(\bar{p}))ds + \frac{1}{\beta} \sum_{r\in [\numLinks]} y_r \ln{y_r} \\
%     \text{s.t} & \quad \sum_{r\in[\numLinks]} y_r = \frac{\meanInflow}{\meanOutflow}
% \end{aligned}

% \end{equation}


We shall now show that \eqref{eq: PriceDynamics} satisfies conditions \ref{enum: Assm1}-\ref{enum: Assm4} in Theorem \ref{thm: HirshResult}. This ensures global convergence to the equilibrium set which is guaranteed to be singleton by Proposition \ref{prop: pEqExists}. 
For better presentation, for any \(i,j\in[\numLinks]\), we shall concisely denote the gradient of \(\fixedPointFlow_i(\priceContinuous)\) with respect to \(\priceContinuous_j\) by \(\grad_j \fixedPointFlow(\priceContinuous)\).  
Using \eqref{eq: xEquilibrium} for any \(i\neq j\) we have
\begin{align}
    \exp(-\beta \costPrice_j(\fixedPointFlow_j(\priceContinuous),\priceContinuous_j)) \fixedPointFlow_i(\priceContinuous)= \exp(-\beta \costPrice_i(\fixedPointFlow_i(\priceContinuous),\priceContinuous_i)) \fixedPointFlow_j(\priceContinuous)
\end{align}
Taking derivative of the above equation with respect to \(\priceContinuous_k\) for \(k\neq i\neq j\): 
\begin{align*}
    & \exp(-\beta \costPrice_j(\fixedPointFlow_j(\priceContinuous),\priceContinuous_j))\grad_k\fixedPointFlow_i(\priceContinuous) \\&\quad + \fixedPointFlow_i(\priceContinuous)\exp(-\beta \costPrice_j(\fixedPointFlow_j(\priceContinuous),\priceContinuous_j))(-\beta \grad_x\costPrice_j(\fixedPointFlow_j(\priceContinuous),\priceContinuous_j) \grad_k \fixedPointFlow_j(\priceContinuous)) \\ 
     &= \exp(-\beta \costPrice_i(\fixedPointFlow_i(\priceContinuous),\priceContinuous_i))\grad_k\fixedPointFlow_j(\priceContinuous) \\ &\quad  + \fixedPointFlow_j(\priceContinuous)\exp(-\beta \costPrice_i(\fixedPointFlow_i(\priceContinuous),\priceContinuous_i))(-\beta \grad_x\costPrice_i(\fixedPointFlow_i(\priceContinuous),\priceContinuous_i) \grad_k \fixedPointFlow_i(\priceContinuous)).
\end{align*}
Collecting similar terms together we get 
\begin{align*}
    &\grad_k\fixedPointFlow_i(\priceContinuous)\lr{\exp(-\beta \costPrice_j(\fixedPointFlow_j(\priceContinuous),\priceContinuous_j))} \\&\quad + \grad_k\fixedPointFlow_i(\priceContinuous)\lr{\fixedPointFlow_j(\priceContinuous)\exp(-\beta \costPrice_i(\fixedPointFlow_i(\priceContinuous),\priceContinuous_i))(\beta \grad_x\costPrice_i(\fixedPointFlow_i(\priceContinuous),\priceContinuous_i) )} \\
    &= \grad_k\fixedPointFlow_j(\priceContinuous) \lr{\exp(-\beta \costPrice_i(\fixedPointFlow_i(\priceContinuous),\priceContinuous_i))} \\&\quad + \grad_k\fixedPointFlow_j(\priceContinuous) \lr{ \fixedPointFlow_i(\priceContinuous)\exp(-\beta \costPrice_j(\fixedPointFlow_j(\priceContinuous),\priceContinuous_j))(\beta \grad_x\costPrice_j(\fixedPointFlow_j(\priceContinuous),\priceContinuous_j) )} .
\end{align*}
This implies for \(i\neq j\neq k\) and for any \(p\in\R^{\numLinks}\) we have
\begin{align}\label{eq: SameSign}
\grad_k \fixedPointFlow_i(\priceContinuous) \cdot \grad_k \fixedPointFlow_j(\priceContinuous) > 0.
\end{align}
Moreover, by definition of fixed point in \eqref{eq: xEquilibrium} we have the constraint that
\[
\sum_{l\in[\numLinks]}\fixedPointFlow_l(p) = \frac{\lambda}{\mu}.
\]
Taking derivative with respect to \(\priceContinuous_k\) of the above equation we obtain
\begin{align}\label{eq: DerivativeConstraint}
\sum_{l\neq k} \grad_k\fixedPointFlow_l(p) = - \grad_k\fixedPointFlow_k(p) > 0,
\end{align}
where the last inequality follows from Lemma \ref{lem: MonotonicityFlow}. Equation \eqref{eq: DerivativeConstraint} in conjunction with \eqref{eq: SameSign} implies that \(\grad_k \fixedPointFlow_i(p) > 0\) forall \(i\neq k\). This ensures satisfaction of \ref{enum: Assm1}-\ref{enum: Assm2}. The requirement \ref{enum: Assm3}-\ref{enum: Assm4} is also satisfied as for any \(p\in\R^{\numLinks}\), \(\fixedPointFlow(\priceContinuous)\in \lr{0,\frac{\meanInflow}{\meanOutflow}}\). This completes the proof. 
\end{proof}

\todo[inline]{Merge this with section 3.2}
\subsection{Properties of discrete-time stochastic process \eqref{eq: CombinedDT}}\label{ssec: SATheoryConvergence}
% \tdBox{Need to think about the Lipschitz property of p dynamics \eqref{eq: PriceDynamics}. Somehow need to use the property that \(\|X(n)\|\) is bounded a.s. May be we can make arguments such as if we keep \(\mu\) small then process \(X(n)\) will track its asymptotically stable system closely and therefore we can get the Lipschitzness of the dynamics of p. Need to make this formal. May be the arguments of the form: 
% \[
% \Pr(\|X_n\|\geq R) \leq \frac{\avg[\|X_n\|^2]}{R^2} < \infty 
% \]

% \textbf{Update}: I think we should be fine here if we assume that support of \(\zeta\) is bounded and the support of \(\xi\) is contained strictly inside \((0,1)\). Then if we look at the discrete time dynamics in \(X\) then we obtain 
% \[
% X_{i}(n+1) = (1-\xi_i)X_i(n) + \zeta(n+1) h(X_n,P_n)+\mu M_{n}
% \]

% }
Observe that for any \(i\in[\numLinks]\),  \(\{\martingale_i(n+1)\}_n\) in \eqref{eq: MartingaleDefinition} is a martingale difference sequence with respect to the filtration \(\filtration_n = \sigma(\cup_{i\in[\numLinks]} \lr{\flowDiscrete_i(1),\inflow(1),\outflow_i(1),\dots,\flowDiscrete_i(n),\inflow(n),\outflow_i(n)} )\). Using the definition of martingale difference sequence \(\martingale_{i}(n+1)\) and assumptions on random variables $\{\inflow_i(n)\}_{n \in \mathbb{N}}$ and $\{\outflow(n)\}_{n \in \mathbb{N}}$ one can observe that there exists a finite scalar \(K>0\) such that 
\begin{align}\label{eq: martingaleBound}
    \avg[|\martingale_i(n+1)|^2|\filtration_n] \leq K\lr{1+\|\flowDiscrete_i(n)\|^2} \quad \forall i, n.
\end{align}


% The aim, now, is to understand whether the coupled stochastic process converges and to explicate its limiting behavior, with a goal towards showing asymptotic convergence to socially optimal flows. 

Our assumption that the random variables \(\inflow(n),\outflow(n)\)  have finite support ensures that  \(\flowDiscrete_n,\priceDiscrete_n\) in \eqref{eq: CombinedDT} are bounded almost surely. Specifically, \(\flowDiscrete_n\in\lr{0,\frac{\inflowUpper}{\outflowLower}}\) almost surely. This ensures that the vector fields in \eqref{eq: singularPerturbedODE}  are Lipschitz functions (as they take bounded sets to bounded sets).

We can therefore deploy the machinery of constant step-size two-timescale stochastic approximation presented in \cite[p. 112]{borkar2009stochastic}. 

\begin{theorem}\label{thm: BorkarSAConvergence}
The iterates of the stochastic process \eqref{eq: CombinedDT} will satisfy the following 
\begin{align}
    \limsup_{n\ra+\infty}\avg[\|\flowDiscrete_n-\fixedPointFlow(\fixedPointPrice)\|^2+\|\priceDiscrete_n-\fixedPointPrice\|^2] = \mathcal{O}(\meanOutflow)+\mathcal{O}\lr{\frac{a}{\meanOutflow}}.
\end{align}
\end{theorem}
\begin{proof}
The proof of the above theorem follows by observing that the modelling assumptions posited in \S\ref{sec: Model} and the properties of approximating continuous time dynamical system derived in \S\ref{ssec: PropFixedPoint}-\S\ref{ssec: Convergence} satisfies all the standard hypothesis of constant step size two time scale stochastic approximation theory (refer \cite[p. 112]{borkar2009stochastic}). 
\end{proof}



==> setup.tex <==
\section{Setup}
We now introduce the time-dynamical model that models inflows and outflows on the network, along with an adaptive tolling scheme. We show that over time, the tolling scheme converges to a price that induces a socially optimal flow, as in the sense of minimizing the function in \ref{thm: SocialCost}.


There is an $\numLinks$-link parallel network and a pair of nodes connecting them. At every time $n \in \mathbb{N}$, there is $\flowDynamic_i(n)$ units of flow present on the $i$-th link. Each link is endowed with a cost function $\costLink_i(\cdot, \cdot) :\mathbb{R} \times \mathbb{R} \rightarrow \mathbb{R}$.  For any link \(i\in[\numLinks]\) and \(n\in\N\) the toll prices are denoted by $\priceDynamic_i(n) \in \mathbb{R}$. Therefore, $C_i$ is now a function of both the flow and the price on each link $i$.

\begin{assumption}
$C_i(\cdot, \cdot)$ is increasing in both arguments and convex in the first. 
\end{assumption}


\subsection{Routing Dynamics}
We consider the following routing dynamics and study the convergence of the flow process to a socially optimal profile. : 
\begin{align}
\flowDynamic_i(n+1) & = 
\flowDynamic_i(n) + 
\frac{\exp(-\beta 
\costLink_i(\flowDynamic_i(n), 
\priceDynamic_i(n)))}{\sum_{j=1}^{R}  \exp (-\beta 
\costLink_j(\flowDynamic_j(n), 
\priceDynamic_j(n)))} \zeta(n+1) - 
\xi_i(n+1) \flowDynamic_i(n) \\ &= 
\flowDynamic_i(n) + \mu \left( 
\frac{\lambda}{\mu} 
\frac{\exp(-\beta 
\costLink_i(\flowDynamic_i(n), 
\priceDynamic_i(n)))}{\sum_{j=1}^{R}  \exp (-\beta\costLink_j( 
\flowDynamic_j(n), 
\priceDynamic_j(n)))} - 
\flowDynamic_i(n) \right) + \mu M_i(n+1) \\
\priceDynamic_i(n+1) &= (1-a)\priceDynamic_i(n) + a  \flowDynamic_i(n) \frac{\partial C_i}{\partial x_i}(\flowDynamic_i(n), \priceDynamic_i(n))
\end{align}
We define the basic quantities used in the routing dynamic:

\begin{definition} 
The function
\begin{align}
    (X_i(n), P_i(n)) \rightarrow \frac{\exp(- \beta C_i(X_i(n), P_i(n))}{\sum_{j=1}^{R} \exp(-\beta C_i(X_i(n), P_i(n)))}
\end{align}
is the \emph{route choice model}. $\zeta(n)$, the \emph{inflow rate}, is an i.i.d. random variable with mean $\mu$. $\xi_i(n)$, the \emph{completion rate on link $i$}, is an i.i.d. random variable with mean $\lambda. $
\end{definition}

We assume $\mu < \lambda R$ to ensure stability (the inflow rate is smaller than the net outflow rate).

\begin{proposition}
When $a = 0$, and $\beta \nearrow \infty$, $X_i(n) \rightarrow \bar{X}$ where $\bar{X}$ is the (unique) Wardrop equilibrium. 
\end{proposition}

\begin{proposition}
When $a << \mu$, $x_i(n) \rightarrow x^{*}$, where $x^{*}$ is an optimal flow for the social cost function $S(x) = x_i C_i(x_i)$ for $\beta \rightarrow \infty$.
\end{proposition}

\begin{lemma}
$\bar{X}(p)$ is monotone in $p$. 
\end{lemma}

\begin{assumption}\label{assm: CostAssumption}
We assume that for any \(i \in [\numLinks]\),  \(\costPrice_i(x_i,p_i) \defas \costLink_i(x_i)+p_i\). Moreover, for every \(i\in [\numLinks]\)  \(\frac{\partial \costLink_i(x)}{\partial x} > 0. \)
\end{assumption}
For any \(p\in \R^{\numLinks}\), let's define the following continuous time ode 
\begin{align}
\label{eq: continuousDyn}
    \dot{x}_i(t) = \frac{\meanOutflow}{\meanInflow} \frac{\exp\lr{-\beta \costPrice_i(x_i(t),p_i)}}{\sum_{j\in[\numLinks]}\exp\lr{-\beta \costPrice_j(x_j(t),p_j)}} - x_i(t), \quad \forall i \in [\numLinks] 
\end{align}

Define \(h_i(x;p) \defas  \frac{\meanOutflow}{\meanInflow} \frac{\exp\lr{-\beta \costPrice_i(x_i,p_i)}}{\sum_{j\in[\numLinks]}\exp\lr{-\beta \costPrice_j(x_j,p_j)}}\) for \(i\in [\numLinks]\). We claim that \(\frac{\partial h_i(x;p)}{\partial x_j} > 0\) for all \(i\neq j\). Indeed 

where the inequality follows from Assumption \ref{assm: CostAssumption}.
It now follows from \cite[Theorem 5.1]{hirsch1985systems} that for any \(p\in \R^{\numLinks}\) the trajectories of \ref{eq: continuousDyn} converges to the set \(\EXSet(p) \defas \{x\in \R^{\numLinks}: h(x;p) = x\}\). We claim that for every \(p\in\R^{\numLinks}\), \(E(p)\) is a singleton set. 

We further check that the forward orbit $O_{+}(x)$, which is the image of the curve $t \rightarrow \phi_t(x)$, $t \in I(x)$, and $\phi_t(x)$ is the flow of the differential equation $\dot{x} = h(x;p)$, has a compact closure. To do this we check conditions from  \cite[Theorem 5.1]{hirsch1985systems}. Namely:

\begin{enumerate}
    \item The ode is cooperative and irreducible (i.e. the matrix $[\frac{\partial h_i}{\partial x_j}](x;p)$ is irreducible for every $x$ and $p$).
    \item $h_i(0) \geq 0$ \\
    \item For any $x \in \mathbb{R}^R_{+}$ there exists $y > x$ (entrywise) with $h_i(y;p) < 0$ for all $i$.  
\end{enumerate}

(1) is checked earlier. (2) is trivial because $h_i(0) = \frac{\lambda}{\mu} \frac{\exp(-\beta \tilde{C}(0,p_i)}{\sum_{j \in [\numLinks]} \exp(-\beta \costPrice(0, p_j)} \geq 0$. (3) holds because 




Define \(g(x;p) \defas h(x;p) -x\). Naturally, we can write \eqref{eq: continuousDyn} as \(\dot{x} = g(x;p)\). For any \(x\in \R^{\numLinks}\), we define 
\[
g_{\infty}(x;p) \defas \lim_{s\ra\infty}\frac{g(sx;p)}{s} = \lim_{s\ra\infty} \frac{h(sx;p)}{s} - x = -x 
\]
The equality follows because \(h(\cdot;p)\) is bounded for any \(p\in\R^{\numLinks}\). Therefore, the ode \(\dot{y}(t)  =g_{\infty}(y(t);p)\) has origin as its globally asymptotically (exponentially, to be precise) stable equilibrium. 


\begin{align}
\label{eq: continuousDyn}
     \frac{\meanOutflow}{\meanInflow} \frac{\exp\lr{-\beta \costPrice_i(x_i(p),p_i)}}{\sum_{j\in[\numLinks]}\exp\lr{-\beta \costPrice_j(x_j(p),p_j)}} &= x_i(p), &&\quad \forall i \in [\numLinks] \\
    x_i(p) \frac{\partial C_i(x_i(p),p_i)}{\partial x_i} &= p_i&&\quad \forall i \in [\numLinks]
\end{align}


\section{Outline of lemmas}
\begin{enumerate}
    \item Existence of $p*$ through Brouwer fixed point theorem ($\bar{X}(p) \frac{\partial C}{\partial x}(\bar{X}(p), p)$ takes bounded sets to bounded sets). 
    \item Product of nonnegative monotonic functions is monotonic. 
    \item Show that \(\bar{X}(p,\beta)\) is monotonic in p 
    \item Use Lyapunov argument 
\end{enumerate}
